Quiet Triggers, Loud Footprints: A Tri-Space Measurement Study of Backdoor Stealthiness

Backdoor attacks on deep neural networks are commonly evaluated by attack success rate and benign accuracy, yet their stealthiness remains inconsistently defined and measured. Existing work often studies only one observable aspect of stealthiness, such as trigger imperceptibility, feature-space separability, parameter-space concentration, or evasion of particular defenses. This creates a fragmented picture: an attack may appear stealthy under one metric while leaving conspicuous footprints elsewhere. This paper presents a tri-space measurement study of backdoor stealthiness in image classification. We distinguish latent stealthiness---the ideal but unobservable difficulty of distinguishing a backdoored system from a benign one---from measurable footprints in three spaces: input, feature, and parameter space. Under this framework, we evaluate representative backdoor attacks across four datasets and three model architectures using a broad suite of footprint metrics. Our results show that stealthiness is not monolithic: attacks that are quiet in one space are often loud in another, and existing attacks rarely achieve consistently small footprints across all three spaces. We further analyze agreement and disagreement among stealthiness metrics and study how footprint measurements interact with attack success rate. Based on observed blind spots in existing measurements, we introduce two diagnostic metrics: Class-Specific Davies--Bouldin Index (CDBI), which captures class-conditional feature overlap, and TAC--UCLC Product (TUP), which identifies channels that are both trigger-responsive and downstream influential. These metrics are intended to augment, not replace, the broader measurement suite. Finally, we provide practical guidance for future stealthiness evaluations.

==> sections/analyses/analysis1.tex <==


\section{Metric Disagreement}
\label{sec:metric_disagreement}

A prerequisite for any stealthiness benchmark is to know whether its metrics are
interchangeable estimates of one underlying property or whether they capture distinct,
non-substitutable footprints. We test this directly. We orient all sixteen footprint metrics
so that a larger value always denotes a larger footprint (i.e.\ less stealth), inverting the
four metrics for which higher is stealthier (PSNR, SSIM, pHash, and CDBI). Treating each
backdoored ResNet18 configuration: dataset $\times$ attack $\times$ poisoning
rate as one observation, we compute pairwise Spearman rank correlations
($\rho$). We use Spearman because we care about agreement on the ordering of attacks,
not the linear scale of any metric.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.92\linewidth]{img/metric_rank_correlation.pdf}
%     \caption{Spearman rank correlation among stealthiness footprint metrics, after orienting
%     every metric so that larger values indicate a larger footprint (less stealth). Each
%     backdoored ResNet18 configuration (dataset $\times$ attack $\times$ poisoning rate,
%     $N{=}76$) is one observation; $*$ marks $p<0.05$. Black lines separate the input,
%     feature, and parameter spaces. Metrics cluster within spaces but largely disagree across
%     them: the input block is highly redundant, whereas input--feature and input--parameter
%     correlations are near zero or negative. This supports tri-space reporting rather than a
%     single stealthiness scalar.}
%     \label{fig:metric_correlation}
% \end{figure*}

\begin{table}[t]
\centering
\caption{Average Spearman rank correlation among footprint metrics, within vs.\ across
spaces. ``Within-dataset'' correlations are computed per dataset and averaged (Fisher $z$),
which removes cross-dataset scale confounds; ``pooled'' treats all $76$ configurations as one
sample. Agreement is high within the input space, weaker within the feature and (especially)
parameter spaces, and collapses across spaces.}
\label{tab:metric_agreement}
\begin{tabular}{lcc}
\toprule
\textbf{Metric group} & \textbf{Within-dataset $\rho$} & \textbf{Pooled $\rho$} \\
\midrule
Input--Input          & $+0.69$ & $+0.66$ \\
Feature--Feature      & $+0.61$ & $+0.57$ \\
Parameter--Parameter  & $+0.50$ & $+0.27$ \\
\midrule
Input--Feature        & $-0.09$ & $-0.11$ \\
Input--Parameter      & $-0.28$ & $-0.24$ \\
Feature--Parameter    & $+0.42$ & $+0.35$ \\
\bottomrule
\end{tabular}
\end{table}

\autoref{fig:metric_correlation} and \autoref{tab:metric_agreement} show that the metrics are
not interchangeable. Agreement is strongest within the input space (within-dataset
$\bar\rho{=}{+}0.69$, pooled ${+}0.66$), where several metrics are near-duplicates: MSE and
PSNR are rank-identical by construction ($\rho{=}1.00$), and SSIM and LPIPS agree at
$\rho{\approx}0.90$. The lone exception is $\ell_\infty$, which is nearly uncorrelated with or
opposite to the other input metrics (e.g.\ $\rho(\ell_1,\ell_\infty){=}{-}0.08$,
$\rho(\mathrm{SAM},\ell_\infty){=}{-}0.33$), because patch triggers perturb a few pixels
maximally while warping/blending triggers spread small changes over the whole image. Agreement
weakens within the feature space (within-dataset $\bar\rho{=}{+}0.61$; e.g.\
$\rho(\mathrm{SS},\mathrm{DSWD}){=}0.49$) and is weakest within the parameter space
(within-dataset $\bar\rho{=}{+}0.50$). Parameter agreement is also the most scale-sensitive:
UCLC and TAC agree only moderately within a dataset ($\rho{=}0.44$) and appear uncorrelated
once datasets are pooled ($\rho{=}0.04$, the near-white cell in \autoref{fig:metric_correlation}),
because activation magnitudes differ sharply across datasets. Either way, metrics built to
probe the same space rank attacks differently, so the choice of metric materially
changes the stealthiness conclusion.

Across spaces, the divergence is starker. Input--feature and input--parameter correlations are
essentially zero or negative (\autoref{tab:metric_agreement}). The negative input--parameter
trend is itself informative: TUP correlates negatively with the input-space metrics
(e.g.\ $\rho(\ell_1,\mathrm{TUP}){=}{-}0.68$, $\rho(\mathrm{IS},\mathrm{TUP}){=}{-}0.51$),
quantifying the trade-off in our title---attacks that are quiet in the input space (BadNets,
BppAttack) tend to be loud in the parameter space, while the input-loud clean-label attacks
(Narcissus, Grond) are parameter-quiet. The only non-trivial cross-space agreement is
feature--parameter ($+0.42$ within-dataset, $+0.35$ pooled), and it attenuates when we restrict
to effective attacks (ASR\,$\ge$\,$60\%$: $+0.35\rightarrow+0.29$ pooled), indicating it is
partly an attack-strength effect rather than a shared stealthiness signal, an effect we
isolate in \autoref{sec:asr_sensitivity}.

Two clarifications scope these results. First, SS and CDBI are strongly rank-correlated
overall ($\rho{\approx}0.89$ pooled, $0.78$ within-dataset), confirming that CDBI is a
feature-space metric in the same family as SS rather than an unrelated quantity; the regimes in
which the two diverge and in which CDBI is the more faithful measure are the subject
of \autoref{sec:cdbi_disagreement}. Second, the within-dataset and pooled summaries in
\autoref{tab:metric_agreement} agree in their qualitative ordering, but pooling across datasets
with very different activation scales deflates parameter-space agreement ($\bar\rho$ from
$0.50$ to $0.27$); we therefore report within-dataset correlations as the primary summary and
display the pooled matrix (with significance) in \autoref{fig:metric_correlation}. Taken
together, these results establish the central premise of our study: a small footprint under one
metric, or in one space, does not imply a small footprint elsewhere. Stealthiness is therefore
a multi-view measurement problem, and a claim of stealthiness must state which footprint
it refers to rather than treating stealthiness as a single scalar.





==> sections/analyses/analysis2.tex <==
\section{How Does CDBI Differ from SS?} \label{sec:cdbi_disagreement}
We next examine cases that highlight the extent to which CDBI and SS lead to different interpretations of feature-space stealthiness. SS treats the clean and poisoned samples as two global clusters. This can penalize poisoned samples that fragment by source class, even when each source-class fragment overlaps with the benign target-class region. CDBI instead evaluates overlap class-conditionally.

Table~\ref{tab:ss_cdbi_disagreement} reports ranking differences between the two metrics. As seen in \autoref{app:t-sne}, samples poisoned by WaNet form subgroups based on their source class. SS penalizes this weak global cohesion, whereas CDBI measures whether each subgroup is close to the benign target-class cluster. This explains the large difference in rank.

Another case where poisoned samples cluster by their source class is Adap-Blend. However, this attack achieves not only the lowest SS, but also the lowest CDBI. Grond ranks slightly higher with both metrics, but we would argue it is more stealthy than Adap-Blend, judging from the t-SNE embeddings. Therefore, the cases of Adap-Blend and Grond show a limitation in both SS and CDBI. This limitation is still present in CDBI because Adap-Blend also poisons target-class samples. These samples have high feature-space overlap with benign samples, skewing the class-conditional average computed by CDBI.

Another limitation shared by both metrics is their preference for low-ASR attacks. The poisoned samples in these attacks may remain close to benign samples in feature space precisely because the backdoor was not successfully injected. Therefore, SS and CDBI should always be interpreted together with ASR; they should not be used alone to claim successful feature-space stealthiness.

\begin{table}[t]
    \centering
    \caption{Representative SS--CDBI rankings computed within the same dataset, model architecture and poisoning rate after orienting both metrics so that lower rank indicates smaller feature-space footprint.}
    \label{tab:ss_cdbi_disagreement}
    
    \begin{tabular}{lcccc}
    
        \toprule
        
        \textbf{Dataset} & PR & \textbf{Attack} & \textbf{SS rank} & \textbf{CDBI rank} \\
        
        \midrule

        CIFAR-10 & 5\% & WaNet & 3/9 & 7/9 \\
        CIFAR-10 & 5\% & Adap-Blend & 1/9 & 1/9 \\
        CIFAR-10 & 5\% & Grond & 4/9 & 3/9 \\
        
        \bottomrule
    
    \end{tabular}
\end{table}

==> sections/analyses/analysis3.tex <==
\section{How Does TUP Differ from UCLC and TAC?} \label{sec:tup_disagreement}
UCLC and TAC measure different aspects of a parameter-space footprint. UCLC estimates downstream influence, but a high-UCLC channel need not be trigger-relevant. TAC measures trigger-induced activation change, but a high-TAC channel need not be influential for the final prediction. For example, TAC can be high simply because a trigger leaves a large footprint in input space. To avoid this, we have defined the TAC ratio $R_j$ in \autoref{sec:new_metrics:tup}.

TUP computes the product between the UCLC and TAC ratio of each channel, and then takes the average. The metric is designed to highlight channels that are both influential for the final prediction and sensitive to the trigger. To test this behavior, we plot the channel-wise TUP measurements for several backdoored models in \autoref{fig:tup_scatter}. We have selected the models with the highest and lowest TUP on CIFAR-10, CIFAR-100 and Imagenette. %\todo{Henk: I can also add Tiny ImageNet here}

\definecolor{highTUP}{HTML}{fde725}
\definecolor{midTUP}{HTML}{a0f43c}
\definecolor{lowTUP}{HTML}{440154}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/parameter_correlation}
    \caption{TAC-UCLC Product (TUP) measurements for each channel in the final layer of backdoored models. Channels are colored from \textcolor{lowTUP}{lowest} \textcolor{midTUP}{to} \textcolor{highTUP}{highest} TUP, and the top-10 channels are outlined.}
    \label{fig:tup_scatter}
\end{figure}

We observe that most of the time, TUP indeed emphasizes the desired channels which are located in the upper-right region of the plots. The only exceptions are BppAttack on CIFAR-100 and Grond on Imagenette, where there is no positive correlation between UCLC and the TAC ratio. Therefore, these two metrics offer different views of parameter-space stealthiness, and combining them into the TUP metric can lead to new insights.

This analysis also illustrates TUP's limitations. TUP is a white-box evaluator metric because it requires the trigger transformation and internal activations. Moreover, attacks that distribute their backdoor functionality across many moderately affected channels may avoid producing a single extreme TUP channel. For example, \autoref{fig:tup_scatter} shows that the TUP measurements for the CIFAR-10 Grond model are all quite close. We therefore interpret TUP as a diagnostic for concentrated parameter-space footprints, not as a complete parameter-space stealthiness definition.

==> sections/analyses/analysis4.tex <==

\section{Sensitivity to Low-ASR Configurations}
\label{sec:asr_sensitivity}

Low-ASR configurations create an interpretation challenge: a small footprint may indicate
either a stealthy attack or a backdoor that was never successfully implanted. To test whether
our conclusions depend on such cases, we recompute the per-space attack rankings after
excluding configurations with ASR below $60\%$ and $80\%$. Rankings use the same within-dataset
percentile-footprint aggregation as \autoref{sec:metric_disagreement}, averaged over each
attack's surviving configurations; this removes $15$ and $25$ of the $76$ configurations,
respectively.

The central conclusions are stable (\autoref{tab:asr_sensitivity}). The stealthiest attack in
each space is unchanged across all three filters, BppAttack in the input space, Adap-Patch in
the feature space, and Grond in the parameter space, and no attack is stealthiest in all
three spaces under any filter. Even the most balanced attack, Grond, still sits near the
$42$nd loudness percentile in its worst space ($0.42$ on all configurations, $0.45$ at
ASR$\ge$$60\%$), so no attack occupies the stealthy tail of all three spaces simultaneously.
Rank stability is high within each space (Kendall's $\tau\!\ge\!0.91$ for the input and feature
spaces and $0.94/0.76$ for the parameter space; \autoref{tab:asr_stability} and
\autoref{fig:asr_rank_stability}).

Two points scope these results honestly. First, the strictest filter is data-limited for the
attacks that rarely reach high ASR: at ASR$\ge$$80\%$ the feature- and parameter-space winners
(Adap-Patch and Grond) survive on a single high-ASR configuration each. Grond is well supported
at ASR$\ge$$60\%$ ($5$ configurations), whereas Adap-Patch retains only $2$, it seldom reaches
high ASR, so its apparent feature-stealth must be read alongside its low ASR. Crucially,
however, even these few successful Adap-Patch and Grond configurations remain the
stealthiest in their respective spaces, so the per-space winners are not produced by failed
runs. Second, the composite cross-space ranking is
less stable ($\tau=0.73/0.56$) than any individual space; this is expected rather than
concerning, because the three spaces capture different footprints
(\autoref{sec:metric_disagreement}), which is precisely why we report per-space rather than a
single composite ranking.

Finally, the verdicts of our two proposed metrics are robust to attack effectiveness. CDBI
consistently identifies Narcissus as the stealthiest feature-space attack and TUP identifies
Grond as the stealthiest parameter-space attack (with Narcissus marginally overtaking at
ASR$\ge$$60\%$) across all filters. Because Narcissus and Grond retain successful, high-ASR
configurations, these rankings are not artifacts of failed backdoors; the distinct,
case-specific scenario in which CDBI can over-credit an individual low-ASR
configuration is examined in \autoref{sec:cdbi_disagreement}. Overall, excluding failed attacks
does not change which attacks are stealthy in which space, nor the conclusion that none is
stealthy across all three.


\begin{table*}[t]
\centering
\caption{Sensitivity of the main conclusions to ASR filtering. Per-space rankings use
within-dataset percentile footprints averaged over each attack's surviving configurations
(lower~$=$~stealthier). The per-space winners and the tri-space conclusion are unchanged when
low-ASR (failed) attacks are excluded.}
\label{tab:asr_sensitivity}
\begin{tabular}{lccc}
\toprule
\textbf{Conclusion} & \textbf{All configs} & \textbf{ASR$\ge$60\%} & \textbf{ASR$\ge$80\%} \\
\midrule
Stealthiest input-space footprint      & BppAttack     & BppAttack     & BppAttack \\
Stealthiest feature-space footprint    & Adap-Patch    & Adap-Patch    & Adap-Patch \\
Stealthiest parameter-space footprint  & Grond         & Grond         & Grond \\
Same attack best in all three spaces?  & No            & No            & No \\
Most balanced attack (min worst space) & Grond ($0.42$) & Grond ($0.45$) & Grond ($0.36$) \\
CDBI top-ranked attack                 & Narcissus     & Narcissus     & Narcissus \\
TUP top-ranked attack                  & Grond         & Narcissus     & Grond \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table}[t]
\centering
\caption{Rank stability under ASR filtering: Kendall's $\tau$ between the attack ordering on
all configurations and after excluding low-ASR ones. Per-space rankings are highly stable; the
composite (overall) ranking is less so, as expected because the three spaces measure different
footprints (\autoref{sec:metric_disagreement}).}
\label{tab:asr_stability}
\begin{tabular}{lcc}
\toprule
\textbf{Space} & \textbf{All vs ASR$\ge$60\%} & \textbf{All vs ASR$\ge$80\%} \\
\midrule
Input     & $+0.96$ & $+0.91$ \\
Feature   & $+0.96$ & $+0.91$ \\
Parameter & $+0.94$ & $+0.76$ \\
\midrule
Overall (composite) & $+0.73$ & $+0.56$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/asr_filter_rank_stability.pdf}
    \caption{Per-space attack rank stability under ASR filtering. Each line is an attack; its
    footprint rank (1 $=$ stealthiest) is recomputed after excluding configurations below the
    ASR threshold. The stealthiest attack in each space (BppAttack, Adap-Patch, Grond) stays at
    rank~1 throughout, and the orderings are largely preserved.}
    \label{fig:asr_rank_stability}
\end{figure*}


==> sections/analyses/analysis5.tex <==
\subsection{Benchmark Artifact and Extensibility}

To make the measurement protocol reusable, we organize the artifact as an extensible benchmark rather than a collection of one-off scripts. The benchmark separates attacks, models, datasets, and metrics through a small set of wrappers. Each attack implementation exports a backdoored model and poisoned train/test data, which are normalized into a common record containing the model, clean and poisoned datasets, poisoned-sample indicators, original labels, target labels, and attack metadata. This wrapper layer allows attacks implemented in different codebases to be evaluated under the same measurement protocol.

Metrics consume standardized artifacts rather than attack-specific internals. Input-space metrics operate on paired clean and poisoned image batches. Feature-space metrics consume saved predictions and penultimate-layer representations extracted from clean and backdoored inputs. Parameter-space metrics consume model parameters and, when needed, saved activation differences. This design allows new metrics to be added without reimplementing attacks, and new attacks to be added by providing only a wrapper that exposes poisoned-data construction, trigger/test-set generation, the trained model, and configuration metadata.

The benchmark output schema records benign accuracy, attack success rate, dataset, architecture, poison rate, target class, random seed, attack configuration, and the measured input-, feature-, and parameter-space footprints. Intermediate artifacts, including extracted features, predictions, activation changes, and poisoned-sample indices, are saved to make the results auditable and reusable. Thus, the artifact supports the goal of the paper: measuring observable backdoor footprints under a shared protocol rather than producing a fixed leaderboard.
Table~\ref{tab:artifact_components} summarizes the artifact components that separate attack execution, model introspection, metric computation, and result aggregation.

\begin{table*}[t]
\centering
\caption{Benchmark artifact components.}
\label{tab:artifact_components}
\begin{tabular}{ll}
\toprule
\textbf{Component} & \textbf{Purpose} \\
\midrule
Attack wrapper & Normalizes trigger generation, poisoned data, and attack metadata \\
Model wrapper & Standardizes prediction, feature extraction, and parameter access \\
Metric API & Computes input-, feature-, and parameter-space footprint values \\
Run schema & Stores BA, ASR, metrics, configurations, and reproducibility metadata \\
Aggregation scripts & Produce benchmark tables and derived analyses from saved runs \\
Extension hooks & Allow new attacks or metrics to be added under the same protocol \\
\bottomrule
\end{tabular}
\end{table*}

==> sections/analyses/analysis6.tex <==


\section{Cross-Architecture Stability}
\label{sec:cross_arch}

We test whether the tri-space picture is specific to ResNet18 by comparing attack rankings
across ResNet18, VGG16, and ViT-Small. Input-space metrics depend only on the trigger, not the
model, so input-space rankings are identical across architectures by construction. For the
feature space, SS and DSWD are available for all three architectures on CIFAR-10 (the $8$
attacks trained on all three; DFST was not trained on VGG/ViT, and DFBA has no feature cluster).
Parameter-space metrics are channel-based and apply only to CNNs; moreover VGG16 models exist
for only three attacks, too few for a meaningful rank correlation, so we report parameter-space
cross-architecture stability as a limitation rather than a coefficient.

\autoref{tab:arch_stability} and \autoref{fig:arch_feature_scatter} show that feature-space
rankings are consistent between the two convolutional networks (combined-feature Kendall
$\tau=0.73$, Spearman $\rho=0.85$ for ResNet--VGG) but only weakly aligned with ViT-Small
(ResNet--ViT $\tau=0.35$, and just $0.07$ for SS alone). Two factors explain the ViT divergence.
First, feature-space stealthiness is a property of the learned representation, which differs
substantially between convolutional and attention-based models. Second, several attacks fail to
implant on ViT-Small (e.g.\ WaNet, BppAttack, and Adap-Patch all have low ASR; cf.\ our
performance table), so their ViT feature footprints reflect failed rather than stealthy attacks,
echoing the low-ASR caution of \autoref{sec:asr_sensitivity}. The qualitative tri-space
conclusion is unaffected: no attack is uniformly stealthy on any architecture, and the spaces
remain non-substitutable; what varies with architecture is the precise feature-space ordering.

Because the paper computes CDBI and TUP only for ResNet18, we recompute them (without retraining)
on the VGG16 models that exist; Grond, Narcissus, and DFBA across three datasets as a
consistency check (\autoref{tab:vgg_newmetrics}). The parameter metric TUP transfers
consistently on CIFAR-10 and Imagenette, where Grond is the stealthiest and DFBA the loudest of
the three attacks on both architectures. On CIFAR-100 the ordering differs: Narcissus is the
TUP-stealthiest on both architectures, while the loudest attack swaps between Grond (VGG16) and
DFBA (ResNet18). DFBA's TUP is markedly smaller on VGG16
than ResNet18 (e.g.\ $0.99$ vs.\ $10.20$ on CIFAR-10), which reflects the single-layer limitation
discussed in \autoref{sec:tup_disagreement}: DFBA's compromised neuron need not lie in the last
convolutional layer that TUP inspects, and its location is architecture-dependent. The feature
metric CDBI is, as expected, more architecture-sensitive: its magnitudes and the
Grond-versus-Narcissus order change across architectures (the two agree on CIFAR-10 but reverse
on CIFAR-100 and Imagenette), mirroring the architecture dependence of SS and DSWD above. We
therefore read CDBI as an architecture-specific feature-space diagnostic rather than an absolute
scale comparable across models. Extending parameter-space metrics to ViT for which no
channel-Lipschitz analogue exists remains future work; a candidate is the spectral norm of the
attention-head projection matrices.





\begin{table}[t]
\centering
\caption{Cross-architecture stability of attack rankings on CIFAR-10 (Kendall's $\tau$ over the
$8$ attacks trained on all three architectures). Input-space rankings are architecture-independent
by construction. Feature-space rankings agree between the two CNNs but only weakly with ViT.
Parameter-space metrics are channel-based and do not transfer to ViT; VGG parameter data exists
for only three attacks, too few for a rank correlation (see text).}
\label{tab:arch_stability}
\begin{tabular}{lccc}
\toprule
\textbf{Space / metric} & \textbf{ResNet--VGG} & \textbf{ResNet--ViT} & \textbf{VGG--ViT} \\
\midrule
Input (by construction) & $1.00$ & $1.00$ & $1.00$ \\
Feature: SS             & $0.57$ & $0.07$ & $0.21$ \\
Feature: DSWD           & $0.64$ & $0.43$ & $0.79$ \\
Feature: combined       & $0.73$ & $0.35$ & $0.54$ \\
Parameter (CNN-only)    & --     & --     & --     \\
\bottomrule
\end{tabular}
\end{table}

\begin{table*}[t]
\centering
\caption{Transfer of the proposed metrics to VGG16: CDBI and TUP recomputed (no retraining) for
the three attacks with available VGG16 models, against ResNet18. CDBI is undefined for the
data-free DFBA. TUP rankings are broadly consistent across architectures (Grond stealthiest,
DFBA loudest on CIFAR-10 and Imagenette), whereas CDBI's values and the Grond--Narcissus order
shift with architecture, consistent with feature-space metrics depending on representation
geometry.}
\label{tab:vgg_newmetrics}
\begin{tabular}{llcccc}
\toprule
\textbf{Dataset} & \textbf{Attack} & \textbf{CDBI (VGG)} & \textbf{CDBI (ResNet)}
& \textbf{TUP (VGG)} & \textbf{TUP (ResNet)} \\
\midrule
CIFAR-10   & Grond     & $1.21$ & $0.87$ & $0.52$  & $1.87$  \\
CIFAR-10   & Narcissus & $0.84$ & $0.77$ & $0.63$  & $2.15$  \\
CIFAR-10   & DFBA      & --     & --     & $0.99$  & $10.20$ \\
\midrule
CIFAR-100  & Grond     & $1.78$ & $1.95$ & $6.20$  & $8.86$  \\
CIFAR-100  & Narcissus & $0.86$ & $3.47$ & $3.73$  & $8.75$  \\
CIFAR-100  & DFBA      & --     & --     & $4.35$  & $10.60$ \\
\midrule
Imagenette & Grond     & $2.83$ & $24.0$ & $1.11$  & $1.61$  \\
Imagenette & Narcissus & $6.68$ & $4.27$ & $1.26$  & $2.64$  \\
Imagenette & DFBA      & --     & --     & $11.35$ & $13.50$ \\
\bottomrule
\end{tabular}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{img/arch_feature_scatter.pdf}
    \caption{Combined feature-space rank of each attack on CIFAR-10: ResNet18 vs.\ VGG16 and
    ViT-Small ($1=$ stealthiest). VGG16 tracks ResNet18 (points near the diagonal), whereas
    ViT-Small diverges, reflecting its different representation geometry and the many attacks
    that fail to implant on ViT.}
    \label{fig:arch_feature_scatter}
\end{figure}

==> sections/background.tex <==
\section{Backdoor Attacks and Stealthiness}
\label{sec:background}

\newcommand{\model}{\ensuremath{f_\theta}}
\newcommand{\backdooredModel}{\ensuremath{\hat{\model}}}

% \subsection{Backdoor Attacks}
% \label{subsec:backdoor}

A backdoor attack is a targeted poisoning attack on a classifier \(\backdooredModel\) that keeps normal behavior on clean inputs but forces the prediction of an attacker-chosen target class \(y_t\) when a specific pattern (the trigger) is present. We consider all-to-one attacks and denote by \(\mathcal{T}(x)\) the operation that inserts the trigger into an image \(x\). Performance is reported on a held-out test set: benign accuracy \(\mathrm{BA}=\tfrac{1}{|D_{\text{test}}|}\sum_{(x,y)\in D_{\text{test}}}\mathbf{1}[\backdooredModel(x)=y]\) and attack success rate \(\mathrm{ASR}=\tfrac{1}{|D_{\text{test}}|}\sum_{(x,\,\cdot)\in D_{\text{test}}}\mathbf{1}[\backdooredModel(\mathcal{T}(x))=y_t]\). The attacker typically poisons a fraction \(\pi\) of training samples by applying \(\mathcal{T}\). In dirty-label attacks, poisoned samples are relabeled to \(y_t\) during training. However, in clean-label attacks~\cite{turner2019cleanlabel,zeng2022narcissus}, labels are unchanged, and poisoning is limited to samples that already have \(y_t\) as their labels. Stronger supply-chain settings let the adversary alter the training process or publish a pre-trained backdoored model. The goal across settings is high ASR with BA close to the clean baseline, making the backdoor effective yet hard to notice in the recognition of benign images.


% \subsection{Backdoor Stealthiness}
% \label{subsec:overview_stealthiness}

Backdoor stealthiness refers to the extent to which a backdoored model resembles a benign one, and it can be examined across the input, feature, and parameter spaces. In the input space, stealthiness is determined by the degree of visual perturbation introduced by the trigger. This can be judged by humans, or more rigorously quantified using metrics such as $l_p$ norms, Mean Squared Error (MSE), and Peak Signal-to-Noise Ratio (PSNR). In the feature space, stealthiness is evaluated by comparing the representations produced by benign and backdoor inputs, where features are defined as the outputs of the penultimate layer of the neural network, i.e., the input to the final classification layer. In the parameter space, stealthiness is assessed through the sensitivity of neurons to the trigger, as the backdoor functionality is typically concentrated in a small subset of neurons that significantly contribute to the malicious behavior.

==> sections/conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusion}

%This work provides a comprehensive analysis of backdoor attack stealthiness across input, feature, and parameter spaces. 
Through systematic evaluation of ten attacks using quantitative metrics, we demonstrate that achieving comprehensive stealthiness remains a non-trivial goal. None of the considered attacks achieves consistent stealthiness across all three spaces simultaneously, but Grond could be considered relatively stealthy in all three domains. Our findings underscore the inherent trade-offs in backdoor design and reveal fundamental limitations in existing attack methodologies.
The evaluation also critically examines current stealthiness metrics, highlighting their strengths and weaknesses in capturing different aspects of backdoor behavior. In response to identified limitations, we propose two novel metrics that offer improved characterization of stealthiness properties. These metrics provide researchers with enhanced tools for developing and evaluating backdoor attacks. We also conduct correlation analysis between backdoor defenses and stealthiness metrics to identify metrics that indicate stealth consistency. From there, we propose a novel tri-space stealthiness metric.
We suggest that future backdoor attacks be evaluated using comprehensive stealthiness metrics across multiple domains. However, our metrics are diagnostic tools that require a reference benign model or access to the trigger pattern, limiting their use in strictly black-box defensive scenarios.
We plan to extend this benchmarking framework to other modalities (e.g., NLP, Audio) and develop new parameter-space metrics specifically tailored for transformer-based architectures (ViT).
Our study assumes a classification task on static images; extending these metrics to multi-modal tasks or generative models remains future work. 
%Regarding our proposed metrics, CDBI relies on dimensionality reduction (t-SNE), which can be sensitive to hyperparameters such as perplexity and random seeds; while we fixed these for reproducibility, future work should explore seed-robust alternatives. Similarly, while TUP improves upon raw parameter analysis, it currently evaluates only the last convolutional layer; future iterations could aggregate sensitivity across all layers. 



==> sections/correlation.tex <==
\section{Metric Validation Methodology: Residual Correlation Analysis}
\label{sec:correlation_methodology}

To empirically validate whether our proposed metrics (and existing baselines) reflect an attack's stealthiness, we quantify the relationship between these metrics and the actual evasion performance against state-of-the-art defenses. A naive correlation analysis, however, would be statistically flawed due to confounding variables, specifically the varying difficulty of datasets and the intrinsic strength of different attacks. For instance, a defense might perform poorly on a specific dataset simply because the dataset is more complex, not because the attack is stealthier. Similarly, an attack might have a low post-defense ASR simply because its initial ASR was low, unrelated to its stealthiness footprint.
To isolate the predictive power of the stealthiness metrics from these biases, we employ a \textit{Partial Correlation} approach using residuals. We detail our three-stage analysis framework below.

\subsection{Data Alignment and Standardization}
First, we align all variables such that a higher value consistently indicates higher \textit{stealthiness}. Let $M$ be the set of stealthiness metrics (e.g., $L_2$, TUP, CDBI) and $D$ be the set of defense outcomes.
For a given metric $m \in M$, if the standard interpretation is ``lower is better/stealthier'' (e.g., $L_2$ norm, TAC, TUP), we invert the sign: $\hat{m} = -m$.
% \begin{equation}
%     \hat{m} = -m.
% \end{equation}
For defense outcomes $d \in D$, we standardize the interpretation to ``Defense Evasion Success''. If a defense reports a Detection F1 score (where higher means detected/failed stealth), we invert it. If a defense reports Post-Defense ASR (where higher means evasion/successful stealth), we keep the raw value:
\begin{equation}
    \hat{d} = 
    \begin{cases} 
    d & \text{if } d \text{ is ASR-based} \\
    -d & \text{if } d \text{ is Detection-based}.
    \end{cases}
\end{equation}
This ensures that for all pairs $(\hat{m}, \hat{d})$, a positive correlation implies that the metric correctly predicts defense evasion.

\subsection{Confounder Removal via Residuals}
\label{sec:correlation:resid}
To remove the influence of experimental biases, we model the dependency of both the metric $\hat{m}$ and the defense outcome $\hat{d}$ on the confounding factors. We define the set of confounders $Z$ to include the Dataset identity (categorical) and the baseline Attack Strength (ASR before defense)  $Z = \{ \text{Dataset}, \text{ASR}_{\text{pre}} \}$.
% \begin{equation}
%     Z = \{ \text{Dataset}, \text{ASR}_{\text{pre}} \}.
% \end{equation}
We deliberately exclude the \textit{Attack Type} from the confounders. Controlling for the attack identity would mathematically remove the variance we aim to study (e.g., the difference in $L_2$ norm between a patch attack and a warping attack).

We fit an Ordinary Least Squares (OLS) regression model to predict the expected values of $\hat{m}$ and $\hat{d}$ given $Z$:
\begin{align}
    \hat{m} &= \beta_m Z + \epsilon_m \\\nonumber
    \hat{d} &= \beta_d Z + \epsilon_d.
\end{align}
where $\beta$ represents the regression coefficients. Conceptually, the residual ($\epsilon$) is the difference between the observed value and the value predicted by the control variables. It represents the ``net'' behavior of the metric or defense that remains after mathematically stripping away the expected influence of dataset difficulty and baseline attack strength. Thus, $\epsilon_m$ and $\epsilon_d$ encapsulate the purified variations attributable to the stealthiness profile itself.

\subsection{Statistical Significance and Correlation}
Finally, we calculate the Spearman's rank correlation coefficient $\rho$ between the residuals $\epsilon_m$ and $\epsilon_d$. We choose Spearman's $\rho$ over Pearson's $r$ to capture monotonic non-linear relationships, as stealthiness metrics often scale differently than defense probabilities (e.g., exponential growth in a metric vs. linear decay in ASR).
The validity score $V$ for a metric-defense pair is given by  $V(m, d) = \text{Spearman}(\epsilon_m, \epsilon_d)$.
% \begin{equation}
%     V(m, d) = \text{Spearman}(\epsilon_m, \epsilon_d).
% \end{equation}

\subsubsection{Significance Testing (P-values)}
Given the finite sample size of our aggregated dataset, observed correlations could potentially arise from stochastic noise rather than a true underlying relationship. To mitigate this risk, we perform hypothesis testing for each correlation coefficient.
We test the null hypothesis $H_0: \rho = 0$ (implying no monotonic association between the metric and defense evasion) against the alternative hypothesis $H_1: \rho \neq 0$.

The \textbf{$p$-value} represents the probability of observing a correlation coefficient as extreme as the one calculated, assuming the null hypothesis is true. A low $p$-value indicates that it is highly unlikely for such a relationship to appear by random chance. We enforce a significance threshold of $\alpha = 0.05$. In our visualization (the heatmap), we mark any result where $p < 0.05$ as statistically significant.

\subsection{Data Aggregation and DataFrame Construction}
\label{subsec:dataframe_construction}

%To facilitate the residual correlation analysis, 
We consolidated our experimental results into a unified structured dataset (DataFrame). This dataset aggregates the performance of 9 backdoor attacks against 10 state-of-the-art defenses across 2 benchmark datasets, capturing variations in poisoning rates. %The construction and role of each component are detailed below:

\subsubsection{Data Composition}
The DataFrame consists of $N$ observations, with rows representing unique (Attack, Dataset, Poisoning Rate) settings.
\begin{compactitem}
    \item \textbf{Attacks ($A$):} We included 9 attacks (discussed in Appendix~\ref{sec:methodology:train_settings:backdoor_specific}).
    %covering diverse triggers and strategies: \textit{BadNets, Blended, WaNet, BppAttack, Adaptive-Patch, Adaptive-Blend, DFST, Narcissus,} and \textit{Grond}. 
    These attacks provide the primary variation in stealthiness metrics (the independent variables).
    
    \item \textbf{Defenses ($D$):} We evaluated 10 defenses to serve as the ground-truth outcomes (the dependent variables):
    \begin{compactitem}
        \item \textit{Detection-based:} SPECTRE, STRIP, Spectral Signatures (SS), BTI-DBF, BAN.
        \item \textit{Mitigation/Restoration-based:} CLP, I-BAU, FeatureRE, Neural Cleanse (NC), TABOR.
    \end{compactitem}
    
    \item \textbf{Datasets ($S$):} The analysis spans \textit{CIFAR-10} and \textit{Imagenette}. Including multiple datasets is critical for statistical power and allows us to control for dataset-specific difficulty (e.g., higher image resolution in Imagenette may naturally inflate $L_2$ norms compared to CIFAR-10).
    
    \item \textbf{Poisoning Rates ($P$):} For each attack-dataset pair, we included results for two distinct poisoning regimes: a \textit{High} rate (typically 5\%) and a \textit{Low} rate (typically 0.3\%, or 2\% for specific attacks like WaNet/BppAttack where 0.3\% is ineffective). This variation is essential as it creates a spread in both the metric footprints (e.g., high vs. low visual distortion) and the defense evasion success.
\end{compactitem}

\subsubsection{Role of Variables in Residual Analysis}
In the context of the formula defined in Section~\ref{sec:correlation:resid}, these data components play distinct roles:
\begin{compactitem}
    \item \textbf{Attacks ($A$):} The attack identity is \textit{not} explicitly modeled as a variable in the regression formula. Instead, the attacks act as the generators of variance in the stealthiness metrics (e.g., WaNet generates low $L_2$ values, Patch attacks generate high $L_2$). We correlate these metric values directly, rather than the attack labels, to determine which specific features drive evasion.
    
    \item \textbf{Datasets ($S$):} This serves as a \textbf{categorical confounder} in the control set $Z$. By including `C(Dataset)` in the regression model, we mathematically remove the baseline differences in metric magnitudes and defense performance attributable solely to the image domain (e.g., ``Imagenette is harder to defend than CIFAR-10''), isolating the effect of the attack's stealthiness.
    
    \item \textbf{Poisoning Rates ($P$):} This factor drives the \textbf{Attack Strength Confounder} ($\text{ASR}_{\text{pre}}$). A high poisoning rate typically yields a stronger attack (high $\text{ASR}_{\text{pre}}$) but a louder footprint. By controlling for $\text{ASR}_{\text{pre}}$ in $Z$, we ensure that a metric is not deemed ``predictive'' simply because it correlates with the raw strength of the attack; it must predict evasion \textit{beyond} what is expected from a strong attack.
\end{compactitem}



\subsection{Interpreting the Matrix: The ``Stealth-Consistency'' Sign}
\label{subsec:interpreting_matrix}

The resulting residual correlation matrix in Figure~\ref{fig:residual_correlations} provides a standardized view of metric validity. Because we have aligned all inputs (metrics) and outputs (defenses) to the same semantic direction, where a higher value denotes greater stealth, the interpretation of the correlation coefficient $\rho$ is uniform across the entire matrix. Detailed results are in Appendix~\ref{sec:defense_results}.

\begin{compactitem}
    \item \textbf{Positive Correlation ($\rho > 0$, Red cells):} This indicates \textit{Stealth Consistency}. It means that when the metric claims an attack is stealthy, the defense confirms it by failing to detect the attack. A high positive value validates the metric as a reliable predictor of real-world evasion for that specific defense.
    
    \item \textbf{Negative Correlation ($\rho < 0$, Blue cells):} This indicates a \textit{Stealth Trade-off} or \textit{Inverse Relationship}. It implies that optimizing for this specific metric (making the attack ``stealthier'' in the metric's view) actually makes the attack \textit{easier} for the defense to detect. This often highlights a ``loud footprint'' where minimizing one trace (e.g., input noise) inadvertently amplifies another (e.g., feature distortion).
    
    \item \textbf{Near-Zero Correlation ($\rho \approx 0$, White cells):} This indicates \textit{Orthogonality}. The defense is effectively ``blind'' to the feature measured by the metric; variations in the metric score have no statistical bearing on whether the defense succeeds or fails.
\end{compactitem}

% We first consider the intersection between the input-space metrics (first 11 columns) and the defense \textbf{Neural Cleanse (NC)}. For most metrics, we observe a statistically significant result of $\rho < 0$, which implies a trade-off; attacks that strive for extreme imperceptibility result in a lower reversed norm, making them \textit{easier} for Neural Cleanse to detect. 

% For the feature-space metrics (\textbf{SS}, \textbf{DSWD}, and \textbf{CDBI}), the most significant correlation is observed between SS and the \textbf{SPECTRE defense}. This indicates that the silhouette score can reliably predict whether a backdoor attack would be detected by this defense.

% Finally, among the parameter-space metrics (\textbf{UCLC}, \textbf{TAC}, and \textbf{TUP}), we observe a relatively low correlation between UCLC and the \textbf{CLP} defense. This is surprising, since CLP prunes neurons based on their UCLC. However, it could be explained by the fact that benign neurons may also have high UCLC. Therefore, the UCLC score of an attack may be high even though CLP does not substantially decrease its ASR, resulting in a low correlation. We have designed the TUP metric to decrease the influence of these benign neurons on the stealthiness score. Judging from the correlation results, the metric seems to be effective, as its correlation with CLP is the highest among all defenses and metrics.

%\todo{yes, this text is strange. We have some basic discussion in next section so I would remove this text}

% \textbf{Example Interpretation:}
% Consider the intersection between the metric \textbf{LPIPS} and the defense \textbf{Neural Cleanse (NC)}. 
% Recall that we inverted LPIPS (so higher values mean lower perceptual error/higher stealth) and used the raw NC Reversed Norm (where higher values mean the defense failed to reverse a small trigger/higher stealth). The result of $\rho < 0$ implies a trade-off. Attacks that strive for extreme invisibility (low LPIPS) result in a lower reversed norm, making them \textit{easier} for Neural Cleanse to detect. As such, the ``stealthiness'' metric (LPIPS) is actually a predictor of vulnerability.
% \begin{compactitem}
%     \item If the cell is \textbf{red} ($\rho > 0$): It implies that attacks with lower perceptual error (invisible triggers) are also harder for Neural Cleanse to reverse. The metric accurately predicts evasion.
%     \item If the cell is \textbf{blue} ($\rho < 0$): It implies a trade-off. Attacks that strive for extreme invisibility (low LPIPS) result in a lower reversed norm, making them \textit{easier} for Neural Cleanse to detect. In this case, the ``stealthiness'' metric (LPIPS) is actually a predictor of vulnerability.
% \end{compactitem}

\begin{figure*}[!htbp]
\centering
\includegraphics[width = 0.9\linewidth]{img/residuals_heatmap_all.png}
\caption{Residual correlation matrix between various stealthiness metrics and defenses.}
\label{fig:residual_correlations}
\end{figure*}

==> sections/defense_metric_correlations.tex <==
\section{Backdoor Defense Results}
\label{sec:defense_results}

In Tables~\ref{tab:ban_fixed} to~\ref{tab:f1_imagenette_attacks}, we report the results of the backdoor defense experiments performed for the correlation analysis in Section~\ref{sec:correlation_methodology}.

% To further investigate the practical implications of stealthiness metrics, we analyze their correlation with the performance of three representative defense mechanisms covering the input, feature, and parameter spaces. This analysis aims to determine whether the proposed metrics serve as reliable indicators of an attack's vulnerability to detection or mitigation.

% \subsection{Experimental Setup}
% We selected the following defenses for evaluation on the CIFAR-10 dataset:
% \begin{enumerate}
%     \item \textbf{Neural Cleanse (NC)~\cite{wang2019nc} (Input Space):} A trigger synthesis defense. We measure the $L_1$ norm of the reversed trigger. A \textit{lower} reversed trigger norm indicates a higher confidence that a backdoor exists (less stealthy).
%     \item \textbf{BTI-DBF~\cite{xu2024towards} (Feature Space):} A variation of activation clustering. We measure the number of \textit{detected} (removed) poisoned samples. A \textit{higher} number indicates effective detection (less stealthy).
%     \item \textbf{Channel Lipschitz-based Pruning (CLP)~\cite{zheng2022clp} (Parameter Space):} A pruning defense. We measure the \textit{Attack Success Rate (ASR)} after pruning. A \textit{lower} post-defense ASR indicates effective mitigation (less stealthy).
% \end{enumerate}

% We calculated the Pearson correlation coefficient ($r$) between our stealthiness metrics and the defense outcomes across our evaluated attacks at both high ($5\%$) and low ($0.3\%$, except $2\%$ for WaNet and BppAttack) poisoning rates (PR). DFBA does not fit this methodology since it does not have a poisoning rate. Therefore, its defense outcomes are not considered when calculating the correlation.

% \subsection{Results and Analysis}
% The raw performance of the defenses against the evaluated attacks is presented in Table~\ref{tab:defense_results}, and the Pearson correlation coefficients are detailed in Table~\ref{tab:pearson_results}.

% \textbf{Parameter Space Alignment (CLP).}
% We observe a strong negative correlation between parameter-space metrics and the ASR of the model after CLP defense. Specifically, \textbf{TAC} shows a correlation of $r=-0.6598$ and \textbf{UCLC} shows $r=-0.5719$ (at PR 5\%).
% \textit{Interpretation:} Since a high TAC/UCLC value indicates low stealthiness (high sensitivity), and a low post-defense ASR indicates a successful defense, a negative correlation confirms that attacks with high channel sensitivity are significantly more vulnerable to pruning. This validates that TAC and UCLC are strong predictors of parameter-space defense efficacy.

% \textbf{Input Space and Trigger Reversal (NC).}
% For Neural Cleanse, the $l_\infty$ norm exhibits a strong negative correlation ($r=-0.7136$ at PR 0.3\%).
% \textit{Interpretation:} NC successfully reverses a trigger (resulting in a small norm) when the attack has a distinct, non-stealthy footprint. Attacks with high $l_\infty$ perturbations allow NC to converge on a smaller, more obvious trigger pattern, hence the negative correlation. Interestingly, feature space metrics like DSWD also show a negative correlation ($r=-0.6606$ at PR 5\%), suggesting that attacks with poor feature stealthiness are easier for input-space scanners to reverse-engineer.

% \textbf{Feature Space Detection (BTI-DBF).}
% For BTI-DBF, we observe a strong positive correlation with the $l_\infty$ norm ($r=0.7497$ at PR 5\%).
% \textit{Interpretation:} This indicates that attacks with high pixel-level intensity (like BadNets) are easily clustered and removed by BTI-DBF. Conversely, we noted a negative correlation between BTI-DBF detection and DSWD ($r=-0.3585$). This counter-intuitive result highlights a divergence in "stealthiness" definitions: BTI-DBF effectively caught BadNets (which has low DSWD/high stealthiness in feature space but high $l_\infty$), but missed Grond (which has high DSWD but low $l_\infty$). This suggests that BTI-DBF's clustering capability on this dataset was driven more by artifacts stemming from input-space perturbations than by the distributional shifts measured by DSWD.



\begin{table*}[htbp]
    \centering
    \scriptsize
    \caption{Defense Performance Overview on CIFAR-10. The efficacy of three defenses against the evaluated attacks. For NC, a lower reversed norm implies detection. For CLP, lower ASR implies mitigation. For BTI-DBF, higher detected samples imply detection.}
    \label{tab:defense_results_cifar10}
    \begin{tabular}{l *{2}{c} *{2}{c} *{2}{c}}
    \toprule
    & \multicolumn{2}{c}{\textbf{Neural Cleanse (Input)}} & \multicolumn{2}{c}{\textbf{CLP (Parameter)}} & \multicolumn{2}{c}{\textbf{BTI-DBF (Feature)}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    \textbf{Attack} & \textbf{Rev. Norm (5\%)} & \textbf{Rev. Norm (0.3\%)} & \textbf{ASR (5\%)} & \textbf{ASR (0.3\%)} & \textbf{Detected (5\%)} & \textbf{Detected (0.3\%)} \\
    \midrule
    Badnet      & 136.8 & 118.3 & 11.36 & 99.72 & 2499 & 0 \\
    Blended     & 214.4 & 305.5 & 95.87 & 90.68 & 0    & 1101 \\
    Wanet       & 222.0 & 323.2 & 24.72 & 0.76  & 46   & 0 \\
    Bpp         & 253.0 & 375.6 & 0.70  & 0.63  & 0    & 0 \\
    Adap-P      & 299.2 & 170.8 & 11.43 & 37.54 & 1969 & 0 \\
    Adap-B      & 255.8 & 299.5 & 54.32 & 44.00 & 0    & 577 \\
    DFST        & 246.3 & 292.2 & 39.11 & 79.02 & 0    & 0 \\
    Narcis.     & 181.4 & 239.4 & 99.92 & 92.13 & 0    & 2500 \\
    Grond       & 226.0 & 282.3 & 92.64 & 72.55 & 0    & 1813 \\
    DFBA        & \multicolumn{2}{c}{289.9} & \multicolumn{2}{c}{10.05} & \multicolumn{2}{c}{649} \\
    \bottomrule
    \end{tabular}
\end{table*}



\begin{table*}[htbp]
    \centering
    \scriptsize
    \caption{Defense Performance Overview on Imagenette. Efficacy of three defenses against the evaluated attacks. For NC, values reflect the reversed norm of Target Class 0. For CLP, lower ASR implies mitigation. For BTI-DBF, higher detected samples imply detection.}
    \label{tab:defense_results_imagenette}
    \begin{tabular}{l *{2}{c} *{2}{c} *{2}{c}}
    \toprule
    & \multicolumn{2}{c}{\textbf{Neural Cleanse (Input)}} & \multicolumn{2}{c}{\textbf{CLP (Parameter)}} & \multicolumn{2}{c}{\textbf{BTI-DBF (Feature)}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    \textbf{Attack} & \textbf{Rev. Norm (5\%)} & \textbf{Rev. Norm (0.3\%)} & \textbf{ASR (5\%)} & \textbf{ASR (0.3\%)} & \textbf{Detected (5\%)} & \textbf{Detected (0.3\%)} \\
    \midrule
    Badnet      & 230.83 & 453.18 & 47.23 & 0.53 & 0.0 & 0.0 \\
    Blended     & 627.69 & 848.25 & 98.93 & 76.17 & 9129.0 & 0.0 \\
    Wanet       & 857.01 & 773.29 & 69.19 & 87.45 & 0.0 & 0.0 \\
    Bpp         & 190.39 & 713.54 & 1.92 & 1.02 & 0.0 & 32.0 \\
    Adap-P      & 372.33 & 1020.85 & 33.04 & 10.24 & 0.0 & 38.0 \\
    Adap-B      & 672.30 & 888.59 & 95.41 & 72.07 & 0.0 & 0.0 \\
    DFST        & 819.28 & 814.91 & 98.42 & 98.21 & 245.0 & 196.0 \\
    Narcis.     & 932.27 & 878.91 & 83.38 & 45.92 & 0.0 & 0.0 \\
    Grond       & 552.04 & 1105.30 & 52.48 & 2.01 & 0.0 & 0.0 \\
    DFBA        & \multicolumn{2}{c}{652.58} & \multicolumn{2}{c}{11.79} & \multicolumn{2}{c}{0.0} \\
    \bottomrule
    \end{tabular}
\end{table*}


\begin{table}[htbp]
\centering
\scriptsize
\caption{BAN Performance (Target Number).  Values represent the detected target number; higher values indicate more effective detection.}
\label{tab:ban_fixed}
\setlength{\tabcolsep}{5pt} 
\begin{tabular}{l *{4}{c}}
\toprule
Attack & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
(PR) & 5\% & 0.3\% & 5\% & 0.3\% \\
\midrule
Badnet  & 5000 & 451 & 288 & 50 \\
Blended & 914  & 531 & 104 & 27 \\
Wanet   & 4721 & 5000 & 941 & 209 \\
Bpp     & 1884 & 5000 & 715 & 0 \\
Adap-P  & 5000 & 765 & 947 & 596 \\
Adap-B  & 1313 & 946 & 947 & 7 \\
DFST    & 5000 & 468 & 947 & 0 \\
Narcis. & 448  & 417 & 0 & 116 \\
Grond   & 538  & 586 & 45 & 79 \\
DFBA    & \multicolumn{2}{c}{818} & \multicolumn{2}{c}{947} \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[htbp]
\centering
\scriptsize
\caption{TABOR Performance (Rev. Norm). For TABOR, lower values typically indicate potential trigger detection in the input space.}
\label{tab:tabor_results}
\setlength{\tabcolsep}{4.5pt} 
\begin{tabular}{l *{4}{c}}
\toprule
Attack & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
(PR) & 5\% & 0.3\% & 5\% & 0.3\% \\
\midrule
Badnet  & 194.86 & 175.40 & 234.71 & 463.87 \\
Blended & 251.00 & 350.76 & 638.59 & 857.80 \\
Wanet   & 241.89 & 358.66 & 861.03 & 777.16 \\
Bpp     & 283.23 & 319.90 & 198.39 & 721.79 \\
Adap-P  & 339.43 & 213.35 & 376.74 & 1030.89 \\
Adap-B  & 292.93 & 329.12 & 683.30 & 903.25 \\
DFST    & 324.40 & 376.97 & 830.71 & 823.22 \\
Narcis. & 208.73 & 284.75 & 943.41 & 888.09 \\
Grond   & 253.89 & 325.57 & 561.01 & 1118.90 \\
DFBA    & \multicolumn{2}{c}{330.81} & \multicolumn{2}{c}{662.63} \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htbp]
\centering
\scriptsize 
\caption{FeatureRE Performance (ASR \%).}
\label{tab:featurere_fixed}
\setlength{\tabcolsep}{5pt} 
\begin{tabular}{l *{4}{c}}
\toprule
Attack & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
(PR) & 5\% & 0.3\% & 5\% & 0.3\% \\
\midrule
Badnet  & 7.77  & 34.44 & 93.83 & 81.48 \\
Blended & 14.44 & 11.11 & 75.31 & 38.27 \\
Wanet   & 97.78 & 56.67 & 100.0 & 30.86 \\
Bpp     & 23.33 & 41.11 & 100.0 & 81.48 \\
Adap-P  & 65.56 & 87.78 & 77.78 & 64.20 \\
Adap-B  & 93.33 & 95.56 & 82.72 & 55.56 \\
DFST    & 57.78 & 75.56 & 90.12 & 50.62 \\
Narcis. & 53.33 & 11.11 & 44.44 & 69.14 \\
Grond   & 12.22 & 4.44  & 45.68 & 64.20 \\
DFBA    & \multicolumn{2}{c}{17.78} & \multicolumn{2}{c}{76.54} \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[h!]
%     \centering
%     \caption{\textbf{Correlation Analysis.} Pearson correlation coefficients ($r$) between stealthiness metrics and defense outcomes. \textbf{Note:} For NC and CLP, a \textit{negative} correlation implies the metric correctly predicts defense success (e.g., High TAC $\rightarrow$ Low ASR). For BTI-DBF, a \textit{positive} correlation implies prediction of detection (e.g., High $l_\infty$ $\rightarrow$ High Detection).}
%     \label{tab:pearson_results}
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l|cc|cc|cc}
%     \toprule
%     & \multicolumn{2}{c|}{\textbf{Neural Cleanse}} & \multicolumn{2}{c|}{\textbf{CLP}} & \multicolumn{2}{c}{\textbf{BTI-DBF}} \\
%     \textbf{Metric} & \textbf{PR=5\%} & \textbf{PR=0.3\%} & \textbf{PR=5\%} & \textbf{PR=0.3\%} & \textbf{PR=5\%} & \textbf{PR=0.3\%} \\
%     \midrule
%     \multicolumn{7}{l}{\textit{Input Space Metrics}} \\
%     $l_1$       & 0.0394  & 0.2134  & 0.3626  & 0.4439  & -0.4245 & 0.1234 \\
%     $l_2$       & -0.0083 & -0.0098 & 0.1809  & 0.5026  & -0.1626 & -0.0731 \\
%     $l_\infty$  & -0.4204 & \textbf{-0.7136} & -0.4309 & 0.4392  & \textbf{0.7497}  & -0.5035 \\
%     \midrule
%     \multicolumn{7}{l}{\textit{Feature Space Metrics}} \\
%     SS          & -0.6085 & 0.0896  & 0.1380  & 0.4056  & -0.1345 & 0.1764 \\
%     DSWD        & \textbf{-0.6606} & 0.2219  & 0.3225  & 0.4134  & -0.3585 & 0.2989 \\
%     \midrule
%     \multicolumn{7}{l}{\textit{Parameter Space Metrics}} \\
%     UCLC        & 0.3932  & -0.1646 & \textbf{-0.5719} & -0.3834 & 0.3995  & -0.3897 \\
%     TAC         & 0.1712  & 0.2804  & \textbf{-0.5259} & \textbf{-0.6598} & -0.0894 & -0.3918 \\
%     \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[htbp]
\centering
\scriptsize % Use scriptsize to ensure 9 columns fit a standard USENIX column
\caption{I-BAU ASR Results (ResNet18)}
\label{tab:ibau_asr_fixed}
\setlength{\tabcolsep}{1.8pt} % Very tight spacing to prevent column overflow
\begin{tabular}{l *{8}{c}} % Ensures perfect alignment for all data columns
\toprule
Attack & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{Imagenette} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
 (PR) & \multicolumn{2}{c}{.05} & \multicolumn{2}{c}{.003} & \multicolumn{2}{c}{.05} & \multicolumn{2}{c}{.003} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 (B/A) & Bef. & Aft. & Bef. & Aft. & Bef. & Aft. & Bef. & Aft. \\
\midrule
Adap-B  & .232 & .083 & .045 & .056 & .875 & .029 & .525 & .019 \\
Adap-P  & .108 & .112 & .883 & .080 & .670 & .021 & .017 & .001 \\
Badnet  & 1.00 & .346 & 1.00 & .028 & 1.00 & .000 & .867 & .000 \\
Blended & .998 & .333 & .948 & .000 & .989 & .000 & .735 & .001 \\
Bpp     & .998 & .334 & .005 & .340 & .736 & .001 & .010 & .000 \\
Dfst    & .654 & .233 & .324 & .058 & .324 & .008 & .457 & .010 \\
Grond   & .425 & .033 & .201 & .168 & .009 & .011 & .005 & .016 \\
Narcis. & 1.00 & .145 & .989 & .000 & .861 & .000 & .136 & .000 \\
Wanet   & .985 & .327 & .203 & .338 & .972 & .000 & .610 & .000 \\
\bottomrule
\addlinespace[2pt]
\multicolumn{9}{l}{\textit{Bef.: Before Defense, Aft.: After Defense (ASR)}} \\
\end{tabular}
\end{table}




% \begin{table}[htbp]
% \centering
% \scriptsize % Reduced font size to fit USENIX column
% \caption{F1 Scores for CIFAR-100 (ResNet18, PR: 0.05)}
% \label{tab:f1_cifar100}
% \setlength{\tabcolsep}{4pt} % Tighten horizontal space
% \begin{tabular}{l cccc}
% \toprule
% Attack & AC & SPEC & STRIP & SS \\
% \midrule
% Adap-B & \textcolor{red}{.000} & .000 & .578 & \textcolor{green}{.088} \\
% Adap-P & \textcolor{red}{.000} & .000 & .474 & .061 \\
% Badnet & \textcolor{red}{.000} & .000 & \textcolor{green}{.995} & \textcolor{red}{.000} \\
% Blended & \textcolor{red}{.000} & .000 & .994 & .004 \\
% Bpp     & \textcolor{green}{.001} & .000 & .819 & \textcolor{red}{.000} \\
% Dfst    & \textcolor{red}{.000} & .000 & \textcolor{red}{.036} & .051 \\
% Grond   & \textcolor{red}{.000} & .000 & .171 & .019 \\
% Narcis. & N/A & N/A & N/A & N/A \\
% Wanet   & \textcolor{red}{.000} & .000 & .989 & \textcolor{green}{.088} \\
% \bottomrule
% \addlinespace[2pt]
% \multicolumn{5}{l}{\textit{AC: ActivationClustering, SPEC: SPECTRE, SS: SpectralSignatures}} \\
% \end{tabular}
% \end{table}



\begin{table}[htbp]
\centering
\scriptsize 
\caption{F1 Scores for CIFAR-10 (ResNet18).}
\label{tab:f1_cifar10_attacks_updated}
\setlength{\tabcolsep}{6pt} % Increased spacing for better readability
\begin{tabular}{l cc cc cc}
\toprule
Attack & \multicolumn{2}{c}{SPECTRE} & \multicolumn{2}{c}{STRIP} & \multicolumn{2}{c}{Spectral Signatures} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
(PR) & .05 & .003 & .05 & .003 & .05 & .003 \\
\midrule
Adap-B             & .056 & .006 & .016 & .018 & .010 & .000 \\
Adap-P             & .081 & .006 & .107 & .723 & .052 & .001 \\
BadNet             & .120 & .008 & .995 & .995 & .217 & .038 \\
Blended            & .053 & .006 & .993 & .970 & .000 & .011 \\
Bpp                & .117 & .007 & .878 & .903 & .110 & .001 \\
DFST               & .067 & .006 & .000 & .000 & .001 & .000 \\
Grond              & .089 & .006 & .061 & .073 & .099 & .010 \\
Narcissus          & .080 & .006 & .995 & .963 & .000 & .006 \\
Wanet              & .089 & .007 & .943 & .807 & .001 & .001 \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[htbp]
\centering
\scriptsize 
\caption{F1 Scores for Imagenette (ResNet18).}
\label{tab:f1_imagenette_attacks}
\setlength{\tabcolsep}{6pt} % Increased spacing now that we have more room
\begin{tabular}{l cc cc cc}
\toprule
Attack & \multicolumn{2}{c}{SPECTRE} & \multicolumn{2}{c}{STRIP} & \multicolumn{2}{c}{Spectral Signatures} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
(PR) & .05 & .003 & .05 & .003 & .05 & .003 \\
\midrule
Adap-B    & .063 & .006 & .188 & .030 & .022 & .000 \\
Adap-P    & .078 & .005 & .697 & .127 & .017 & .000 \\
Badnet    & .116 & .008 & .978 & .960 & .220 & .039 \\
Blended   & .054 & .005 & .977 & .857 & .158 & .033 \\
Bpp       & .096 & .010 & .793 & .825 & .202 & .001 \\
Dfst      & .051 & .006 & .007 & .055 & .000 & .000 \\
Grond     & .093 & .006 & .244 & .216 & .074 & .007 \\
Narcissus & .088 & .006 & .877 & .423 & .054 & .006 \\
Wanet     & .071 & .008 & .933 & .893 & .061 & .000 \\
\bottomrule
\end{tabular}
\end{table}

==> sections/defense_metric_correlations_new.tex <==
\section{Supplementary Defense Outcomes}
\label{app:defense_results}

Tables~\ref{tab:defense_overview_merged}--\ref{tab:f1_merged} report the complete defense outcomes underlying the summaries in Sections~\ref{sec:defense_external_checks} and~\ref{sec:defense_association}. The tables cover both mitigation and detection defenses across the evaluated attacks and datasets. For mitigation defenses, we report post-defense attack success rate (ASR), with lower values indicating that the defense more effectively suppresses the backdoor while preserving benign behavior. For detection defenses, we report F1 score, with higher values indicating more reliable discrimination between benign and backdoored samples or models. For BTI-DBF, the reported counts are the numbers of training samples flagged as poisoned; these counts include false positives and can therefore exceed the number of actually poisoned samples.

These outcomes are used as auxiliary external checks on the footprint measurements. In particular, they allow us to examine whether attacks with smaller measured footprints are also harder for defenses with related mechanisms to mitigate or detect. The comparison is intentionally mechanism-specific: input-oriented defenses are expected to align more closely with input-space footprints, representation-based detectors with feature-space footprints, and pruning or repair methods with parameter-space footprints. We therefore do not treat defense success or failure as a definition of stealthiness. A defense may fail because it inspects the wrong space, uses an unsuitable threshold, or does not exploit a footprint that is nevertheless measurable. Conversely, successful defense does not imply that an attack is globally conspicuous. The full tables are provided to make the residual association analysis auditable and to show the heterogeneity of defense outcomes across attacks and datasets.

\begin{table*}[htbp]
    \centering
    \scriptsize
    \caption{Defense performance overview. For NC, a lower reversed norm implies detection (values reflect target class 0). For CLP, lower ASR implies mitigation. For BTI-DBF, higher detected samples imply detection.}
    \label{tab:defense_overview_merged}
    \begin{tabular}{ll *{2}{c} *{2}{c} *{2}{c}}
    \toprule
    & & \multicolumn{2}{c}{\textbf{Neural Cleanse (Input)}} & \multicolumn{2}{c}{\textbf{CLP (Parameter)}} & \multicolumn{2}{c}{\textbf{BTI-DBF (Feature)}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    \textbf{Dataset} & \textbf{Attack} & \textbf{Rev. Norm (5\%)} & \textbf{Rev. Norm (0.3\%)} & \textbf{ASR (5\%)} & \textbf{ASR (0.3\%)} & \textbf{Detected (5\%)} & \textbf{Detected (0.3\%)} \\
    \midrule
    \multirow{10}{*}{CIFAR-10} 
    & Badnet      & 136.8 & 118.3 & 11.36 & 99.72 & 2499 & 0 \\
    & Blended     & 214.4 & 305.5 & 95.87 & 90.68 & 0    & 1101 \\
    & Wanet       & 222.0 & 323.2 & 24.72 & 0.76  & 46   & 0 \\
    & Bpp         & 253.0 & 375.6 & 0.70  & 0.63  & 0    & 0 \\
    & Adap-P      & 299.2 & 170.8 & 11.43 & 37.54 & 1969 & 0 \\
    & Adap-B      & 255.8 & 299.5 & 54.32 & 44.00 & 0    & 577 \\
    & DFST        & 246.3 & 292.2 & 39.11 & 79.02 & 0    & 0 \\
    & Narcis.     & 181.4 & 239.4 & 99.92 & 92.13 & 0    & 2500 \\
    & Grond       & 226.0 & 282.3 & 92.64 & 72.55 & 0    & 1813 \\
    & DFBA        & \multicolumn{2}{c}{289.9} & \multicolumn{2}{c}{10.05} & \multicolumn{2}{c}{649} \\
    \midrule
    \multirow{10}{*}{Imagenette}
    & Badnet      & 230.83 & 453.18 & 47.23 & 0.53 & 0.0 & 0.0 \\
    & Blended     & 627.69 & 848.25 & 98.93 & 76.17 & 9129.0 & 0.0 \\
    & Wanet       & 857.01 & 773.29 & 69.19 & 87.45 & 0.0 & 0.0 \\
    & Bpp         & 190.39 & 713.54 & 1.92  & 1.02  & 0.0 & 32.0 \\
    & Adap-P      & 372.33 & 1020.85& 33.04 & 10.24 & 0.0 & 38.0 \\
    & Adap-B      & 672.30 & 888.59 & 95.41 & 72.07 & 0.0 & 0.0 \\
    & DFST        & 819.28 & 814.91 & 98.42 & 98.21 & 245.0 & 196.0 \\
    & Narcis.     & 932.27 & 878.91 & 83.38 & 45.92 & 0.0 & 0.0 \\
    & Grond       & 552.04 & 1105.30& 52.48 & 2.01  & 0.0 & 0.0 \\
    & DFBA        & \multicolumn{2}{c}{652.58} & \multicolumn{2}{c}{11.79} & \multicolumn{2}{c}{0.0} \\
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[htbp]
    \centering
    \scriptsize
    \caption{Performance of BAN (Detected Targets), TABOR (Rev. Norm), and FeatureRE (ASR \%). Columns are standardized to PR 5\% and 0.3\% for consistency.}
    \label{tab:misc_defenses_merged}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l cccc cccc cccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{BAN (Detected)}} & \multicolumn{4}{c}{\textbf{TABOR (Rev. Norm)}} & \multicolumn{4}{c}{\textbf{FeatureRE (ASR \%)}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{Imagenette} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
    \textbf{Attack} & \textbf{5\%} & \textbf{0.3\%} & \textbf{5\%} & \textbf{0.3\%} & \textbf{5\%} & \textbf{0.3\%} & \textbf{5\%} & \textbf{0.3\%} & \textbf{5\%} & \textbf{0.3\%} & \textbf{5\%} & \textbf{0.3\%} \\
    \midrule
    Badnet  & 5000 & 451 & 288 & 50 & 175.40 & 194.86 & 234.71 & 463.87 & 7.77  & 34.44 & 81.48 & 93.83 \\
    Blended & 914  & 531 & 104 & 27 & 350.76 & 251.00 & 638.59 & 857.80 & 14.44 & 11.11 & 38.27 & 75.31 \\
    Wanet   & 4721 & 5000& 941 & 209& 358.66 & 241.89 & 861.03 & 777.16 & 97.78 & 56.67 & 30.86 & 100.0 \\
    Bpp     & 1884 & 5000& 715 & 0  & 319.90 & 283.23 & 198.39 & 721.79 & 23.33 & 41.11 & 81.48 & 100.0 \\
    Adap-P  & 5000 & 765 & 947 & 596& 339.43 & 213.35 & 376.74 & 1030.89& 65.56 & 87.78 & 64.20 & 77.78 \\
    Adap-B  & 1313 & 946 & 947 & 7  & 329.12 & 292.93 & 683.30 & 903.25 & 93.33 & 95.56 & 55.56 & 82.72 \\
    DFST    & 5000 & 468 & 947 & 0  & 376.97 & 324.40 & 830.71 & 823.22 & 57.78 & 75.56 & 50.62 & 90.12 \\
    Narcis. & 448  & 417 & 0   & 116& 284.75 & 208.73 & 943.41 & 888.09 & 53.33 & 11.11 & 44.44 & 69.14 \\
    Grond   & 538  & 586 & 45  & 79 & 325.57 & 253.89 & 561.01 & 1118.90& 12.22 & 4.44  & 64.20 & 45.68 \\
    DFBA    & \multicolumn{2}{c}{818} & \multicolumn{2}{c}{947} & \multicolumn{2}{c}{330.81} & \multicolumn{2}{c}{662.63} & \multicolumn{2}{c}{17.78} & \multicolumn{2}{c}{76.54} \\
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table}[htbp]
    \centering
    \scriptsize 
    \caption{I-BAU ASR Results (ResNet18)}
    \label{tab:ibau_asr_fixed}
    \setlength{\tabcolsep}{1.8pt} 
    \begin{tabular}{l *{8}{c}} 
    \toprule
    Attack & \multicolumn{4}{c}{CIFAR-10} & \multicolumn{4}{c}{Imagenette} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    (PR) & \multicolumn{2}{c}{.05} & \multicolumn{2}{c}{.003} & \multicolumn{2}{c}{.05} & \multicolumn{2}{c}{.003} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    (B/A) & Bef. & Aft. & Bef. & Aft. & Bef. & Aft. & Bef. & Aft. \\
    \midrule
    Adap-B  & .232 & .083 & .045 & .056 & .875 & .029 & .525 & .019 \\
    Adap-P  & .108 & .112 & .883 & .080 & .670 & .021 & .017 & .001 \\
    Badnet  & 1.00 & .346 & 1.00 & .028 & 1.00 & .000 & .867 & .000 \\
    Blended & .998 & .333 & .948 & .000 & .989 & .000 & .735 & .001 \\
    Bpp     & .998 & .334 & .005 & .340 & .736 & .001 & .010 & .000 \\
    Dfst    & .654 & .233 & .324 & .058 & .324 & .008 & .457 & .010 \\
    Grond   & .425 & .033 & .201 & .168 & .009 & .011 & .005 & .016 \\
    Narcis. & 1.00 & .145 & .989 & .000 & .861 & .000 & .136 & .000 \\
    Wanet   & .985 & .327 & .203 & .338 & .972 & .000 & .610 & .000 \\
    \bottomrule
    \addlinespace[2pt]
    \multicolumn{9}{l}{\textit{Bef.: Before Defense, Aft.: After Defense (ASR)}} \\
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \scriptsize 
    \caption{F1 Scores for CIFAR-10 and Imagenette (ResNet18).}
    \label{tab:f1_merged}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{l cc cc cc}
    \toprule
    & \multicolumn{2}{c}{\textbf{SPECTRE}} & \multicolumn{2}{c}{\textbf{STRIP}} & \multicolumn{2}{c}{\textbf{Spectral Signatures}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    \textbf{Attack} & \textbf{.05} & \textbf{.003} & \textbf{.05} & \textbf{.003} & \textbf{.05} & \textbf{.003} \\
    \midrule
    \multicolumn{7}{c}{\textit{CIFAR-10}} \\
    \midrule
    Adap-B          & .056 & .006 & .016 & .018 & .010 & .000 \\
    Adap-P          & .081 & .006 & .107 & .723 & .052 & .001 \\
    BadNet          & .120 & .008 & .995 & .995 & .217 & .038 \\
    Blended         & .053 & .006 & .993 & .970 & .000 & .011 \\
    Bpp             & .117 & .007 & .878 & .903 & .110 & .001 \\
    DFST            & .067 & .006 & .000 & .000 & .001 & .000 \\
    Grond           & .089 & .006 & .061 & .073 & .099 & .010 \\
    Narcissus       & .080 & .006 & .995 & .963 & .000 & .006 \\
    Wanet           & .089 & .007 & .943 & .807 & .001 & .001 \\
    \midrule
    \multicolumn{7}{c}{\textit{Imagenette}} \\
    \midrule
    Adap-B    & .063 & .006 & .188 & .030 & .022 & .000 \\
    Adap-P    & .078 & .005 & .697 & .127 & .017 & .000 \\
    Badnet    & .116 & .008 & .978 & .960 & .220 & .039 \\
    Blended   & .054 & .005 & .977 & .857 & .158 & .033 \\
    Bpp       & .096 & .010 & .793 & .825 & .202 & .001 \\
    Dfst      & .051 & .006 & .007 & .055 & .000 & .000 \\
    Grond     & .093 & .006 & .244 & .216 & .074 & .007 \\
    Narcissus & .088 & .006 & .877 & .423 & .054 & .006 \\
    Wanet     & .071 & .008 & .933 & .893 & .061 & .000 \\
    \bottomrule
    \end{tabular}
\end{table}

==> sections/experimental_settings_obsolete.tex <==
\begin{table*}
    \footnotesize
    \centering
    \caption{Mean $\mu$ and standard deviation $\sigma$ used to normalize each dataset in this study. Normalization is performed separately for each of the three color channels.}
    \label{tab:normalization}
    \begin{tabular}{c ccc ccc ccc ccc}
        \toprule
        Dataset & \multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} & \multicolumn{3}{c}{Tiny-ImageNet} & \multicolumn{3}{c}{Imagenette} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} Color channel & R&G&B & R&G&B & R&G&B & R&G&B\\ \midrule
        $\mu$ & 0.4914 & 0.4822 & 0.4465 & 0.5071 & 0.4865 & 0.4409 & 0.4802 & 0.4481 & 0.3975 & 0.4671 & 0.4593 & 0.4306\\
        $\sigma$ & 0.247 & 0.243 & 0.261 & 0.2673 & 0.2564 & 0.2762 & 0.2302 & 0.2265 & 0.2262 & 0.2692 & 0.2657 & 0.2884\\
        \bottomrule
    \end{tabular}
\end{table*}


\section{Experimental Settings}
\label{sec:experimental_settings}

We evaluate footprints using the metrics in Table~\ref{tab:metrics} across the datasets, architectures, and attacks described below.

\paragraph{Datasets}
We use CIFAR-10/100~\cite{krizhevsky2009cifar} (50k/10k, RGB, $32{\times}32$), Imagenette~\cite{repoImagenette} (10 classes; we center-crop to square and downscale to $80{\times}80$), and Tiny-ImageNet~\cite{le2015tiny} (200 classes, native $64{\times}64$). Unless specified otherwise, we follow BackdoorBench data processing for each dataset. 
% Augmentations: \texttt{RandomCrop(padding=4)}, \texttt{RandomRotation($\pm10^\circ$)}, \texttt{RandomHorizontalFlip(p=0.5)} (CIFAR-10 only), and channel-wise \texttt{Normalize}.

\paragraph{Architectures}
We use ResNet-18~\cite{he2015resnets}, VGG-16~\cite{simonyan2015vgg}, and ViT-Small~\cite{alexey2021vit} for conducting experiments. Implementations are aligned across attacks (e.g., adaptive average pooling for non-$32{\times}32$ inputs) to ensure comparable feature dimensions and training behavior.

\paragraph{Implementations}
We use official repositories for Adap-Patch/Blend, DFST, Grond, DFBA, and BackdoorBench~\cite{baoyuan2022bb} for BadNets, Blend, WaNet, BppAttack, and benign baselines; Narcissus is ported into BackdoorBench. Minor fixes standardize normalization, batching, and trigger I/O across attacks.


\subsection{Training Settings}
\label{sec:exp_settings:train_settings}

\textbf{Optimizer and schedule.} All models train from scratch with SGD (momentum 0.9, weight decay $5{\times}10^{-4}$) and MultiStepLR (milestones at epochs 100 and 150 with $\gamma{=}0.1$; total 200 epochs). Batch size is 100 (CIFAR-10/100), 20 (Imagenette), and 64 (Tiny-ImageNet), chosen to (i) fit memory and (ii) preserve exact poisoned counts for $5\%$ PR in batch-wise poisoning (see below). These choices follow settings from related work.

\textbf{Targets and poisoning rates.} We use all-to-one attacks targeting class index 0 in each dataset. Poisoning rates (PR) are $5\%$ and $0.3\%$, with a few exceptions. WaNet and BppAttack on CIFAR-10 use $2\%$ instead of $0.3\%$, as their imperceptible triggers are difficult for backdoored models to learn at low poisoning rates. Clean-label attacks (Narcissus, Grond) use $0.7\%$ on CIFAR-100 and $0.4\%$ on Tiny ImageNet instead of $5\%$, since only target-class samples (which make up $1\%$ of CIFAR-100 and $0.5\%$ of Tiny ImageNet) can be poisoned. For batch-wise poisoning (WaNet, BppAttack, DFST), we adopt BackdoorBench’s rounding fix: if $\text{PR}\times\text{batch\_size} < 1$, a single poisoned example is inserted into a fraction of batches so that the dataset-level fraction matches PR in expectation.

\textbf{Normalization.} We normalize inputs during training and evaluation; when a trigger generator operates on unnormalized pixels (e.g., UPGD in Grond), normalization is applied immediately before model forward passes to keep $l_\infty$ constraints on the unnormalized perturbation well-defined.


\subsection{Attack-specific Settings}
\label{sec:methodology:train_settings:backdoor_specific}

We follow paper or repo defaults unless stated otherwise; Table~\ref{tab:atk_settings} summarizes the key settings we adjust or standardize.
\begin{itemize}
  \item \textbf{BadNets.} Checkerboard $3{\times}3$ trigger (CIFAR), proportionally scaled to $7{\times}7$ (Imagenette). To avoid cropping from \texttt{RandomCrop}, we shift the trigger 4 px inward from the bottom-right corner.
  \item \textbf{Blend.} We use the original ``Hello Kitty'' trigger (upscaled to $80{\times}80$ for Imagenette); blend ratio $\alpha{=}0.2$ at test time for consistency with Adap-Blend.
  \item \textbf{BppAttack.} Dithering is disabled (both official and BackdoorBench defaults struggle to maintain ASR with dithering on); color depth $d{=}5$; negative rate equals PR.
  \item \textbf{Adap-Patch / Adap-Blend.} Defaults for CIFAR; Imagenette triggers are scaled proportionally (as for BadNets). For Adap-Patch, we randomize trigger choice on Imagenette to avoid class-order bias in the official implementation.
  \item \textbf{DFST.} Environment fixes (package versions; TensorFlow GPU memory cap) and the BackdoorBench-style batch poisoning fix to enable low PR. Loss weights $(w_{\text{SSIM}},w_{\text{detox}}){=}(0.1,0.3)$.
  \item \textbf{Narcissus.} Surrogate architecture matches the victim; POOD datasets: CIFAR-100 for CIFAR-10 targets, CIFAR-10 for CIFAR-100/Imagenette targets. We train the surrogate on POOD only (then fine-tune on target-class data), consistent with the paper; normalization is aligned to reuse pretrained benign models as surrogates.
  \item \textbf{Grond.} Adds dataset normalization and reuse of benign surrogates. UPGD operates in pixel space with $\|\delta\|_\infty\le8$; ABI uses CLP threshold $u{=}3$.
  \item \textbf{DFBA.} We reuse BackdoorBench-pretrained benign models and modify DFBA to respect normalization by normalizing the patch trigger before computing the switch-neuron bias. Trigger size $3{\times}3$, threshold $\lambda{=}0.1$, and amplification $\gamma$ tuned to the smallest one-decimal value yielding $\text{ASR}{=}100\%$.
\end{itemize}


\begin{table}[t]
\centering
\footnotesize
\caption{Attack-specific settings used in our experiments.}
\label{tab:atk_settings}
\begingroup\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.05}
\begin{threeparttable}
\begin{tabular}{lll}
\toprule
Attack & Setting & Value\\ \midrule
\multirow{2}{*}{BadNets} & pattern & black \& white checkerboard\\
& size & $3{\times}3$ (CIFAR), $7{\times}7$ (Imagenette)\\
\midrule
\multirow{2}{*}{Blend} & trigger & \texttt{hellokitty\_32.png}\tnote{1}\\
& blend $\alpha$ & $0.2$\\
\midrule
\multirow{3}{*}{WaNet} & grid size $k$ & $4$\\
& warp strength $s$ & $0.5$\\
& noise prob.\ $\rho_n$ & $2\times$PR\\
\midrule
\multirow{3}{*}{BppAttack} & color depth $d$ & $5$\\
& dithering & off\\
& negative rate & PR\\
\midrule
\multirow{2}{*}{Adap-Patch} & trigger & default\tnote{2}\\
& conservatism $\eta$ & $2/3$\\
\midrule
\multirow{3}{*}{Adap-Blend} & trigger & default (as Blend)\\
& $(\alpha_{\text{train}},\alpha_{\text{test}})$ & $(0.15, 0.2)$\\
& conservatism $\eta$ & $0.5$\\
\midrule
\multirow{4}{*}{DFST} & blend $\alpha$ & $0.6$\\
& detox ratio & $0.01$\\
& detox epochs & $10$\\
& $(w_{\text{SSIM}},w_{\text{detox}})$ & $(0.1, 0.3)$\\
\midrule
\multirow{4}{*}{Narcissus} & surrogate arch. & = victim arch.\\
& $\|\delta\|_\infty$ & $\le 16$\\
& magnification & $3$\\
& POOD & see text\\
\midrule
\multirow{3}{*}{Grond} & surrogate arch. & = victim arch.\\
& $\|\delta\|_\infty$ & $\le 8$\\
& CLP threshold $u$ & $3$\\
\midrule
\multirow{2}{*}{DFBA} & trigger size & $3{\times}3$\\
& threshold $\lambda$ & $0.1$\\

\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
\item[1] Upscaled to $80{\times}80$ for Imagenette.
\item[2] Triggers scaled for Imagenette as in BadNets.
\end{tablenotes}
\end{threeparttable}
\endgroup
\end{table}

\begin{table}[!t]
    \centering   
    
    \caption{Python library modules implementing each input-space metric.}
    \label{tab:metric_implementations}
    
    \footnotesize
    \setlength{\tabcolsep}{3pt}          % tighter columns
    \renewcommand{\arraystretch}{1.15}   % a bit more row height

    \begin{threeparttable}
        % widths sum to < 1.0\linewidth (leave room for intercolumn space)
        \begin{tabular}{@{}L{0.20\linewidth} L{0.52\linewidth} L{0.24\linewidth}@{}}
            \toprule
            Metric & Implementation & Notes \\ \midrule
            $l^p$ norms &
            \href{https://numpy.org/doc/stable/reference/generated/numpy.linalg.norm.html}{\texttt{numpy.linalg}} & -- \\
            MSE &
            \href{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.mean_squared_error.html}{\texttt{sklearn.metrics}} & -- \\
            PSNR &
            \href{https://scikit-image.org/docs/stable/api/skimage.metrics.html\#skimage.metrics.peak_signal_noise_ratio}{\texttt{skimage.metrics}} & -- \\
            SSIM &
            \href{https://scikit-image.org/docs/stable/api/skimage.metrics.html\#skimage.metrics.structural_similarity}{\texttt{skimage.metrics}} & -- \\
            LPIPS &
            \href{https://pypi.org/project/lpips/}{\texttt{lpips}} & v0.1 (AlexNet) \\
            IS &
            \href{https://pytorch.org/docs/stable/hub.html}{\texttt{torch.hub}}; \href{https://docs.scipy.org/doc/scipy/reference/generated/scipy.special.rel_entr.html}{\texttt{scipy.special}} &
            Inception v3; KL divergence \\
            pHash &
            \href{https://pypi.org/project/ImageHash/}{\texttt{imagehash}} & -- \\
            SAM &
            \href{https://lightning.ai/docs/torchmetrics/stable/image/spectral_angle_mapper.html}{\texttt{torchmetrics.functional.image}} &
            Handles RGB $(0,0,0)$ via $\varepsilon$\tnote{1} \\
            \bottomrule
        \end{tabular}

        \begin{tablenotes}\footnotesize
            \item[1] To avoid divide-by-zero for pixels with value $(0,0,0)$, we replace them by $(\varepsilon,\varepsilon,\varepsilon)$ with $\varepsilon=10^{-8}$ before computing SAM.
        \end{tablenotes}
    \end{threeparttable}
    
\end{table}

\FloatBarrier




\subsection{Stealthiness Metric Implementations}
\label{sec:methodology:metrics}

\textbf{Input-space metrics.} We compute $l_p$ norms ($p\!\in\!\{1,2,\infty\}$), MSE, PSNR, SSIM~\cite{wang2004ssim}, LPIPS~\cite{zhang2018lpips}, IS~\cite{salimans2016is}, pHash (DCT-based; Hamming similarity), and SAM~\cite{yuhas1992sam} with standard libraries (see \autoref{tab:metric_implementations} for exact modules). All scores are averaged over the test set. For asymmetric trigger attacks, we also report the results for training sets.

\textbf{Feature-space metrics.} For Silhouette Score (SS)~\cite{rousseeuw1987silhouette} we follow Activation Clustering (AC)~\cite{chen2018ac} but (i) include all training samples (not only correctly classified ones), (ii) embed penultimate-layer activations with t-SNE (sklearn, perplexity = 30.0) rather than ICA, and (iii) cluster by ground truth poison labels (clean vs.\ triggered) to measure separability from the attacker’s perspective. Scores are computed per target class and then averaged. For DSWD~\cite{doan2021dswd}, we project clean/triggered embeddings onto discriminant directions derived from classifier weights and accumulate 1D Wasserstein-2 distances using \texttt{ot.wasserstein\_1d}; directions and layer are fixed across models for comparability. Lower SS/DSWD implies greater feature-space stealthiness.

\textbf{Parameter-space metrics.} UCLC and TAC follow CLP~\cite{zheng2022clp}. UCLC is data-free and upper-bounds each channel’s downstream sensitivity; TAC measures the expected activation change caused by the trigger, per channel, over a held-out set. We (i) evaluate UCLC on all convolutional channels and report the maximum (backdoors can localize to a few units), and (ii) compute TAC on the last conv layer only (as in~\cite{xu2025grond}), reporting its maximum statistics. When inputs are normalized, TAC uses the same normalized pipeline as training/inference to avoid scale artifacts.



\subsection{Additional Cross-Architecture Analysis}
\label{app:architecture_ranking}

Figure~\ref{fig:architecture_feature_ranks} compares the combined
feature-space rankings across architectures.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{img/arch_feature_scatter.pdf}
    \caption{Combined feature-space footprint rank of each attack on CIFAR-10 for ResNet18 versus VGG16 and ViT-Small. Rank 1 denotes the smallest measured feature-space footprint. VGG16 broadly follows the
ResNet18 ordering, whereas ViT-Small diverges, reflecting differences in representation geometry and the low ASR of several attacks on
ViT-Small.}
\label{fig:architecture_feature_ranks}
\end{figure}

==> sections/experiments.tex <==
% Table 11 in the thesis
\renewcommand{\arraystretch}{0.8}
\begin{table}[t]
    \centering
    \scriptsize
    \setlength\tabcolsep{3pt}
    \caption{Backdoor performance of ResNet18 models. The benign accuracy (BA) is shown for both benign and backdoored models. The poisoning rate (PR) is specified for backdoored models, and their attack success rate (ASR) is also reported. For the backdoored models, ASR scores below 60\% are highlighted in red.
    *The poisoning rates vary per dataset.}
    \label{tab:attack-performance-4datasets}
    \begin{tabular}{lccccccccc}
    \toprule
        \multirow{2}{*}{Attack} & \multirow{2}{*}{PR (\%)} & \multicolumn{2}{c}{C10} & \multicolumn{2}{c}{C100} & \multicolumn{2}{c}{Tiny} & \multicolumn{2}{c}{Imagenette}\\
         \cmidrule(lr){3-4}
         \cmidrule(lr){5-6}
         \cmidrule(lr){7-8}
         \cmidrule(lr){9-10}
         ~ & ~ & BA & ASR & BA & ASR & BA & ASR & BA & ASR \\
         \midrule
         Benign & - & 94.7 & - & 73.3 & - & 59.21 & - & 87.7 & -\\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{BadNets} & 5 & 94.5 & 100 & 72.9 & 100 & 58.37 & 99.97 & 88.3 & 100\\
         ~ & 0.3 & 94.7 & 100 & 73.5 & 99.8 & 59.12 & 94.04 & 88.1 & 86.7\\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{Blend} & 5 & 94.3 & 99.8 & 72.4 & 99.7 & 58.24 & 99.38 & 88.6 & 98.9\\
         ~ & 0.3 & 94.8 & 94.8 & 73.6 & 88.6 & 58.74 & 84.22 & 88.6 & 73.5\\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{WaNet} & 5 & 93.4 & 98.5 & 66.8 & 99.8 & 57.88 & 99.93 & 86.6 & 97.2\\
         ~ & \scriptsize{2/0.3/0.3/0.3$^*$} & 93.5 & 95.3 & 66.6 & 91.7 & 58.64 & 87.94 & 79.1 & 61.0\\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{Bpp} & 5 & 94.4 & 99.8 & 73.0 & 99.9 & 59.36 & 98.43 & 88.9 & 73.6 \\
         ~ & \scriptsize{2/0.3/0.3/0.3$^*$} & 94.6 & 69.5 & 73.0 & 88.0 & 58.56 & \textcolor{red}{4.72} & 88.3 & \textcolor{red}{1.02} \\
         \cmidrule(lr){2-10}
         \multirow{2}{1cm}{Adap\\Patch} & 5 & 93.9 & \textcolor{red}{30.1} & 70.9 & 66.7 & 56.97 & \textcolor{red}{41.62} & 87.6 & \textcolor{red}{20.2}\\
         ~ & 0.3 & 94.5 & 92.2 & 72.7 & \textcolor{red}{2.98} & 58.39 & \textcolor{red}{0.26} & 88.1 & \textcolor{red}{0.565}\\
         \cmidrule(lr){2-10}
         \multirow{2}{1cm}{Adap\\Blend} & 5 & 94.0 & \textcolor{red}{53.9} & 71.8 & 90.6 & 57.59 & 96.36 & 87.6 & 94.9\\
         ~ & 0.3 & 94.6 & 87.9 & 72.6 & 82.0 & 58.9 & 81.58 & 88.5 & \textcolor{red}{54.4} \\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{DFST} & 5 & 95.0 & 100 & 73.6 & 100 & 59.23 & 100 & 88.7 & 99.5\\
         ~ & 0.3 & 94.8 & 100 & 73.6 & 99.9 & 58.79 & 99.84 & 88.4 & 99.7\\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{Narcissus} & \scriptsize{5/0.7/0.4/5$^*$} & 94.4 & 100 & 73.0 & 70.9 & 59.04 & 98.82 & 87.8 & 86.1\\
         ~ & 0.3 & 94.7 & 98.9 & 72.8 & \textcolor{red}{33.1} & 58.97 & 98.97 & 88.7 & \textcolor{red}{13.6} \\
         \cmidrule(lr){2-10}
         \multirow{2}{*}{Grond} & \scriptsize{5/0.7/0.4/5$^*$} & 94.7 & 92.9 & 74.7 & \textcolor{red}{58.7} & 59.02 & 76.32 & 87.0 & 60.2\\
         ~ & 0.3 & 94.5 & 76.6 & 74.7 & \textcolor{red}{43.5} & 58.68 & 74.29 & 87.4 & \textcolor{red}{1.81}\\
         \cmidrule(lr){2-10}
         DFBA & - & 94.3 & 100 & 72.0 & 100 & 55.95 & 100 & 87.6 & 100\\
         \bottomrule
    \end{tabular}
\end{table}


% four datasets in one, input space stealthiness
\begin{table*}[t]
    \scriptsize
    \centering
    \caption{Input-space stealthiness evaluation on four datasets.}
    % \setlength\tabcolsep{3pt}
    \renewcommand{\arraystretch}{0.7}
    \label{tab:input-stealthiness-all}
    \begin{tabular}{llcccccccccc}
    \toprule
    \multirow{2}{*}{Dataset} & Metric & $l_1 \downarrow$ & $l_2 \downarrow$ & $l_\infty \downarrow$ & MSE $\downarrow$& PSNR $\uparrow$& SSIM $\uparrow$& LPIPS $\downarrow$& IS $\downarrow$& pHash $\uparrow$& SAM $\downarrow$\\
    ~ & Ideal value & 0 & 0 & 0 & 0 & $\infty$ & 1 & 0 & 0 & 100 & 0 \\
    \midrule
    \multirow{13}{*}{CIFAR-10} & BadNets & \best{13.2} & 2.84 & 0.811 & 2.64e-3 & 25.8 & 0.956 & 4.41e-3 & 0.170 & 95.2 & \best{1.44e-3} \\
    ~ & Blend & 230 & 4.92 & 0.191 & 8.01e-3 & 21.0 & 0.784 & 0.0483 & 2.37 & 89.8 & 0.0830 \\
    ~ & WaNet & 46.5 & 1.42 & 0.173 & 7.17e-4 & 31.5 & 0.978 & 4.32e-3 & 0.270 & 96.1 & 0.0119 \\
    ~ & BppAttack & 24.6 & \best{0.525} & \best{0.0196} & \best{8.97e-5} & \best{40.5} & \best{0.992} & \best{1.94e-4} & \best{0.150} & \best{99.2} & 0.0239 \\
    ~ & Adap-Patch (train) & 22.5 & 2.06 & 0.315 & 1.53e-3 & 28.7 & 0.972 & 4.78e-3 & 0.296 & 95.2 & 9.43e-3 \\
    ~ & Adap-Patch (test) & 74.1 & 6.77 & \worst{0.913} & 0.0151 & 18.2 & 0.956 & 0.0120 & 0.724 & 87.7 & 8.94e-3 \\
    ~ & Adap-Blend (train) & 87.0 & 2.63 & 0.142 & 2.30e-3 & 26.4 & 0.903 & 0.0136 & 0.823 & 92.4 & 0.0336 \\
    ~ & Adap-Blend (test) & 232 & 4.97 & 0.192 & 8.15e-3 & 20.9 & 0.783 & 0.0485 & 2.37 & 89.8 & 0.0831 \\
    ~ & DFST & 487 & \worst{10.8} & 0.489 & \worst{0.0400} & \worst{14.0} & 0.719 & 0.165 & 2.22 & 88.6 & 0.316 \\
    ~ & Narcissus (train) & 188 & 3.43 & 0.0627 & 3.83e-3 & 24.2 & 0.818 & 0.0545 & 1.44 & 91.8 & 0.101 \\
    ~ & Narcissus (test) & \worst{542} & 9.98 & 0.188 & 0.0325 & 14.9 & \worst{0.532} & \worst{0.184} & \worst{3.68} & \worst{82.2} & \worst{0.331} \\
    ~ & Grond & 87.6 & 1.62 & 0.0348 & 8.59e-4 & 30.7 & 0.934 & 2.92e-3 & 0.918 & 97.9 & 0.0833 \\
    ~ & DFBA & 13.5 & 2.99 & 0.844 & 2.94e-3 & 25.3 & \best{0.992} & 1.66e-3 & 0.159 & 97.4 & 2.83e-3 \\
    \midrule
    \multirow{13}{*}{CIFAR-100} & BadNets & \best{13.3} & 2.91 & 0.839 & 2.79e-3 & 25.6 & 0.955 & 5.39e-3 & 0.182 & 94.1 & \best{1.66e-3} \\
    ~ & Blend & 232 & 4.98 & 0.191 & 8.23e-3 & 20.8 & 0.765 & 0.0512 & \worst{2.25} & 89.0 & 0.0876 \\
    ~ & WaNet & 55.3 & 1.64 & 0.177 & 9.55e-4 & 30.2 & 0.968 & 6.72e-3 & 0.308 & 95.2 & 0.0154 \\
    ~ & BppAttack & 24.3 & \best{0.520} & \best{0.0196} & \best{8.83e-5} & \best{40.5} & 0.991 & \best{2.06e-4} & \best{0.138} & \best{99.1} & 0.0235 \\
    ~ & Adap-Patch (train) & 22.7 & 2.09 & 0.320 & 1.59e-3 & 28.5 & 0.971 & 4.78e-3 & 0.297 & 94.4 & 9.51e-3 \\
    ~ & Adap-Patch (test) & 74.5 & 6.96 & \worst{0.928} & 0.0159 & 18.0 & 0.956 & 0.0135 & 0.805 & 86.2 & 9.73e-3 \\
    ~ & Adap-Blend (train) & 87.9 & 2.66 & 0.142 & 2.36e-3 & 26.3 & 0.894 & 0.0144 & 0.796 & 91.5 & 0.0356 \\
    ~ & Adap-Blend (test) & 234 & 5.02 & 0.192 & 8.36e-3 & 20.8 & 0.764 & 0.0513 & \worst{2.25} & 89.0 & 0.0877 \\
    ~ & DFST & 509 & \worst{11.3} & 0.495 & \worst{0.0444} & \worst{13.5} & 0.708 & \worst{0.169} & 2.16 & 87.7 & 0.312 \\
    ~ & Narcissus (train) & 174 & 3.27 & 0.0627 & 3.50e-3 & 24.6 & 0.884 & 0.0147 & 0.622 & 94.3 & 0.126 \\
    ~ & Narcissus (test) & \worst{528} & 9.82 & 0.188 & 0.0315 & 15.0 & \worst{0.630} & 0.166 & 2.22 & \worst{84.6} & \worst{0.347} \\
    ~ & Grond & 86.9 & 1.61 & 0.0347 & 8.50e-4 & 30.7 & 0.929 & 4.97e-3 & 0.876 & 97.9 & 0.0720 \\
    ~ & DFBA & 13.5 & 3.02 & 0.843 & 3.04e-3 & 25.2 & \best{0.993} & 7.74e-3 & 0.146 & 95.9 & 4.18e-3 \\
    \midrule
    \multirow{13}{*}{Tiny-ImageNet} & BadNets & 58.36 & 4.99 & 0.73 & 2.23e-3 & 26.53 & 0.96 & 4.15e-2 & 0.11 & 91.79 & 3.47e-3\\
    ~ & Blend & 921.81 & 9.95 & 0.2 & 8.22e-3 & 20.85 & 0.81 & 0.11 & 1.11 & 89.44 & 0.11\\
    ~ & WaNet & 317.02 & 4.94 & 0.35 & 2.20e-3 & 26.58 & 0.93 & 4.03e-2 & 0.27 & 97.35 & 2.60e-2\\
    ~ & BppAttack & 96.26 & \best{1.04} & \best{1.96e-2} & \best{8.76e-5} & \best{40.57} & 0.99 & \best{8.75e-4} & 9.75e-2 & 99.42 & 3.14e-2\\
    ~ & Adap-Patch (train) & 23.54 & 2.17 & 0.33 & 4.22e-4 & 34.22 & 0.99 & 2.56e-3 & 5.07e-2 & 96.93 & 2.93e-3\\
    ~ & Adap-Patch (test) & 75.68 & 7.06 & \worst{0.96} & 4.11e-3 & 23.87 & 0.99 & 8.12e-3 & 0.17 & 92.05 & 3.05e-3\\
    ~ & Adap-Blend (train) & 358.75 & 5.45 & 0.15 & 2.47e-3 & 26.07 & 0.91 & 4.19e-2 & 0.49 & 91.8 & 4.67e-2\\
    ~ & Adap-Blend (test) & 955.04 & 10.28 & 0.2 & 8.77e-3 & 20.58 & 0.79 & 0.13 & 1.42 & 89.21 & 0.11\\
    ~ & DFST & 1.97e+3 & 22.16 & 0.53 & 4.18e-2 & 13.83 & 0.68 & 0.32 & 1.72 & 87.87 & 0.31\\
    ~ & Narcissus (train) & 1.23e+3 & 12.1 & 0.2 & 1.19e-2 & 19.23 & 0.65 & 0.22 & 1.55 & 85.56 & 0.26\\
    ~ & Narcissus (test) & \worst{3.29e+3} & \worst{33.31} & 0.59 & \worst{9.05e-2} & \worst{10.43} & \worst{0.36} & \worst{0.56} & \worst{4.73} & \worst{70.98} & \worst{0.5}\\
    ~ & Grond & 671.95 & 6.31 & 6.67e-2 & 3.25e-3 & 24.89 & 0.8 & 0.16 & 1.68 & 96.83 & 0.17\\
    ~ & DFBA & \best{13.34} & 3.01 & 0.87 & 7.49e-4 & 31.26 & \best{0.99} & 2.09e-3 & \best{4.42e-2} & \best{99.59} & \best{1.34e-3}\\
    \midrule
    \multirow{13}{*}{Imagenette} & BadNets & 73.3 & 6.94 & 0.879 & 2.54e-3 & 26.0 & 0.981 & 0.0152 & 0.0331 & 97.2 & 1.44e-3 \\
    ~ & Blend & 1.62e-3 & 13.8 & 0.198 & 0.0100 & 20.0 & 0.697 & 0.203 & 3.10 & 89.9 & 0.0968 \\
    ~ & WaNet & 225 & 2.94 & 0.190 & 4.94e-4 & 33.3 & 0.981 & 0.0140 & 0.0775 & 98.0 & 0.0111 \\
    ~ & BppAttack & 151 & \best{1.30} & \best{0.0196} & \best{8.79e-5} & \best{40.6} & 0.983 & \best{1.87e-3} & 0.0990 & 99.4 & 0.0294 \\
    ~ & Adap-Patch (train) & 136 & 5.18 & 0.342 & 1.54e-3 & 28.2 & 0.967 & 0.0229 & 0.175 & 94.7 & 0.0101 \\
    ~ & Adap-Patch (test) & 424 & 16.7 & \worst{0.960} & 0.0147 & 18.4 & 0.955 & 0.0540 & 0.238 & 86.9 & 9.00e-3 \\
    ~ & Adap-Blend (train) & 615 & 7.35 & 0.147 & 2.87e-3 & 25.4 & 0.865 & 0.0769 & 0.844 & 92.0 & 0.0413 \\
    ~ & Adap-Blend (test) & 1.64e3 & 13.9 & 0.198 & 0.0102 & 19.9 & 0.697 & 0.203 & 3.09 & 89.9 & 0.0969 \\
    ~ & DFST & 3.22e3 & \worst{28.9} & 0.532 & \worst{0.0456} & \worst{13.5} & 0.692 & 0.335 & 1.52 & 88.1 & \worst{0.334} \\
    ~ & Narcissus (train) & 1.17e3 & 8.55 & 0.0627 & 3.81e-3 & 24.2 & 0.861 & 0.113 & 0.669 & 93.4 & 0.139 \\
    ~ & Narcissus (test) & \worst{3.31e3} & 24.6 & 0.188 & 0.0317 & 15.0 & \worst{0.615} & \worst{0.428} & \worst{3.37} & \worst{82.8} & 0.268 \\
    ~ & Grond & 476 & 3.66 & 0.0352 & 7.00e-4 & 31.6 & 0.882 & 0.0482 & 1.02 & 99.1 & 0.0521 \\
    ~ & DFBA & \best{13.5} & 3.05 & 0.855 & 4.90e-4 & 33.1 & \best{0.999} & 2.07e-3 & \best{0.0312} & \best{99.8} & \best{8.93e-4} \\
    \bottomrule
    \end{tabular}
\end{table*}


\section{Experimental Results}
\label{sec:experimental_results}

%In this section, we present our results from three perspectives: input-space, feature-space, and parameter-space.
The experiments are conducted on four datasets (CIFAR-10~\cite{krizhevsky2009cifar}, CIFAR-100~\cite{krizhevsky2009cifar}, Tiny-ImageNet~\cite{le2015tiny}, Imagenette~\cite{repoImagenette}) and three model architectures (ResNet~\cite{he2015resnets}, VGG~\cite{simonyan2015vgg}, ViT~\cite{alexey2021vit}). Details on stealthiness metrics are in Appendix~\ref{sec:stealthiness_metrics}, and on experimental settings in Appendix~\ref {sec:experimental_settings}. We provide a baseline measurement on the CIFAR-10 dataset for stealthiness metrics in Appendix~\ref{sec:baselines}, and experimental results for VGG and ViT in Appendix~\ref{sec:other-arch}. Finally, we discuss the limitations of our experiments in Appendix~\ref{sec:limitations}.

\subsection{The Performance of Backdoor Attacks}
\label{subsec:input-space-stealthiness}

To evaluate the stealthiness of backdoor attacks, it is necessary to ensure the attack is successfully applied to the models.
% Otherwise, if the attack is successful and the model can be considered a benign model, since it contains no backdoor.
% The backdoor stealthiness of the benign model is meaningless since no designed backdoor in the benign model.
Table~\ref{tab:attack-performance-4datasets} provides the performance of ten backdoor attacks and benign models on the four datasets.
The attack success rate (ASR) is marked red if it is lower than 60\% (the threshold of 60\% is chosen following~\cite{xu2025grond}).

\textcolor{black}{
\textbf{Note on Low-ASR Models.} Several attack configurations (e.g., BppAttack at 0.3\% PR) result in an ASR below 60\%. We include these models in our stealthiness analysis for completeness, as it is scientifically valuable to understand whether ``failed'' attacks still leave detectable footprints. However, readers should interpret high stealthiness scores for low-ASR models with caution; a footprint is naturally smaller when the malicious functionality is not successfully embedded. In our subsequent validation (Section~\ref{sec:correlation_methodology}), we explicitly control for attack strength to ensure our metrics predict evasion beyond simple correlations with ASR.
}

We have controlled the ASR of WaNet and BppAttack on CIFAR-10 by changing the poisoning rate from 0.3\% to 2\%, which Qi et al. claim is the minimum poisoning rate for WaNet~\cite[Figure 6]{qi2023wanetlowpr}. For Adap-Patch and Adap-Blend, resolving the low ASR is more difficult because it is influenced by the ratio between the poisoned and regularization samples. Although skewing this ratio in favor of the poisoned samples may increase the ASR, it could also degrade the attacks' feature-space stealthiness.

% \noindent
% \textbf{Attack Success Rate (ASR) Analysis.}
% The ASR could be decreased due to lower poisoning rates in \autoref{tab:attack-performance-4datasets}.
% For example, on the CIFAR-10 dataset, both WaNet and BppAttack fail to achieve a high ASR at the lower poisoning rate of 0.3\%. For WaNet, we cannot compare our ASR directly with the original paper, as the authors exclusively used a poisoning rate of 10\%~\cite[Section 4.1]{nguyen2021wanet}. However, our result is supported by other research evaluating WaNet on CIFAR-10. For example, Qi et al. found that to successfully inject the backdoor, the minimum poisoning rate for WaNet is 2\%~\cite[Figure 6]{qi2023wanetlowpr}. Furthermore, Xu et al. were also unable to achieve satisfactory ASR with WaNet at a poisoning rate of 0.5\%~\cite[Section 5.2]{xu2025grond}.

% For BppAttack, the lowest poisoning rate used in the original paper is 2.5\%~\cite[Figure 6]{wang2022bppattack}. At this poisoning rate, the authors of BppAttack achieved an ASR below 25\% on CIFAR-10. At our significantly lower poisoning rate of 0.3\%, it seems logical that the ASR decreases even
% further. Furthermore, the fact that the BppAttack ASR is lower than WaNet's at this poisoning rate makes sense when considering the stealthiness results in Table~\ref{tab:input-stealthiness-all}, which show that BppAttack's trigger is stealthier in input space than WaNet's. As such, the model may struggle more to distinguish the poisoned samples from the benign samples for BppAttack than for WaNet.


% \noindent
% \textbf{Large Drop in Benign Accuracy for WaNet.}
% We observe that the benign accuracies of almost all backdoored models are quite close to the benign model's; the few exceptions all occur for the WaNet attack. Specifically, both CIFAR-100 models and the Imagenette model with 0.3\% PR achieve a significantly lower accuracy than their respective benign models.

% For the CIFAR-100 models, we suspect that the cause of this phenomenon is the complexity of the dataset. Usually, backdoor attacks can achieve a high BA and ASR because the victim models have spare learning capacity~\cite{liu2018finepruning}; the backdoor can be inserted into neurons that are not used for the benign classification task. With CIFAR-100, however, the benign classification task may require more of the model's capacity due to the large number of classes, causing the backdoor to impact the model's performance on this task significantly.

% On the other hand, the low benign accuracy of the Imagenette model is probably caused by the dataset having a relatively low amount of poisoned data samples due to its smaller size. At 0.3\% PR, the expected amount of poisoned samples is $0.3\% \times 9469 \approx 28$, which may not be sufficient for the model to properly distinguish them from the benign samples in a way that generalizes well to the testing dataset.

% \todo{while we give results for other models in appendix, we should mention if they are aligned or not or what is happenning}


\subsection{Input-space Stealthiness} \label{subsec:experimental_results_input}

\noindent
\textbf{Overview.}
We compare a clean image from the Imagenette testing dataset with its poisoned versions for all attacks in Figure~\ref{fig:imagenette-triggers}. 
The evaluation results on input space metrics are provided in Table~\ref{tab:input-stealthiness-all}.
In general, BppAttack is considered the stealthiest attack by the vast majority of metrics. Only the metrics that favor patch-based triggers, like the $l_1$ norm, SAM, and (to a lesser extent) SSIM, consider BadNets or DFBA to be stealthier. For the Imagenette and Tiny-ImageNet datasets, DFBA achieves significantly better stealthiness than for the other two datasets, due to its trigger staying the same size across all datasets, despite the images now being larger. Besides the three metrics mentioned above, DFBA also outperforms BppAttack with the IS and pHash metrics.

WaNet, which uses a dynamic trigger like BppAttack, also achieves good stealthiness results across all metrics and datasets. We find it interesting that while WaNet and BppAttack are no longer considered state-of-the-art backdoor attacks, they still achieve higher input-space stealthiness than more recent attacks like Narcissus and Grond, which also consider this type of stealthiness. The reason for this is probably that the latter two attacks aim to be invisible ($l_\infty = 8$ in related adversarial machine learning papers), rather than being more invisible than all other attacks in the input space.
Furthermore, they assume a weaker threat model since they are clean-label attacks. Thus, to consider these additional factors and still be effective, Narcissus and Grond have compromised on input-space stealthiness. 

From our results, this compromise is more apparent for Narcissus. Its inference-time trigger is actually considered the least stealthy by the majority of the metrics on all datasets. In the Narcissus attack, it is assumed that the trigger can be magnified at inference time because the inputs to the model are less likely to undergo any inspection, be it manual or automatic, during inference than during training; after all, a model deployed for inference should ideally be as fast and efficient as possible. Therefore, the lack of input-space stealthiness of the inference-time trigger is deemed to be a smaller risk. However, if any inference-time inspection does take place, the large perturbation induced by the magnified trigger would surely pose problems for the attack. For example, we would expect Narcissus to be easily detected by the STRIP defense~\cite{gao2020strip} described in Section~\ref{sec:related_work:stealthiness:input}. 

Grond, on the other hand, does not magnify the trigger at inference time. Its trigger is also more stealthy during training because it is generated based on a lower $l_\infty$ norm constraint. The stealthiness difference between Grond and Narcissus is most apparent on the CIFAR-10 dataset; Grond achieves rather consistent results across all datasets, while Narcissus is considered significantly less stealthy on CIFAR-10. We suspect that the choice of public out-of-distribution (POOD) dataset for Narcissus impacts the attack's input-space stealthiness, since CIFAR-100 and Imagenette share the same POOD dataset and achieve similar results.

% After Narcissus, the attack that achieves the worst results is DFST. This may come as a surprise, since DFST uses a dynamic trigger like WaNet and BppAttack, which achieve very good results. However, we believe the DFST results can be explained by the fact that its trigger seems to have a different goal than the other dynamic triggers. Whereas WaNet and BppAttack attempt to remain as close as possible to the original image, the goal of DFST is to make the poisoned images appear natural, so that they do not arouse suspicion in human inspectors. Therefore, our evaluation methodology is somewhat unfair to DFST; in a realistic scenario, a human inspector would likely not have access to the clean version of an image containing the trigger, making it impossible to compare the clean and poisoned versions. Still, our results suggest that the DFST trigger could be detected in other ways. Due to the large perturbation induced by the DFST trigger, we believe the attack could be detected by the STRIP defense, similar to Narcissus.

\noindent
\textbf{\boldmath$l_p$ norm, MSE and PSNR.}
The $l_p$ norm metrics are widely used to quantify the difference between benign images and perturbed images in adversarial machine learning~\cite{madry2019pgd,ian2015fgsm}. 
This paper utilizes $l_1$, $l_2$, and $l_3$ to evaluate the input-space stealthiness.
$l_1$ simply adds up the absolute values of the components, while $l_2$ is the standard notion of vector length and can be thought of as a normalized $l_1$ norm.
In contrast, $l_\infty$ only considers the largest absolute value among the image pixels.
In other words, $l_1$ and $ l_2$ accumulate the change of all pixels, but $l_\infty$ only takes the largest one into account.


Given that patch-based backdoor triggers affect only a small set of all pixels, they are favored by the $l_1$ and $l_2$ norms.
In contrast, patch-based triggers are not suitable in terms of $l_\infty$, as they can significantly alter a few pixels.
Take BadNets (patch-based) and Narcissus in Table~\ref{tab:input-stealthiness-all} as an example, while BadNets has much smaller $l_1$ and $l_2$ values, Narcissus is stealthier in terms of $l_\infty$. This phenomenon also applies to WaNet, BppAttack, DFST, and Grond.

% In addition, MSE is essentially L2 squared, and PSNR is the logarithmic measure based on MSE, normalized by signal range (MAX). Therefore, we observe similar measurements for the two metrics. In both cases, BppAttack is deemed the stealthiest, whereas DFST is considered the least stealthy.


\noindent
\textbf{SSIM, LPIPS, and IS.}
While the SSIM initially appears to align with previous metrics in ranking BppAttack and DFBA as the most stealthy triggers and the Narcissus inference-time trigger as the least, its unique contribution is revealed in the significant performance gap it identifies between the Narcissus and DFST triggers. Unlike the pixel-based $l_\infty$ norm, which is an exception but operates on a single pixel, SSIM evaluates the entire image's structural information to approximate human perceptual judgment. We posit that this methodological focus explains the pronounced difference, as SSIM effectively captures the noisier, more disruptive structural distortion introduced by the Narcissus trigger (as evidenced in Figure~\ref {fig:imagenette-triggers}), which substantially degrades image coherence and recognizability compared to the DFST trigger.

In addition, LPIPS and IS perform similarly to SSIM. For both metrics, DFST is considered significantly stealthier than inference-time Narcissus. Again, we believe this is because the DFST trigger leaves the subject of the images more recognizable than the magnified Narcissus trigger. Consequently, the Inception network's predicted class distribution changes less for DFST, and the IS value is smaller. 

% \todo{Observation is made for LPIPS and IS, but explanation only includes IS}

\noindent
\textbf{pHash.}
A more general observation unique to the pHash metric is that the relative difference between the greatest and smallest measurement is quite small. We think this is caused by the compression techniques used in pHash, such as converting images to grayscale, which are necessary to turn the images into 64-bit long hashes. The small hash size of pHash is useful for its intended application of efficiently comparing images. However, it causes a lot of information in the image to be lost. This makes it less suitable for evaluating backdoor stealthiness, as some differences induced by the trigger may be ignored.


% \begin{table}
%     \centering
%     \caption{Stealthiness of each individual Adap-Patch training trigger, as measured by MSE and SAM.}
%     \label{tab:results_sam_adap-patch}
%     \begin{tabular}{lc cc}
%         \toprule

%         \multicolumn{2}{c}{Adap-Patch} & \multirow{2}{*}{MSE} & \multirow{2}{*}{SAM} \\
%         \cmidrule(lr){1-2} Trigger & $\alpha_\text{train}$ \\ \midrule

%         Phoenix corner & 0.5 & 1.49e-3 & 4.30e-3 \\ 
%         Firefox & 0.2 & 1.08e-3 & 0.0226 \\ 
%         BadNets & 0.5 & 2.86e-3 & 1.88e-3 \\
%         Trojan square & 0.3 & 6.92e-4 & 8.91e-3 \\

%         \bottomrule
%     \end{tabular}
% \end{table}


\renewcommand{\arraystretch}{0.7}
\begin{table}[t]
\scriptsize
\centering
\setlength\tabcolsep{0.75pt}
\caption{Feature-space stealthiness of backdoored ResNet18 models trained on four datasets. The metrics used to evaluate each model are the silhouette score (SS) and discriminant sliced-Wasserstein distance (DSWD). For each metric and dataset, the \best{best} and \worst{worst} results are highlighted. Results that may be affected by the low ASR of the corresponding models (see Table~\ref{tab:attack-performance-4datasets}) are \underline{underlined}. The poisoning rates vary per dataset: Var.$^\dagger$: 2/0.3/0.3/0.3\%. Var.$^\ddagger$: 5/0.7/0.4/5\%.}
\label{tab:results_feature_resnet18}
\begin{tabular}{l c c c c c c c c c cccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{PR (\%)} 
& \multicolumn{2}{c}{C10} 
& \multicolumn{2}{c}{C100} 
& \multicolumn{2}{c}{Tiny} 
& \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& & SS$\downarrow$ & DSWD$\downarrow$ &
SS$\downarrow$ & DSWD$\downarrow$ &
SS$\downarrow$ & DSWD$\downarrow$ & 
SS$\downarrow$ & DSWD$\downarrow$\\
\midrule
\multirow{2}{*}{BadNets} 
& 5   & 0.507 & 2.01 & 0.511 & 1.27 & 0.295 & 1.067 & 0.588 & 1.78\\
& 0.3 & 0.355 & 2.54 & 0.462 & 1.29 & 0.463 & 1.145 & 0.260 & 1.49\\
\cmidrule(lr){2-10}
\multirow{2}{*}{Blend} 
& 5   & 0.473 & 2.05 & 0.435 & 1.27 & 0.339 & 1.339 & 0.022 & 1.60\\
& 0.3 & 0.276 & 2.08 & 0.379 & 1.32 & 0.423 & 1.236 & 0.097 & 1.27\\
\cmidrule(lr){2-10}
\multirow{2}{*}{WaNet} 
& 5   & 0.382 & 1.83 & 0.492 & 1.21 & 0.342 & 1.301 & 0.557 & 1.73\\
& Var.$^\dagger$ & 0.378 & 1.62 & 0.217 & 0.877 & 0.303 & 0.926 & 0.192 & 0.474\\
\cmidrule(lr){2-10}
\multirow{2}{*}{Bpp} 
& 5   & 0.500 & 1.91 & 0.527 & 1.37 & 0.433 & 1.36 & 0.607 & 1.34\\
& Var.$^\dagger$ & 0.371 & 0.952 & 0.540 & 1.31 & \underline{0.347} & \best{\underline{0.049}} & \underline{0.227} & \best{\underline{0.040}}\\
\cmidrule(lr){2-10}
\multirow{2}{1cm}{Adap\\Patch} 
& 5   & \underline{0.254} & \best{\underline{0.765}} & 0.060 & 0.46 & \best{\underline{0.067}} & \underline{0.248} & \underline{0.082} & \underline{0.588}\\
& 0.3 & 0.0500 & 1.91 & \underline{0.058} & \best{\underline{0.224}} & \underline{0.245} & \underline{0.084} & \underline{-0.046} & \underline{0.106}\\
\cmidrule(lr){2-10}
\multirow{2}{1cm}{Adap\\Blend} 
& 5   & \underline{0.231} & \underline{1.15} & \best{0.038} & 0.693 & 0.213 & 0.717 & 0.0630 & 1.26\\
& 0.3 & 0.149 & 2.10 & 0.191 & 1.28 & 0.311 & 0.996 & \best{\underline{-0.066}} & \underline{0.965}\\
\cmidrule(lr){2-10}
\multirow{2}{*}{DFST} 
& 5   & \worst{0.519} & 2.26 & 0.509 & 1.34 & 0.485 & 1.707 & \worst{0.64} & 2.20\\
& 0.3 & 0.339 & 2.63 & \worst{0.730} & 1.93 & \worst{0.63} & 1.74 & 0.261 & 2.15\\
\cmidrule(lr){2-10}
\multirow{2}{*}{Narcissus} 
& Var.$^\ddagger$ & 0.491 & 2.23 & 0.074 & 0.945 & 0.314 & 1.977 & 0.043 & 1.34\\
& 0.3 & -0.007 & 1.90 & \underline{0.062} & \underline{0.852} & 0.302 & 1.703 & \underline{-0.016} & \underline{0.883}\\
\cmidrule(lr){2-10}
\multirow{2}{*}{Grond} 
& Var.$^\ddagger$ & 0.435 & 1.82 & \underline{0.233} & \underline{0.861} & 0.327 & 1.122 & 0.031 & 1.05\\
& 0.3 & \best{-0.101} & 1.65 & \underline{0.208} & \underline{0.786} & 0.355 & 1.071 & \underline{0.055} & \underline{0.286}\\
\cmidrule(lr){2-10}
DFBA & - & - & \worst{15.2} & - & \worst{18.0} & - & \worst{10.74} & - & \worst{4.64}\\
\bottomrule
\end{tabular}
\end{table}

\noindent
\textbf{SAM.}
For the SAM, we observe a difference between the BadNets and DFBA measurements. BadNets is considered stealthier than DFBA and achieves the highest stealthiness with the SAM metric. Furthermore, WaNet achieves better stealthiness than BppAttack, while the opposite was true for all previous metrics. To explain these observations, a detailed analysis of the SAM measurements for the four aforementioned attacks is conducted in Appendix~\ref{sec:sam_analysis}.




\subsection{Feature-space Stealthiness}
\label{subsec:feature-space-stealthiness}

\noindent
\textbf{Overview.}
Based on our feature-space stealthiness evaluation (see \autoref{tab:results_feature_resnet18}), we have found that the behavior of the SS and DSWD metrics is quite different. For instance, the silhouette score is affected less by the ASR of a backdoored model than by DSWD. Another advantage of the silhouette score is that the feature-space t-SNE embedding on which it is based can be easily visualized (see Appendix~\ref{app:t-sne}, Figures~\ref{fig:cifar-tsne},~\ref{fig:cifar100-tsne},~\ref{fig:tiny-tsne}, and~\ref{fig:imagenette-tsne} for t-SNE plots on four datasets), providing support. On the other hand, from our results, DSWD is affected less by the poisoning rate of the attack than the silhouette score, except for the attacks where the t-SNE embeddings show the poisoned samples truly become harder to separate from the benign samples. Therefore, we believe that a backdoor attack should be evaluated against both of them to measure its feature-space stealthiness effectively.

\noindent
\textbf{Adaptive and Clean-label Attacks are Stealthiest.}
Adap-Patch, Adap-Blend, Narcissus, and Grond consistently achieve low silhouette scores. This result is not surprising for the adaptive attacks, as their trigger diversification and regularization samples are specifically designed to reduce the cohesion of the poisoned samples and their separation from the benign samples in feature space.

For Narcissus and Grond, we believe the high stealthiness of both models can be attributed to the same two factors. First, both attacks are clean-label, so the t-SNE embeddings are based only on samples originally from the target class. Second, both attacks use a trigger based on target class features. Therefore, the only difference between the clean samples and the poisoned samples is the features induced by the trigger, which are similar to those contained in the clean samples.

For the clean-label attacks, the silhouette scores on the CIFAR-10 dataset at 5\% PR are relatively high. We believe this makes sense from a stealthiness perspective for Narcissus, as the benign and poisoned clusters are quite easily separable in the t-SNE embedding (see Figure~\ref{fig:cifar-tsne}). Although this is not the case for Grond, the silhouette score is still quite high compared to other attacks, because the poisoned cluster is very cohesive. For example, the silhouette score of the 5\% WaNet model is lower than the Grond model because of the lack of cohesion in its poisoned cluster. However, the clusters are also easier to separate for WaNet. Therefore, we would argue that the Grond model may be considered stealthier. It seems that by considering both the cohesion and separability of the clusters, the silhouette score metric may result in measurements that are illogical from a stealthiness perspective.
With the DSWD metric, Grond outperforms the other three attacks. We believe this is because DSWD is measured on the testing dataset, where the asymmetric triggers of the adaptive attacks are stronger, whereas Grond's trigger remains unchanged. 

\noindent
\textbf{Correlation with ASR.}
We observe that the backdoored models with an ASR below 60\%, which are underlined in Table~\ref{tab:results_feature_resnet18}, generally achieve lower DSWD measurements than the backdoored models with higher ASR. Therefore, there seems to be a strong correlation between the ASR and DSWD of a backdoored model. The reason is that both the ASR and DSWD are measured on the poisoned testing dataset. A low DSWD indicates that the model extracts similar features from the benign and poisoned versions of data samples. Consequently, the model is unlikely to classify the poisoned samples as the target class, causing a low ASR.

For the silhouette score, the correlation with the ASR is weaker. For CIFAR-10 and CIFAR-100, the minimum SS is achieved by backdoored models with more than 60\% ASR. This is not the case for Imagenette, but the backdoored model with minimum SS still achieves close to 60\% ASR. The weaker correlation between the silhouette score and the ASR could be explained by the fact that the silhouette score is measured on the training dataset.

\noindent
\textbf{Poisoned Samples Form Distinct Groups.}
In the t-SNE embeddings in the feature space (see Figure~\ref{fig:cifar-tsne}), there are distinct groups within the cluster of poisoned samples. It is especially noticeable in the embeddings of the BadNets, WaNet, and BppAttack models with a 5\% poisoning rate. The poisoned samples are grouped by their ground-truth label in smaller clusters. This can be explained by the fact that the backdoored model is not only trained to associate the trigger with the target class, but also to classify benign samples correctly. Therefore, the backdoored models will also extract the benign features still present in the poisoned samples, which differ between each class. We suspect that the clustering by ground truth label is strongest for the aforementioned three attacks because they keep the benign features mostly intact; the BadNets trigger only covers a small part of the image, while the imperceptible WaNet and BppAttack triggers only slightly perturb the whole image.


\renewcommand{\arraystretch}{0.7}
\begin{table}[t]
\scriptsize
\centering
\caption{Parameter-space stealthiness of backdoored ResNet18 models trained on our three chosen datasets. The two metrics used to evaluate each model are the upper bound on the channel Lipschitz constant (UCLC) and trigger-activated change (TAC), both of which have the ideal value 0. For each metric and dataset, the \best{best} and \worst{worst} results are highlighted. Results that may be affected by the low ASR of the corresponding models (see Table~\ref{tab:attack-performance-4datasets}) are \underline{underlined}. *The poisoning rates vary per dataset.}
\label{tab:uclc-tac}
\setlength\tabcolsep{1pt}
\begin{tabular}{l c c c c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{PR (\%)} 
& \multicolumn{2}{c}{C10} 
& \multicolumn{2}{c}{C100} 
& \multicolumn{2}{c}{Tiny} 
& \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& & UCLC$\downarrow$ & TAC$\downarrow$ & UCLC$\downarrow$ & TAC$\downarrow$ & UCLC$\downarrow$ & TAC$\downarrow$ & UCLC$\downarrow$ & TAC$\downarrow$\\
\midrule
Benign & - & 6.09 & - & 4.92 & - & 4.19 & - & 5.31 & - \\
\cmidrule(lr){2-10}
\multirow{2}{*}{BadNets} 
& 5   & 6.59 & 3.90 & 4.64 & 7.32 & 4.52 & 21.34 & 6.22 & 15.3 \\
& 0.3 & 7.99 & 8.03 & 5.86 & 9.17 & 4.57 & 38.89 & 5.39 & 18.4 \\
\cmidrule(lr){2-10}
\multirow{2}{*}{Blend} 
& 5   & 6.49 & 3.05 & 4.73 & 6.46 & 4.54 & 23.87 & 4.99 & 6.24 \\
& 0.3 & 5.76 & 4.30 & 4.92 & 9.69 & 4.85 & 25.31 & 5.37 & 6.04 \\
\cmidrule(lr){2-10}
\multirow{2}{*}{WaNet} 
& 5   & 6.33 & 10.7 & 6.52 & 20.9 & 4.27 & 31.08 & 7.05 & 64.0 \\
& 2/0.3/0.3/0.3$^*$ & 7.68 & 14.3 & 6.39 & 11.2 & 4.02 & 30.13 & 6.49 & 2.55 \\
\cmidrule(lr){2-10}
\multirow{2}{*}{Bpp} 
& 5   & 9.42 & 8.50 & 8.76 & 16.3 & 7.9 & 32.41 & 8.82 & 59.2 \\
& 2/0.3/0.3/0.3$^*$ & 7.38 & 7.48 & 7.21 & 10.0 & \best{\underline{3.95}} & 10.63 & \underline{5.19} & \best{\underline{0.394}} \\
\cmidrule(lr){2-10}
\multirow{2}{1cm}{Adap\\Patch} 
& 5   & \underline{10.7} & \underline{6.44} & 5.35 & 6.83 & 4.14 & 14.88 & \underline{6.24} & \underline{11.5} \\
& 0.3 & 9.91 & 3.94 & \underline{6.06} & \best{\underline{1.45}} & 5.57 & \best{\underline{10.44}} & \underline{7.62} & \underline{1.42} \\
\cmidrule(lr){2-10} 
\multirow{2}{1cm}{Adap\\Blend} 
& 5   & \underline{5.60} & \best{\underline{2.14}} & 6.32 & 6.62 & 4.41 & 21.18 & 5.08 & 5.61 \\
& 0.3 & 7.70 & 4.58 & 5.51 & 12.4 & 4.14 & 20.54 & \underline{5.67} & \underline{4.71} \\
\cmidrule(lr){2-10}
\multirow{2}{*}{DFST} 
& 5   & 6.16 & 6.41 & 4.28 & 11.9 & 4.35 & 26.05 & 6.29 & 18.9 \\
& 0.3 & 6.37 & 11.8 & 5.69 & 15.4 & 5.12 & 30.0 & 4.61 & 10.8 \\
\cmidrule(lr){2-10}
\multirow{2}{*}{Narcissus} 
& 5/0.7/0.4/5$^*$ & 7.37 & 6.23 & 6.19 & 6.25 & 4.28 & 35.86 & 5.41 & 5.59 \\
& 0.3 & 6.88 & 2.15 & \underline{5.44} & \underline{3.78} & 4.33 & 27.24 & \underline{6.42} & \underline{4.64} \\
\cmidrule(lr){2-10}
\multirow{2}{*}{Grond} 
& 5/0.7/0.4/5$^*$ & 3.60 & 2.43 & \best{\underline{3.78}} & \underline{6.00} & 4.33 & 21.89 & \best{3.14} & 4.20 \\
& 0.3 & \best{3.18} & 2.30 & \underline{4.10} & \underline{4.32} & 4.33 & 23.79 & \underline{3.73} & \underline{2.19} \\
\cmidrule(lr){2-10}
DFBA & - & \worst{17.8} & \worst{413} & \worst{17.7} & \worst{413} & \worst{21.17} & \worst{959.33} & \worst{18.7} & \worst{959} \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Parameter-space Stealthiness}
\label{subsec:parameter-space-stealthiness}

We evaluate parameter-space stealthiness with the UCLC and TAC metrics. The measurements on
the backdoored ResNet18 models are given in Table~\ref{tab:uclc-tac}.
Results on other architectures are provided in Appendix~\ref{sec:other-arch}.
As explained in Section~\ref{sec:current_metrics:parameter}, UCLC and TAC measure each neuron individually. We compare the backdoored models via their maximum
UCLC and TAC values. In Appendix~\ref{sec:tac-visualization}, we visualize the TAC values of all neurons separately.


\noindent
\textbf{Correlation between ASR and Parameter Metrics.}
From the underlined results in Table~\ref{tab:uclc-tac}, most backdoored models with low ASR also have relatively low TAC.
On CIFAR-10, the lowest TAC is achieved by the Adap-Blend model with 5\% PR. Both on CIFAR-100 and Tiny-ImageNet, the Adap-Patch model with 0.3\% PR yields the lowest measurement. On Imagenette, the 0.3\% PR BppAttack model achieves the lowest TAC.
In the corresponding TAC plots for these backdoored models, their TAC values are quite similar to those of the benign model. In other words, the effect of the triggers on the backdoored models is not very different from their effect on the benign model. The benign model has not been trained to associate the trigger with the target class. Therefore, it makes sense that backdoored models, which are affected similarly by the trigger as the benign models, achieve low ASR. 

Compared to the TAC metric, we observe a weaker correlation between ASR and UCLC. The UCLC measurements are relatively low for some backdoored models with an ASR below 60\%, but the difference is not so significant as with the TAC metric. The only exceptions are the Grond models with low ASR, but the UCLC measurements for Grond are similar regardless of the ASR.

\noindent
\textbf{Grond is the Most Stealthy.}
For each dataset, the two models backdoored by Grond achieve the lowest UCLC. The consistently low UCLC of Grond is related to its Adversarial Backdoor Injection (ABI) module. ABI is a modified version of the CLP defense, which is performed during every training epoch of a Grond model. As explained in~\cite{xu2025grond}, the CLP defense prunes the neurons whose normalized UCLC is greater than some value $u$. This way, the only way to successfully inject the backdoor is to spread it over multiple neurons, which improves Grond's parameter-space stealthiness. In our experiments, the Grond models use $u=3$, and we measure the maximum normalized UCLC over all neurons. Therefore, it makes sense that our measurements for Grond are not much larger than 3.

\noindent
\textbf{DFBA is Least Stealthy.}
For each dataset, the DFBA model achieves not only the highest TAC but also the highest UCLC. However, compared to the other backdoored models, the TAC measurement is more extreme than the UCLC measurement. This is because TAC considers the neurons' activations, while UCLC only examines the neurons' weights. In DFBA, the activation of the compromised neuron on an image containing the trigger grows larger with each layer, whereas its modified weight is the same regardless of the layer. However, based on our UCLC results, it seems the compromised neuron in each layer of the DFBA model remains significantly less stealthy than the most compromised neuron in any other model.




% separated input space tables.
% \begin{table*}[t]
%     \centering
%     \caption{Input-space stealthiness evaluation on CIFAR-10.}
%     \label{tab:tinyimg-input-stealthiness}
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     Metric & $l_1$ & $l_2$ & $l_\infty$ & MSE & PSNR & SSIM & LPIPS & IS & pHash & SAM \\
%     Ideal value & 0 & 0 & 0 & 0 & $\infty$ & 1 & 0 & 0 & 100 & 0 \\
%     \midrule
%     BadNets & \best{13.2} & 2.84 & 0.811 & 2.64e-3 & 25.8 & 0.956 & 4.41e-3 & 0.170 & 95.2 & \best{1.44e-3} \\
%     Blend & 230 & 4.92 & 0.191 & 8.01e-3 & 21.0 & 0.784 & 0.0483 & 2.37 & 89.8 & 0.0830 \\
%     WaNet & 46.5 & 1.42 & 0.173 & 7.17e-4 & 31.5 & 0.978 & 4.32e-3 & 0.270 & 96.1 & 0.0119 \\
%     BppAttack & 24.6 & \best{0.525} & \best{0.0196} & \best{8.97e-5} & \best{40.5} & \best{0.992} & \best{1.94e-4} & \best{0.150} & \best{99.2} & 0.0239 \\
%     Adap-Patch (train) & 22.5 & 2.06 & 0.315 & 1.53e-3 & 28.7 & 0.972 & 4.78e-3 & 0.296 & 95.2 & 9.43e-3 \\
%     Adap-Patch (test) & 74.1 & 6.77 & \worst{0.913} & 0.0151 & 18.2 & 0.956 & 0.0120 & 0.724 & 87.7 & 8.94e-3 \\
%     Adap-Blend (train) & 87.0 & 2.63 & 0.142 & 2.30e-3 & 26.4 & 0.903 & 0.0136 & 0.823 & 92.4 & 0.0336 \\
%     Adap-Blend (test) & 232 & 4.97 & 0.192 & 8.15e-3 & 20.9 & 0.783 & 0.0485 & 2.37 & 89.8 & 0.0831 \\
%     DFST & 487 & \worst{10.8} & 0.489 & \worst{0.0400} & \worst{14.0} & 0.719 & 0.165 & 2.22 & 88.6 & 0.316 \\
%     Narcissus (train) & 188 & 3.43 & 0.0627 & 3.83e-3 & 24.2 & 0.818 & 0.0545 & 1.44 & 91.8 & 0.101 \\
%     Narcissus (test) & \worst{542} & 9.98 & 0.188 & 0.0325 & 14.9 & \worst{0.532} & \worst{0.184} & \worst{3.68} & \worst{82.2} & \worst{0.331} \\
%     Grond & 87.6 & 1.62 & 0.0348 & 8.59e-4 & 30.7 & 0.934 & 2.92e-3 & 0.918 & 97.9 & 0.0833 \\
%     DFBA & 13.5 & 2.99 & 0.844 & 2.94e-3 & 25.3 & \best{0.992} & 1.66e-3 & 0.159 & 97.4 & 2.83e-3 \\
%     \bottomrule
%     \end{tabular}
% \end{table*}



% \begin{table*}[t]
%     \centering
%     \caption{Input-space stealthiness evaluation on CIFAR-100.}
%     \label{tab:cifar100-input-stealthiness}
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     Metric & $l_1$ & $l_2$ & $l_\infty$ & MSE & PSNR & SSIM & LPIPS & IS & pHash & SAM \\
%     Ideal value & 0 & 0 & 0 & 0 & $\infty$ & 1 & 0 & 0 & 100 & 0 \\
%     \midrule
%     BadNets & \best{13.3} & 2.91 & 0.839 & 2.79e-3 & 25.6 & 0.955 & 5.39e-3 & 0.182 & 94.1 & \best{1.66e-3} \\
%     Blend & 232 & 4.98 & 0.191 & 8.23e-3 & 20.8 & 0.765 & 0.0512 & \worst{2.25} & 89.0 & 0.0876 \\
%     WaNet & 55.3 & 1.64 & 0.177 & 9.55e-4 & 30.2 & 0.968 & 6.72e-3 & 0.308 & 95.2 & 0.0154 \\
%     BppAttack & 24.3 & \best{0.520} & \best{0.0196} & \best{8.83e-5} & \best{40.5} & 0.991 & \best{2.06e-4} & \best{0.138} & \best{99.1} & 0.0235 \\
%     Adap-Patch (train) & 22.7 & 2.09 & 0.320 & 1.59e-3 & 28.5 & 0.971 & 4.78e-3 & 0.297 & 94.4 & 9.51e-3 \\
%     Adap-Patch (test) & 74.5 & 6.96 & \worst{0.928} & 0.0159 & 18.0 & 0.956 & 0.0135 & 0.805 & 86.2 & 9.73e-3 \\
%     Adap-Blend (train) & 87.9 & 2.66 & 0.142 & 2.36e-3 & 26.3 & 0.894 & 0.0144 & 0.796 & 91.5 & 0.0356 \\
%     Adap-Blend (test) & 234 & 5.02 & 0.192 & 8.36e-3 & 20.8 & 0.764 & 0.0513 & \worst{2.25} & 89.0 & 0.0877 \\
%     DFST & 509 & \worst{11.3} & 0.495 & \worst{0.0444} & \worst{13.5} & 0.708 & \worst{0.169} & 2.16 & 87.7 & 0.312 \\
%     Narcissus (train) & 174 & 3.27 & 0.0627 & 3.50e-3 & 24.6 & 0.884 & 0.0147 & 0.622 & 94.3 & 0.126 \\
%     Narcissus (test) & \worst{528} & 9.82 & 0.188 & 0.0315 & 15.0 & \worst{0.630} & 0.166 & 2.22 & \worst{84.6} & \worst{0.347} \\
%     Grond & 86.9 & 1.61 & 0.0347 & 8.50e-4 & 30.7 & 0.929 & 4.97e-3 & 0.876 & 97.9 & 0.0720 \\
%     DFBA & 13.5 & 3.02 & 0.843 & 3.04e-3 & 25.2 & \best{0.993} & 7.74e-3 & 0.146 & 95.9 & 4.18e-3 \\
%     \bottomrule
%     \end{tabular}
% \end{table*}



% \begin{table*}[t]
%     \centering
%     \caption{Input-space stealthiness evaluation on Imagenette.}
%     \label{tab:imagenette-input-stealthiness}
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     Metric & $l_1$ & $l_2$ & $l_\infty$ & MSE & PSNR & SSIM & LPIPS & IS & pHash & SAM \\
%     Ideal value & 0 & 0 & 0 & 0 & $\infty$ & 1 & 0 & 0 & 100 & 0 \\
%     \midrule
%     BadNets & 73.3 & 6.94 & 0.879 & 2.54e-3 & 26.0 & 0.981 & 0.0152 & 0.0331 & 97.2 & 1.44e-3 \\
%     Blend & 1.62e-3 & 13.8 & 0.198 & 0.0100 & 20.0 & 0.697 & 0.203 & 3.10 & 89.9 & 0.0968 \\
%     WaNet & 225 & 2.94 & 0.190 & 4.94e-4 & 33.3 & 0.981 & 0.0140 & 0.0775 & 98.0 & 0.0111 \\
%     BppAttack & 151 & \best{1.30} & \best{0.0196} & \best{8.79e-5} & \best{40.6} & 0.983 & \best{1.87e-3} & 0.0990 & 99.4 & 0.0294 \\
%     Adap-Patch (train) & 136 & 5.18 & 0.342 & 1.54e-3 & 28.2 & 0.967 & 0.0229 & 0.175 & 94.7 & 0.0101 \\
%     Adap-Patch (test) & 424 & 16.7 & \worst{0.960} & 0.0147 & 18.4 & 0.955 & 0.0540 & 0.238 & 86.9 & 9.00e-3 \\
%     Adap-Blend (train) & 615 & 7.35 & 0.147 & 2.87e-3 & 25.4 & 0.865 & 0.0769 & 0.844 & 92.0 & 0.0413 \\
%     Adap-Blend (test) & 1.64e3 & 13.9 & 0.198 & 0.0102 & 19.9 & 0.697 & 0.203 & 3.09 & 89.9 & 0.0969 \\
%     DFST & 3.22e3 & \worst{28.9} & 0.532 & \worst{0.0456} & \worst{13.5} & 0.692 & 0.335 & 1.52 & 88.1 & \worst{0.334} \\
%     Narcissus (train) & 1.17e3 & 8.55 & 0.0627 & 3.81e-3 & 24.2 & 0.861 & 0.113 & 0.669 & 93.4 & 0.139 \\
%     Narcissus (test) & \worst{3.31e3} & 24.6 & 0.188 & 0.0317 & 15.0 & \worst{0.615} & \worst{0.428} & \worst{3.37} & \worst{82.8} & 0.268 \\
%     Grond & 476 & 3.66 & 0.0352 & 7.00e-4 & 31.6 & 0.882 & 0.0482 & 1.02 & 99.1 & 0.0521 \\
%     DFBA & \best{13.5} & 3.05 & 0.855 & 4.90e-4 & 33.1 & \best{0.999} & 2.07e-3 & \best{0.0312} & \best{99.8} & \best{8.93e-4} \\
%     \bottomrule
%     \end{tabular}    
% \end{table*}



% \begin{table*}[t]
%     \centering
%     \caption{Input-space stealthiness evaluation on Tiny-ImageNet.}
%     \label{tab:tiny-input-stealthiness}
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     Metric & $l_1$ & $l_2$ & $l_\infty$ & MSE & PSNR & SSIM & LPIPS & IS & pHash & SAM \\
%     Ideal value  & 0 & 0 & 0 & 0 & $\infty$ & 1 & 0 & 0 & 100 & 0 \\
%     \midrule
%     BadNets & 58.36 & 4.99 & 0.73 & 2.23e-03 & 26.53 & 0.96 & 4.15e-02 & 0.11 & 91.79 & 3.47e-03\\
%     Blend & 921.81 & 9.95 & 0.2 & 8.22e-03 & 20.85 & 0.81 & 0.11 & 1.11 & 89.44 & 0.11\\
%     WaNet & 317.02 & 4.94 & 0.35 & 2.20e-03 & 26.58 & 0.93 & 4.03e-02 & 0.27 & 97.35 & 2.60e-02\\
%     BppAttack & 96.26 & \best{1.04} & \best{1.96e-02} & \best{8.76e-05} & \best{40.57} & 0.99 & \best{8.75e-04} & 9.75e-02 & 99.42 & 3.14e-02\\
%     Adap-Patch (train) & 23.54 & 2.17 & 0.33 & 4.22e-04 & 34.22 & 0.99 & 2.56e-03 & 5.07e-02 & 96.93 & 2.93e-03\\
%     Adap-Patch (test) & 75.68 & 7.06 & \worst{0.96} & 4.11e-03 & 23.87 & 0.99 & 8.12e-03 & 0.17 & 92.05 & 3.05e-03\\
%     Adap-Blend (train) & 358.75 & 5.45 & 0.15 & 2.47e-03 & 26.07 & 0.91 & 4.19e-02 & 0.49 & 91.8 & 4.67e-02\\
%     Adap-Blend (test) & 955.04 & 10.28 & 0.2 & 8.77e-03 & 20.58 & 0.79 & 0.13 & 1.42 & 89.21 & 0.11\\
%     DFST & 1.97e+03 & 22.16 & 0.53 & 4.18e-02 & 13.83 & 0.68 & 0.32 & 1.72 & 87.87 & 0.31\\
%     Narcissus (train) & 1.23e+03 & 12.1 & 0.2 & 1.19e-02 & 19.23 & 0.65 & 0.22 & 1.55 & 85.56 & 0.26\\
%     Narcissus (test) & \worst{3.29e+03} & \worst{33.31} & 0.59 & \worst{9.05e-02} & \worst{10.43} & \worst{0.36} & \worst{0.56} & \worst{4.73} & \worst{70.98} & \worst{0.5}\\
%     Grond & 671.95 & 6.31 & 6.67e-02 & 3.25e-03 & 24.89 & 0.8 & 0.16 & 1.68 & 96.83 & 0.17\\
%     DFBA & \best{13.34} & 3.01 & 0.87 & 7.49e-04 & 31.26 & \best{0.99} & 2.09e-03 & \best{4.42e-02} & \best{99.59} & \best{1.34e-03}\\
%     \bottomrule
%     \end{tabular}
% \end{table*}

==> sections/introduction.tex <==
\definecolor{ogreen}{RGB}{55,126,34}
\begin{figure}[t]
\centering
\includegraphics[width = 1\linewidth]{./img/3space_visualization_bar.pdf}
\caption{The visualization of backdoor stealthiness by selected metrics in input space, feature space, and parameter space. The values are normalized. The larger the value, the less stealthy it is. Some of the attacks could achieve stealthiness in one space but fail in others. Only Grond~\cite{xu2025grond} is relatively stealthy in all three spaces.}
\label{fig:3space-bar-visualization}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width = 0.9\linewidth]{./img/iamgeNette_triggers.pdf}
\caption{Benign and 10 poisoned Imagenette images.}
\label{fig:imagenette-triggers}
\end{figure}

\section{Introduction}
\label{sec:introduction}

Deep neural networks (DNNs) have demonstrated prominent success in performing complex tasks. However, they remain vulnerable to security threats such as backdoor attacks. These attacks compromise a model by embedding a secret functionality, often achieved through poisoning the training data with a predefined trigger~\cite{gu2019badnets,chen2017blend,nguyen2021wanet,wang2022bppattack}. Models trained on this poisoned data will exhibit normal behavior on benign inputs but will misclassify any input containing the trigger to an adversary-specified target class.
This poisoning process can be improved (to be more stealthy in feature space or requiring fewer poisoned samples) by asymmetric triggers~\cite{qi2023adap,zhu2024gradient,lin2025revisiting} between training and inference time, or amplifying the intensity of the trigger image~\cite{zeng2022narcissus}.
More powerful backdoor attacks with a more relaxed threat model can access the training process for implementing new loss functions~\cite{cheng2021dfst,mo2024ssdt,bypass2020tan}, or directly modify the network weights~\cite{hong2022handcraft,cao2024dfba}.

A primary objective of backdoor attacks is to evade detection by both humans and automated defenses. Early attacks utilizing visible triggers, such as the patterned square in BadNets~\cite{gu2019badnets} (see Figure~\ref{fig:imagenette-triggers}), are relatively easy to identify. To decrease the visibility of the backdoor trigger, WaNet~\cite{nguyen2021wanet} uses image warping to design invisible and dynamic triggers. 
Lira~\cite{doan2021lira} and BppAttack~\cite{wang2022bppattack} improve the invisible trigger by introducing a trigger generator or image quantization.
However, backdoored models tend to learn separate features, which can be easily detected~\cite{wang2022featurere}.
As a response, Adap-Patch/Blend~\cite{qi2023adap} weakens the feature separation by designing asymmetric triggers. 
Although recent backdoor attacks could achieve stealthiness in one space, they may fail in other spaces. Recent studies highlight this lack of comprehensive stealthiness. BAN~\cite{xu2024ban} finds that input-space-stealthy attacks may be less stealthy in feature space, while Grond~\cite{xu2025grond} notes that parameter-space stealthiness is often overlooked.

Consequently, a systematic evaluation of backdoor stealthiness across multiple spaces is lacking.
Prior work suggests evaluating the comprehensive stealthiness through different types of backdoor defense methods in different spaces~\cite{xu2025grond}. 
However, this paper adopts a complementary approach by analyzing stealthiness directly through distance and similarity metrics in the input, feature, and parameter spaces. 

% \textcolor{red}{This methodology is motivated by two factors. First, the metrics can help quantify the stealthiness and enable more intuitive comparison. Second, evaluating stealthiness indirectly through defense could suffer from fairness issues due to adaptive defenses or attacks~\cite{tramer2020adaptive}} 

\textbf{Scope of Evaluation:} It is crucial to clarify that our evaluation adopts an attacker-centric and red-teaming perspective, rather than a defensive operational one. While defenders in the wild typically lack access to the trigger or ground-truth poisoned samples~\cite{abad2025sok}, the evaluator (e.g., an attacker optimizing their method, or a researcher auditing an attack) inherently possesses white-box access to the trigger, training data, and model parameters. The metrics are designed to serve as stable, objective benchmarks for this "science of security", much like how PSNR requires the original image to evaluate compression quality even if the end-user does not possess it.
This methodology is motivated by two factors. First, unlike defense success rates, which are moving targets subject to the "arms race" of adaptive attacks~\cite{tramer2020adaptive}, quantitative metrics provide a stable mathematical baseline for comparing the fundamental quality of attacks. Second, these metrics allow attackers and auditors to quantify the exact "footprint" left by a backdoor in the model's weights and feature representations, regardless of whether a current defense exists to detect it.
For example, DFST involves minimizing the distance between activations from benign and backdoor neurons. While it improves the performance against defenses such as ABS~\cite{liu2019abs} and NC~\cite{wang2019nc} (RQ4 in~\cite{cheng2021dfst}), DFST exhibits poor feature space stealthiness in terms of Silhouette Score (SS) and discriminant Sliced-Wasserstein Distance (DSWD) (see feature space in Figure~\ref{fig:3space-bar-visualization}), suggesting its vulnerability to a defense specifically designed based on SS or DSWD.

To address this lack of a comprehensive evaluation of backdoor stealthiness, this paper presents a systematic analysis of quantitative stealthiness metrics, evaluating 10 backdoor attacks across four datasets 
%(CIFAR-10~\cite{krizhevsky2009cifar}, CIFAR-100~\cite{krizhevsky2009cifar}, Tiny-ImageNet~\cite{le2015tiny}, and Imagenette~\cite{deng2009imagenet}) 
and three model architectures. %(ResNet18~\cite{he2015resnets}, VGG16~\cite{simonyan2015vgg}, and ViT-Small~\cite{alexey2021vit}). 
Our empirical results indicate that even state-of-the-art attacks fail to achieve stealthiness across all spaces. Furthermore, based on the limitations identified in our analysis, we propose two novel metrics to better capture stealthiness: the Class-Specific Davies–Bouldin Index (CDBI) and the TAC–UCLC Product (TUP).

\textcolor{black}{\textbf{Differentiation from Prior Work.} While existing benchmarks like BackdoorBench~\cite{baoyuan2022bb} standardize attack implementation, they primarily focus on Attack Success Rate and detection by specific defenses. Other studies have investigated individual stealthiness aspects, such as input perceptibility~\cite{liu2022stealthiness} or latent separability~\cite{xu2025grond}. This work differs by (i) providing the first unified \textit{tri-space} analysis (Input, Feature, and Parameter); % across 10 attacks and 3 architectures; 
(ii) shifting the evaluation paradigm from defense-specific proxy metrics (which become obsolete as defenses evolve) to fundamental distance-based metrics; and (iii) proposing and statistically validating two novel metrics (CDBI and TUP) that capture stealthiness properties missed by standard measurements.}

Our contributions are summarized as follows:
\begin{compactitem}
    \item We conduct a review of the backdoor literature to provide an overview of the quantitative stealthiness metrics currently used in the research field.
    \item We use these metrics to systematically evaluate the stealthiness of 10 backdoor attacks: BadNets~\cite{gu2019badnets}, Blend~\cite{chen2017blend}, WaNet~\cite{nguyen2021wanet}, BppAttack~\cite{wang2022bppattack}, Adap-Patch/Blend~\cite{qi2023adap}, DFST~\cite{cheng2021dfst}, Narcissus~\cite{zeng2022narcissus}, Grond~\cite{xu2025grond}, and DFBA~\cite{cao2024dfba}. Our results indicate that, except for Grond, none of the attacks covers all aspects of backdoor stealthiness. However, in terms of trigger imperceptibility, Grond is outperformed by WaNet and BppAttack, which exclusively focus on input-space stealthiness.
    \item We assess the effectiveness of existing metrics and, informed by our findings, propose two novel stealthiness metrics. We demonstrate the utility of these proposed metrics by applying them to the evaluated attacks.
    \item We conduct a correlation analysis between backdoor defenses and stealthiness metrics, allowing us to identify which metrics indicate successful defense.
    \item We propose a novel tri-space stealthiness metric that aggregates the stealthiness contributions from all three domains into a single scalar score. 
\end{compactitem}


==> sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}

We faced four main limitations in our study. 
\textbf{First, the evaluation metrics themselves can bias the results.} Some feature- and parameter-space metrics look ``better'' when a backdoored model is simply less successful. In particular, DSWD (feature space) and TAC (parameter space) tend to give more favorable scores when the attack success rate (ASR) is low, because they are measured on poisoned or trigger-bearing data; this makes cross-attack comparisons harder when many models have low ASR. 
By contrast, UCLC is data-free and more stable, but TAC requires access to triggered inputs, which defenders typically do not have; as such, it is better suited for analysis than for realistic detection.
Moreover, some metrics depend on design choices such as the network layer used and the dimensionality-reduction method (e.g., t-SNE/ICA/PCA) before clustering, which can change the absolute values and rankings. 

\textbf{Second, our attack settings (especially poisoning rates) limit comparability.} Several models (e.g., BppAttack with $0.3\%$ PR) reached low ASR, which in turn affected their feature- and parameter-space scores.
In hindsight, a better protocol would set one common rate that yields high ASR for most attacks and then adjust a second rate per attack to probe sensitivity.
Implementation choices also matter: batch-wise ``rounding'' (when poisoning at very low rates), normalization, and small adjustments to triggers (size/placement) were necessary for reproducibility and fairness, but can still influence outcomes.
Dataset and preprocessing decisions (e.g., Imagenette cropped and downscaled to $80{\times}80$) and fixed training budgets could further constrain how results transfer to other scales or settings.

\textbf{Third, scope and external validity.} We focus on supervised image classification with CNN-centric metrics; current parameter-space metrics (UCLC/TAC) are not directly applicable to ViT, so we did not report parameter-space results for ViT models.
We also take a metric-based perspective instead of a defense-based one; while this avoids adaptivity biases (the bias one encounters when defenses are tuned to the specific attacks under test), it does not directly measure how detectable or removable backdoors are under deployed defenses or by humans. 

\textbf{Fourth, scope of Modality and Taxonomy.} We acknowledge that our current evaluation is concentrated on the image domain. While we note that certain backdoor defenses, such as STRIP and MNTD, are modality-agnostic, the vast majority of existing stealthiness metrics (e.g., LPIPS, SSIM) are inherently designed for visual data. As such, we consider the image domain analysis to provide the most immediate opportunities for a comprehensive, metric-based comparison. Furthermore, while our taxonomy focuses on Input, Feature, and Parameter spaces, we recognize that defenses like MNTD operate by detecting anomalies in the output Space (logits). We view output anomalies as downstream manifestations of feature and parameter irregularities, but we suggest that future taxonomies could explicitly include the output space to characterize attacks that optimize for logit stealthiness.

Overall, these constraints suggest caution in reading across datasets and attacks; future work should calibrate poisoning rates to ensure comparable ASR, add metrics that decouple from ASR and work for non-CNNs, and pair metric-based evaluation with standardized defenses and, where relevant, human perception checks.



% \section{More On Background}
% \label{sec:app:background}

% \subsection{Neural Networks}
% \label{subsec:dnns}

% We model an image classifier as a deep neural network \(\model:\mathbb{R}^{3\times h\times w}\!\to\!\mathbb{R}^{|\mathcal{C}|}\) that maps an RGB image \(x\) to class logits \(z=\model(x)\); the prediction is \(\hat y=\arg\max_{c\in\mathcal{C}} z_c\). Parameters \(\theta\) (weights and biases) are learned by empirical loss minimization on labeled data \(\{(x_i,y_i)\}_{i=1}^N\) with mini-batch SGD and backpropagation, typically using ReLU activations and regularization such as weight decay, batch normalization, and data augmentation. We minimize cross-entropy $H(.)$ between the one-hot label \(p_{y_i}\) and the softmax of the logits: 
% \[\theta^\star=\arg\min_\theta \frac{1}{N}\sum_{i=1}^N H\!\big(p_{y_i},\,\mathrm{softmax}(\model(x_i))\big).\] 

% For images, we consider two architecture families. (i) \textbf{CNNs:} small learnable filters convolve over local patches and are shared across the image; this weight sharing induces (approximate) translation equivariance, while pooling or strides reduce spatial resolution. (ii) \textbf{Vision Transformers (ViT):} the image is split into non-overlapping \(P{\times}P\) patches, linearly projected to token embeddings (plus a [CLS] token), augmented with positional encodings, and processed by multi-head self-attention and MLP blocks; global token–token interactions are learned (no built-in equivariance), and the [CLS] representation is mapped to logits. These architectures constitute the baseline on which we study backdoor mechanisms and the stealthiness metrics that follow.




% \section{Additional Related Work}
% \label{sec:app:related_work}

% \subsection{Input-space Stealthiness}
% \label{sec:related_work:stealthiness:input}

% Early attacks such as BadNets~\cite{gu2019badnets} use visible patch triggers, making poisoned images easy to spot by inspection or by inference-time input screening (e.g., STRIP~\cite{gao2020strip}). STRIP identifies backdoors by superimposing input images with clean samples; consistently low entropy in predictions across blended inputs indicates a trigger's presence. Subsequent attacks pursued imperceptibility. WaNet~\cite{nguyen2021wanet}, Lira~\cite{doan2021lira}, BppAttack~\cite{wang2022bppattack}, among others, design invisible triggers by image processing techniques (image warping, quantization) or train a generator to find the optimal trigger, yielding small per-pixel changes but strong attack effectiveness.
% % the authors report that WaNet often evades both manual checks and STRIP-like screening. 
% These works established that input-space stealthiness is achievable and input-only defenses will miss sufficiently subtle triggers.

% \subsection{Feature-space Stealthiness}
% \label{sec:related_work:stealthiness:feature}

% Although poisoned images may appear visually indistinguishable from clean ones, they can often be separated in the model’s latent space. Activation Clustering (AC)~\cite{chen2018ac} exploits this property by embedding activations, typically after dimensionality reduction, and identifying the presence of two clusters within a class, which indicates a target-class backdoor. This vulnerability has motivated the development of attacks that explicitly reduce latent separability. For instance, Qi et al. introduced Adap-Patch and Adap-Blend~\cite{qi2023adap}, which weaken the association between triggers and target classes such that triggered features more closely overlap with benign features, thereby evading AC in multiple settings. Similarly, WaNet and the adaptive attacks highlight an inherent trade-off: achieving stealthiness in the input space does not necessarily imply stealthiness in the feature space, and vice versa. Complementary research has investigated feature-space stealthiness under relaxed threat models, where tailored loss functions are designed to minimize the distance between benign and backdoored features~\cite{doan2021dswd,bypass2020tan}.

% \subsection{Parameter-space Stealthiness}
% \label{sec:related_work:stealthiness:parameter}

% Parameter-space defenses ask whether a small subset of channels carries the backdoor. Channel Lipschitz–based Pruning (CLP)~\cite{zheng2022clp} estimates a per-channel upper bound on sensitivity (UCLC) and prunes the most sensitive channels without using any data; many input/feature-stealthy attacks still fail under CLP. Xu et al.~\cite{xu2025grond} argued that contemporary attacks are rarely evaluated against such defenses and introduced \emph{Grond}, trained with Adversarial Backdoor Injection (ABI), which penalizes or replaces overly sensitive channels during training to diffuse the trigger’s influence. Grond aims to couple parameter-space stealthiness with imperceptible triggers, and the authors reported that the resulting models also resist several feature-space detectors, suggesting that strong parameter- and input-space stealthiness can induce feature-space stealthiness.

==> sections/new_metrics.tex <==

\renewcommand{\arraystretch}{0.7}
\begin{table}[t]
\scriptsize
\centering
\caption{Stealthiness evaluation of backdoored ResNet18 models trained on four datasets, with the two metrics proposed in this study: 
the Davies-Bouldin index (DBI) and TAC-UCLC product (TUP). For the former metric, 0 is the worst possible measurement, whereas it is the ideal value for the latter metric. For each metric and dataset, the \best{best} and \worst{worst} results are highlighted. Results that may be affected by the low ASR of the corresponding models (see Table~\ref{tab:attack-performance-4datasets}) are \underline{underlined}. *The poisoning rates vary per dataset.}
\label{tab:results_newmetric_resnet18}
\setlength\tabcolsep{1pt}
\begin{tabular}{l c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{PR (\%)} 
& \multicolumn{2}{c}{C10} 
& \multicolumn{2}{c}{C100} 
& \multicolumn{2}{c}{Tiny} 
& \multicolumn{2}{c}{Imagenette} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& & CDBI$\uparrow$ & TUP$\downarrow$ & CDBI$\uparrow$ & TUP$\downarrow$ & CDBI$\uparrow$ & TUP$\downarrow$ & CDBI$\uparrow$ & TUP$\downarrow$\\
\midrule

    \multirow{2}{*}{BadNets} & 5 & 0.574 & 16.2 & 0.424 & 27.7 & 0.646 & 10.227 & \worst{0.418} & 18.4 \\

    & 0.3 & 0.627 & \worst{23.1} & 0.534 & 29.6 & 0.624 & 3.895 & 0.871 & \worst{19.3} \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{Blend} & 5 & 0.738 & 3.68 & 0.620 & 10.2 & 0.53 & 3.885 & 3.07 & 3.30 \\

    & 0.3 & 0.796 & 3.94 & 0.911 & 10.8 & 0.576 & 3.407 & 2.20 & 2.77 \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{WaNet} & 5 & 0.641 & 9.30 & 0.409 & 25.4 & 0.523 & 7.078 & 0.571 & 8.85 \\

    & 2/0.3/0.3/0.3$^*$ & 0.644 & 8.56 & 1.54 & 22.1 & 1.377 & 3.657 & 0.809 & 3.84 \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{Bpp} & 5 & 0.640 & 21.0 & 0.477 & 52.4 & 0.584 & \worst{34.275} & 0.518 & 13.9 \\

    & 2/0.3/0.3/0.3$^*$ & 0.519 & 10.9 & 0.436 & \worst{56.1} & \underline{0.637} & \underline{3.578} & \underline{0.854} & \underline{1.56} \\
    \cmidrule(lr){2-10}

    \multirow{2}{1cm}{Adap\\Patch} & 5 & \underline{1.29} & \underline{8.38} & 1.19 & 13.4 & \best{\underline{1.841}} & \underline{3.522} & \underline{2.90} & \underline{5.72} \\

    & 0.3 & 3.42 & 10.2 & \underline{2.27} & \underline{9.77} & \underline{0.622} & \underline{3.495} & \underline{4.45} & \underline{2.35} \\
    \cmidrule(lr){2-10}

    \multirow{2}{1cm}{Adap\\Blend} & 5 & \underline{1.66} & \underline{3.34} & 1.24 & 9.93 & 0.916 & 3.209 & 3.00 & 3.29 \\

    & 0.3 & 5.19 & 3.63 & 1.53 & 11.2 & 0.497 & 3.451 & \underline{12.3} & \underline{2.45} \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{DFST} & 5 & 0.650 & 3.70 & 0.475 & 8.91 & 0.475 & \best{3.063} & 0.476 & 3.81 \\

    & 0.3 & \worst{0.550} & 4.47 & \worst{0.260} & 11.1 & \worst{0.353} & 3.093 & 0.934 & 4.43 \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{Narcissus} & 5/0.7/0.4/5$^*$ & 0.767 & 2.15 & 3.47 & 8.75 & 1.107 & 3.192 & 4.27 & 2.64 \\

    & 0.3 & \best{5.92} & 2.13 & \best{\underline{4.34}} & \best{\underline{8.48}} & 1.434 & 3.25 & \underline{7.54} & \underline{2.13} \\
    \cmidrule(lr){2-10}

    \multirow{2}{*}{Grond} & 5/0.7/0.4/5$^*$ & 0.868 & 1.87 & \underline{1.95} & \underline{8.86} & 1.074 & 3.236 & \best{24.0} & 1.61 \\

    & 0.3 & 5.81 & \best{1.78} & \underline{1.53} & \underline{8.64} & 1.19 & 3.368 & \underline{12.4} & \best{\underline{1.05}} \\
    \cmidrule(lr){2-10}

    DFBA & - & - & 10.2 & - & 10.6 & - & 3.917 & - & 13.5 \\
\bottomrule
\end{tabular}
\end{table}


\section{Improving the Current Stealthiness Metrics}
\label{sec:new_metrics}

In Section~\ref{sec:experimental_results}, we found that feature-space and parameter-space metrics have certain shortcomings that make it more difficult to compare the stealthiness of attacks. Although this is also the case for the input-space metrics, their large number allows the issue to be mitigated more easily by employing multiple metrics that cover each other’s weaknesses. For both feature and parameter space, we propose improvements to (some of) the existing metrics, to address their shortcomings and encourage the consideration of comprehensive stealthiness in future backdoor research.

\subsection{Class-Specific Davies–Bouldin Index (CDBI)}
\label{sec:new_metrics:cdbi}

\textbf{Motivation.} Silhouette Score (SS) on t-SNE embeddings can disagree with visual separability when (i) clean vs.\ triggered clusters are highly imbalanced (different poisoning rates) and/or (ii) triggered points are split by original class, weakening within-cluster cohesion. We replace SS by the Davies-Bouldin Index~\cite{davies1979dbi}, and make the metric class-specific to reduce these issues.

\textbf{Definition.} Fix a target class \(t\) and a source class \(p\).
Given an embedding \(Z=\{z_i\}\), let \(\mathcal{B}\) be the set of embedded
benign samples of class \(t\) and \(\mathcal{P}\) the set of embedded
poisoned samples originating from source class \(p\) (aiming at \(t\)).
For two clusters, the class-conditional DBI is
\begin{align*}
\mathrm{DBI}_{t,p} &= 
   \frac{S(\mathcal{B}) + S(\mathcal{P})}{M(\mathcal{B},\mathcal{P})}, \\
S(\mathcal{A}) &= \frac{1}{|\mathcal{A}|} \sum_{z\in\mathcal{A}}\|z-\mu_{\mathcal{A}}\|_2, \\
M(\mathcal{B},\mathcal{P}) &= \|\mu_{\mathcal{B}}-\mu_{\mathcal{P}}\|_2,
\end{align*}
where \(\mu_{\mathcal{A}}\) is the centroid of \(\mathcal{A}\).
We then average over source classes:
\[
\mathrm{CDBI} \;=\; \frac{1}{|\mathcal{P}_{\text{src}}|}\sum_{p\in\mathcal{P}_{\text{src}}}\mathrm{DBI}_{t,p}.
\]
Orientation: lower \(M\) (centroids close) or larger \(S\) (diffuse clusters) increases DBI. Thus, \(\mathrm{CDBI}\,\uparrow\) indicates more overlap (more stealthy in feature space), and \(\mathrm{CDBI}\,\downarrow\) indicates clearer separation.

\textbf{Procedure.}
(i) Fix a target class \(t\) and extract penultimate-layer features for all training samples of class \(t\);
(ii) split them into two sets: \(\mathcal{B}\) (benign/clean) and \(\mathcal{P}_{\text{src}}\) (poisoned samples originating from source class \(p\));
(iii) embed features with t-SNE using fixed seed and perplexity;
(iv) for each \(p\in\mathcal{P}_{\text{src}}\), compute \(\mathrm{DBI}_{t,p}\) with \texttt{sklearn.metrics.davies\_bouldin\_score} over the two clusters \((\mathcal{B},\mathcal{P})\);
(v) report \(\mathrm{CDBI}=\frac{1}{|\mathcal{P}_{\text{src}}|}\sum_{p\in\mathcal{P}_{\text{src}}}\mathrm{DBI}_{t,p}\).

\textbf{Why this helps.} DBI depends on relative scatter vs.\ centroid distance and is less biased by cluster-size imbalance than SS; evaluating per class restores cohesion (triggered points of the same class group naturally), making the score track the visual class-conditional overlap seen in t-SNE plots. We specifically aggregate the class-specific scores by taking their average, instead of, e.g., the median, so that all poisoned samples count towards the stealthiness score. This reflects the fact that a defender with access to the training dataset could use any poisoned sample to detect the backdoor.

\subsection{TAC–UCLC Product (TUP)}
\label{sec:new_metrics:tup}

\textbf{Motivation.} TAC measures trigger-driven activation change per channel (data-dependent, informative but not defense-side); UCLC upper-bounds downstream sensitivity per channel (data-free, usable by defenses but can be loose).
% \textcolor{red}{We combine them so a channel counts only if it is both trigger-sensitive and high-impact}. 
We combine the two metrics by multiplying them in a channel-wise manner. This way, a channel achieves a high TUP measurement only if it has both high TAC, meaning it is sensitive to the trigger, and high UCLC, meaning it can be detected in defense scenarios.

\textbf{Per-channel quantities.} Let $a^{(\ell)}_j(x)\in\mathbb{R}^{H\times W}$ and $\hat{a}^{(\ell)}_j(x)\in\mathbb{R}^{H\times W}$ denote the post-activation feature maps of channel $j$ at the last convolutional layer $\ell$ for the benign model $f$ and the backdoored model $\hat{f}_\theta$, respectively.
 For a poisoning insertion operator \(\mathcal{T}\), compute:
\begin{align*}
\mathrm{TAC}^{\text{bkd}}_j &= 
   \mathbb{E}_{x}\,\big\|\hat{a}^{(\ell)}_j(\mathcal{T}(x)) - \hat{a}^{(\ell)}_j(x)\big\|_{2}, \\
\mathrm{TAC}^{\text{ben}}_j &= 
   \mathbb{E}_{x}\,\big\|a^{(\ell)}_j(\mathcal{T}(x)) - a^{(\ell)}_j(x)\big\|_{2}.
\end{align*}

$\mathrm{TAC}^{\text{bkd}}_j$ and $\mathrm{TAC}^{\text{ben}}_j$ are computed using the same (normalized) pipeline and the same image set, and then sorted in ascending order. Their ratio is defined as:
\[
R_j \;=\; \frac{\mathrm{TAC}^{\text{bkd}}_j}{\mathrm{TAC}^{\text{ben}}_j}.
\]

Let \(\mathrm{UCLC}_j\ge 0\) be the per-channel Lipschitz upper bound without layer-wise normalization (we evaluate only at layer \(\ell\)).

\textbf{Definition (TUP).}
\begin{align*}
\mathrm{TUP}_j          &= R_j \cdot \mathrm{UCLC}_j, \\
\mathrm{TUP}_{\text{mean}}   &= \tfrac{1}{C}\sum_{j=1}^{C}\mathrm{TUP}_j.
\end{align*}

Orientation: lower values indicate greater parameter-space stealthiness (no channels that are both highly trigger-sensitive and high-impact).

\textbf{Procedure.} (i) Fix the last conv layer; (ii) compute \(\mathrm{TAC}^{\text{ben}}\) and \(\mathrm{TAC}^{\text{bkd}}\) over the same held-out set (two forward passes per image); (iii) compute per-channel \(\mathrm{UCLC}\) by multiplying downstream operator norms; (iv) form \(R_j\), then \(\mathrm{TUP}_j\); (v) report \(\mathrm{TUP}_{\text{mean}}\).

\textbf{Why this helps.} UCLC is data-free and can therefore be used by defenders, but it can flag many channels that are merely high-gain (false positives). TAC gives a confident indication of trigger sensitivity, but also depends on trigger magnitude and ASR. However, the ratio \(R_j\) cancels the influence of trigger magnitude shared by benign/backdoored models. By taking the product of the two metrics, TUP flags only the channels that can be detected by defenders and are truly sensitive to the trigger.

\subsection{Evaluation of the Developed Metrics} 
\label{sec:new_metrics:results}

We report CDBI (higher is more stealthy) and TUP (lower is more stealthy) results in Table~\ref{tab:results_newmetric_resnet18}.

\subsubsection{CDBI vs.\ SS (does CDBI behave as intended?)}
CDBI reduces two issues we observed with the Silhouette Score (SS).  
(i) Poisoning-rate bias: On CIFAR-10, BadNets at 5\% vs.\ 0.3\% PR shows a small CDBI gap (0.574 vs.\ 0.627), whereas SS widens the gap (0.507 vs.\ 0.355), aligning better with the nearly unchanged visual overlap in t-SNE embeddings (see Figure~\ref{fig:cifar-tsne}). DFST shows a similar effect (0.650 vs.\ 0.550 in CDBI, versus 0.519 vs.\ 0.339 in SS).  
(ii) Class-splitting of poisoned points: When poisoned samples split into class-specific subclusters (e.g., WaNet at 5\% PR), the SS penalizes their weak within-cluster cohesion; CDBI focuses on class-conditional separation and therefore down-weighs such fragmented cases. On CIFAR-10, WaNet-5\% (0.641) ranks below Blend-5\% (0.738) under CDBI, reversing SS’s preference for WaNet and matching the t-SNE impression that WaNet’s poisoned points form multiple sub-groups.


\subsubsection{CDBI across datasets}
For CIFAR-10, the top CDBI comes from clean-label, low-PR attacks: Narcissus-0.3\% (5.92) and Grond-0.3\% (5.81). DFST-0.3\% is the least stealthy (0.550).  
For CIFAR-100, Narcissus-0.3\% leads (4.34, ASR 33.1\%), followed by Adap-Patch-0.3\% (2.27, ASR 2.98\%). DFST-0.3\% is the lowest (0.260). The high CDBI for low-ASR clean-label attacks matches intuition: scarce triggered points overlap more with clean features.  

For Tiny-ImageNet, CDBI values compress near 0.3–1.4 across methods, indicating harder feature-space hiding on the 200-class task. Adap-Patch-5\% is the best (1.841, ASR 41.62), while DFST attains the worst CDBI among feasible PRs (0.353 at 0.3\%). 
For Imagenette, Grond-5\% achieves the largest CDBI (24.0), reflecting strong interleaving of triggered and clean features; Adap-Blend-0.3\% and Grond-0.3\% are also high (12.3, 12.4). BadNets-5\% is lowest (0.418).

Across all four datasets, CDBI (i) reduces poisoning-rate bias relative to SS, and (ii) penalizes class-fragmented triggered clusters, yielding rankings that align with t-SNE visual embeddings. Its ``higher is stealthier'' orientation also makes interpretation straightforward across datasets.

\subsubsection{TUP vs.\ UCLC \& TAC}
The TUP metric is designed to improve upon UCLC by focusing on the neurons in a backdoored model that are truly sensitive to the trigger, as measured by their TAC relative to a benign model. As shown in Table~\ref{tab:uclc-tac}, the models backdoored by Grond consistently achieve low UCLC and TAC in our evaluation. Therefore, we would expect this attack to also have low TUP measurements. Indeed, we observe that the models backdoored by Grond achieve among the lowest measurements on all four datasets

In Section~\ref{subsec:parameter-space-stealthiness}, we found that TAC has a strong correlation with ASR, while UCLC does not. This makes the former metric less effective than the latter when comparing backdoored models with varying attack success rates. We observe that TUP seems more robust against low ASR than TAC; the best TUP measurement is achieved by a backdoored model with an ASR below 60\% for only two of the four datasets, whereas TAC prefers such models for all four of the datasets. 

Concerning the models with the worst measurement, we notice an interesting difference between TUP and the two metrics it is based on. For all datasets, DFBA achieves the worst TAC and UCLC measurements, but the TUP metric considers multiple backdoored models to be significantly less stealthy. TUP takes the average measurement over all neurons in a single layer, so DFBA has an advantage for this metric since it only modifies a single neuron per layer. However, this is not the only reason for DFBA's relatively low TUP measurement. While experimenting with the metric, we found that the UCLC of the neuron modified by DFBA is lower than the layer's average. This indicates that the neurons responsible for DFBA's high UCLC measurements are not located in the layer examined by TUP. Therefore, the TUP metric could be improved further by considering the TAC and UCLC in all layers, instead of just a single layer.

\subsubsection{TUP across datasets} 
For CIFAR-10, Grond-0.3\% (1.78) and Grond-5\% (1.87) achieve the lowest TUP, which makes sense when considering the attack's focus on parameter-space stealthiness. BadNets-0.3\% is the least stealthy (23.1). 
For CIFAR-100, Grond-0.3\% (8.64) and Grond-5\% (8.86) again have good results, but are respectively outperformed by Narcissus-0.3\% (8.48) and Narcissus-5\% (8.75). BppAttack-0.3\% achieves the worst measurement (56.1).

For Tiny-ImageNet, nearly all backdoored models achieve a TUP measurement between 3 and 4, which could be explained by many UCLC and TAC measurements also being similar on this dataset. DFST-5\% (3.063) is considered the stealthiest, whereas the measurement of BppAttack-5\% (34.275) is significantly worse than the others.
Finally, the measurements for Imagenette are similar to CIFAR-10; Grond-0.3\% (1.05) and Grond-5\% (1.61) are stealthiest, while BadNets-0.3\% achieves the worst measurement (19.3).
 



% \subsection{\textcolor{blue}{Practical Application: A Unified Decision Framework}}
% \label{sec:practical_application}
% \textcolor{blue}{
% While this work primarily focuses on the \textit{characterization} and \textit{measurement} of backdoor stealthiness, we acknowledge the practical need for a binary ``Go/No-Go'' decision or a scalar ranking in red-teaming scenarios. Although the implementation and rigorous evaluation of a full detection system remain outside the scope of this study, we propose a \textbf{conceptual framework} to demonstrate how these metrics could be integrated into a unified decision process in future research.}

% \textcolor{blue}{
% \textbf{Composite Stealthiness Score.}
% For automated benchmarking, an evaluator can define a composite "Stealthiness Score" ($S$) as a weighted ensemble of representative metrics from each space. For example, combining LPIPS (Input), CDBI (Feature), and TUP (Parameter):
% \begin{equation}
%     S = w_{in} \cdot (1 - \overline{\text{LPIPS}}) + w_{feat} \cdot \overline{\text{CDBI}} + w_{par} \cdot \frac{1}{\overline{\text{TUP}}}
% \end{equation}
% where $w$ represents the weights assigned based on the specific threat model (e.g., a scenario with heavy human inspection would increase $w_{in}$).
% }

% \textcolor{blue}{
% \textbf{Threshold-based Auditing.}
% Alternatively, for security auditing, the metrics serve as a "logical AND" gate. To be considered \textit{comprehensively stealthy}, an attack must satisfy stealthiness thresholds across all three dimensions simultaneously. An auditor may flag a model for manual inspection if \textit{any} single metric violates its safety bound:
% \begin{equation}
%     \text{Flag if } (\text{TUP} > \tau_{par}) \lor (\text{CDBI} < \tau_{feat}) \lor (\text{LPIPS} > \tau_{in})
% \end{equation}
% where $\tau$ are empirically derived thresholds (e.g., based on benign model baselines). This framework allows attackers to optimize their methods against a concrete "comprehensive" standard, rather than optimizing for a single metric (like LPIPS) while leaving a "loud footprint" in the parameter space (high TUP).  We suggest this threshold-based approach as a promising direction for developing robust, metric-driven backdoor detection systems.
% }







==> sections/recommendations_new.tex <==
\section{Recommendations and Limitations}
\label{sec:recommendations_limitations}



==> sections/stealth_metrics.tex <==
% notation: clean image and its triggered counterpart
\newcommand{\beni}{x}
\newcommand{\adv}{\mathcal{T}(x)}

\section{Stealthiness Metrics}
\label{sec:stealthiness_metrics}
 %This section reviews the metrics used in prior work to quantify each of these aspects. 
 We use \(\beni\) for a benign image and \(\adv\) for its triggered counterpart, \backdooredModel{} for the backdoored model, \(\phi(\cdot)\) for a chosen latent representation, and \(\mathcal{C}\) for the class set. 

\subsection{Input-space Stealthiness Metrics}
\label{sec:current_metrics:input}
Measure how imperceptible the trigger is to humans or simple input-screening defenses by quantifying the difference between \(\beni\) and \(\adv\).

\subsubsection{\boldmath\( l_p \) norms}
The basic proxies are \(l_p\) distances between images (flattened to vectors), e.g.,
\[
\|\beni-\adv\|_p
=
\left(\sum_i |\,\beni_i-\adv_i\,|^p\right)^{\!1/p},\quad p\in\{1,2,\infty\}.
\]
They are simple and model-free. They do not account for spatial structure or human perception; small, localized triggers can have low \(l_2\) but be visually obvious, and vice versa.

\subsubsection{Mean Squared Error (MSE)}
\[
\mathrm{MSE}(\beni,\adv)=\tfrac{1}{n}\sum_{i=1}^n(\beni_i-\adv_i)^2.
\]
Equivalent to squared \(l_2\), that is scaled by $\tfrac{1}{n}$. Easy to compute but shares the same perceptual limitations.

\subsubsection{Peak Signal-to-Noise Ratio (PSNR)}
\[
\mathrm{PSNR}(\beni,\adv)=10\log_{10}\!\left(\frac{\mathrm{MAX}^2}{\mathrm{MSE}(\beni,\adv)}\right),
\]
with \(\mathrm{MAX}=255\) for 8-bit images. Higher is ``better'' (more similar). Since PSNR is a monotone transform of MSE, the former metric inherits the latter's weaknesses.

\subsubsection{Structural SIMilarity (SSIM)}
\label{sec:current_metrics:input:ssim}
SSIM~\cite{wang2004ssim} compares local statistics over sliding windows. For windows \(x,\,y\),
\[
\mathrm{SSIM}(x,y)=
\frac{(2\mu_x\mu_y+C_1)(2\sigma_{xy}+C_2)}
     {(\mu_x^2+\mu_y^2+C_1)(\sigma_x^2+\sigma_y^2+C_2)},
\]
and the image-level score averages window scores. It tracks luminance, contrast, and structure, correlating better with human perception than pixel-wise metrics. It is sensitive to small misalignments and window choices.

\subsubsection{Perceptual Hash (pHash)}
The DCT-based pHash converts the image to grayscale, downsamples, keeps low frequencies via DCT, and then binarizes each coefficient by the median. The “pHash similarity” between \(\beni\) and \(\adv\) is
\[
\mathrm{pHash_{sim}} = \Big(1-\tfrac{d(\mathrm{pHash}(\beni),\,\mathrm{pHash}(\adv))}{64}\Big)\cdot 100\%,
\]
where \(d\) is Hamming distance. Liao et al.~\cite{liao2018backdoorembedding} used it to evaluate the stealthiness of their backdoor attack.

\subsubsection{LPIPS}
LPIPS~\cite{zhang2018lpips} compares deep features from a fixed, \emph{external} network:
\[
\mathrm{LPIPS}(\beni,\adv)=\sum_{\ell} w_\ell\,\big\|\hat\phi_\ell(\beni)-\hat\phi_\ell(\adv)\big\|_2^2,
\]
with layer-wise features \(\phi_\ell\) (normalized to \(\hat\phi_\ell\)) and learned weights \(w_\ell\). It correlates well with human judgments and captures perceptual structure. Note that it is still an \emph{input-space} metric here: features come from a reference network, not the backdoored model. Choice of backbone matters (e.g., VGG vs.\ AlexNet).

\subsubsection{Inception Score (IS)}
Originally for generative models~\cite{salimans2016is}, IS has been used pairwise to compare predictions for \(\beni\) vs.\ \(\adv\):
\[
\mathrm{IS}(\beni,\adv)=\mathrm{KL}\!\left(p(\cdot\,|\,\beni)\,\big\|\,p(\cdot\,|\,\adv)\right),
\]
where \(p(\cdot\,|\,\cdot)\) is the softmax of a fixed Inception network. Large values signal that the trigger changes the semantic prediction. IS depends on the chosen reference model and class set; it is not a purely perceptual measure.

\subsubsection{Spectral Angle Mapper (SAM)}
SAM~\cite{yuhas1992sam} treats each pixel as a 3D color vector and averages the angle between corresponding pixels:
\[
\mathrm{SAM}(\beni,\adv)=
\frac{1}{n}\sum_{i=1}^n
\arccos\!\left(\frac{\langle \beni_i,\adv_i\rangle}{\|\beni_i\|_2\,\|\adv_i\|_2}\right).
\]
Angles emphasize chromatic shifts and are invariant to per-pixel intensity scaling. Prior work reported good alignment with human judgments in attack settings~\cite{liu2022stealthiness}. It can be less sensitive to small structural (spatial) changes.

\subsection{Feature-space Stealthiness Metrics}
\label{sec:current_metrics:feature}
Measure whether latent representations of triggered inputs look indistinguishable from those of clean inputs, especially for the target class.

\subsubsection{Silhouette Score (SS)}
\label{sec:current_metrics:feature:ss}
Given embeddings \(\{\phi(x)\}\), the per-sample silhouette is
\[
s(i)=\frac{b(i)-a(i)}{\max\{a(i),\,b(i)\}},
\]
where \(a(i)\) is the average distance from sample \(i\) to others in its own cluster and \(b(i)\) is the minimum of the average distances to points in any other cluster~\cite{rousseeuw1987silhouette}. Values near \(1\) indicate well-separated clusters; near \(0\), overlapping; negative, likely mis-clustered. For backdoors, one typically forms two clusters (clean vs.\ triggered) for a fixed class, then averages \(s(i)\). Because high-dimensional distances are problematic, prior work reduces dimension first (ICA, t-SNE, or PCA)~\cite{herault1985ica}.

\subsubsection{Discriminant Sliced-Wasserstein Distance (DSWD)}
\label{sec:current_metrics:feature:dswd}
Let \(P\) and \(Q\) be distributions of embeddings for clean and triggered inputs (e.g., at the penultimate layer).
Define the 1D projections \(X^\theta=\langle\theta,X\rangle\) and \(Y^\theta=\langle\theta,Y\rangle\). Then
\begin{align*}
\mathrm{SWD}^2(P,Q)
&= \int_{\mathbb{S}^{d-1}} W_2^2\!\big(X^\theta,\,Y^\theta\big)\, d\theta \nonumber\\[-2pt]
&\approx \tfrac{1}{K}\sum_{k=1}^K W_2^2\!\big(X^{\theta_k},\,Y^{\theta_k}\big).
\end{align*}
DSWD~\cite{doan2021dswd} replaces random \(\theta_k\) with \emph{discriminant} directions derived from the classifier (e.g., class-separating weights), improving efficiency and sensitivity to class-relevant shifts. Lower DSWD indicates greater feature-space stealthiness.

% \subsubsection{Backdoor Mahalanobis Stealthiness (BMS)}
% \label{sec:current_metrics:feature:bms}
% The BMS measures the Mahalanobis distance between backdoor and clean features. The Mahalanobis distance is a measure of the distance between a point (vector) $\mathbf{x}$ and a distribution $D$. Unlike Euclidean distance, it accounts for the correlations between variables and the scale of the data.

% For a test vector $\mathbf{x} \in \mathbb{R}^D$ and a distribution defined by mean vector $\boldsymbol{\mu}$ and covariance matrix $\mathbf{\Sigma}$, the Mahalanobis distance $D_M(\mathbf{x})$ is defined as:
% \begin{align*}
%     D_M(\mathbf{x}) = \sqrt{ (\mathbf{x} - \boldsymbol{\mu})^T \mathbf{\Sigma}^{-1} (\mathbf{x} - \boldsymbol{\mu}) },
% \end{align*}
% where $\mathbf{x}$ is the observation vector (e.g., a feature vector from a neural network). $\boldsymbol{\mu}$ is the mean vector of the reference dataset. $\mathbf{\Sigma}$ is the covariance matrix of the reference dataset. $\mathbf{\Sigma}^{-1}$ is the inverse of the covariance matrix (also known as the Precision Matrix). The $ ^T$ denotes the matrix transpose.

% More specifically, we calculate the $\boldsymbol{\mu}$ and $\mathbf{\Sigma}^{-1}$ of the clean features. Then we apply $D_M$ by backdoor features. The final BMS score is the mean of the Mahalanobis distances of all backdoor features.



\subsection{Parameter-space Stealthiness Metrics}
\label{sec:current_metrics:parameter}

\subsubsection{Upper Bound of the Channel Lipschitz Constant (UCLC)}
UCLC was used by Zheng et al.\ in their Channel Lipschitz based Pruning (CLP) defense~\cite{zheng2022clp}. This defense takes inspiration from the Lipschitz constant, which indicates the sensitivity of a neural network's output to changes in the input. They adapted this metric to measure the sensitivity individually for each channel, or neuron, in the neural network, resulting in the channel Lipschitz constant (CLC). In the CLP defense, an upper bound of the CLC is evaluated for each neuron to prune the most sensitive neurons, which are most likely to contain the backdoor functionality.

UCLC has also been used by Xu et al. in the Adversarial Backdoor Injection (ABI) training mechanism of the Grond attack~\cite{xu2025grond}. Furthermore, they implemented this training mechanism in other backdoor attacks and found that it made them more resistant to parameter-space defenses as well.

\subsubsection{Trigger-Activated Change (TAC)}
Besides UCLC, Zheng et al. proposed another metric to measure channel sensitivity called TAC~\cite{zheng2022clp}. Whereas UCLC is a data-free metric, meaning it can be calculated solely from the model weights, TAC requires inputs containing the backdoor trigger. TAC is not designed to be used in backdoor defenses, since it would be unrealistic for defenders to have access to the trigger. However, in a benchmarking framework, TAC could serve as a critical oracle metric. It allows the evaluator to measure the precise sensitivity of the network to the known trigger. Zheng et al. proposed TAC to study backdoor behavior. Xu et al. also used TAC to illustrate the lack of parameter-space stealthiness of many backdoor attacks~\cite{xu2025grond}.

==> sections/tri-space.tex <==
% \section{Tri-Space Stealthiness: A Unified Metric}
% \label{sec:tri_space_stealthiness}

% Our empirical results indicate that existing backdoor attacks rarely achieve stealthiness simultaneously across the input, feature, and parameter spaces. Attacks that are visually imperceptible often leave traces in the feature or parameter space, and vice versa. To explicitly quantify this trade-off, we introduce a unified \textit{tri-space stealthiness} metric ($S_{tri}$) that aggregates the stealthiness contributions from all three domains into a single scalar score.

% \subsection{Per-Space Stealthiness Scores}
% We define a normalized stealthiness score $S_v \in [0, 1]$ for each view $v \in \{in, feat, param\}$, where $S_v \approx 1$ indicates that the backdoor is indistinguishable from benign behavior, and $S_v \approx 0$ indicates a clearly detectable footprint.

% \paragraph{Input Space ($S_{in}$)}
% In the input space, stealthiness is determined by the perceptual similarity between clean and triggered inputs. We utilize the SSIM~\cite{wang2004ssim}, which naturally provides a value in $[0, 1]$ and is an effective stealthiness metric judging by its results in Sections \ref{subsec:experimental_results_input} and \ref{subsec:interpreting_matrix}. We define the input-space stealthiness score directly as:
% \begin{equation}
%     S_{in} = \text{SSIM}(x, \mathcal{T}(x))
% \end{equation}
% where a value of 1 implies perfect perceptual stealthiness.

% \paragraph{Feature Space ($S_{feat}$)}
% In the feature space, we utilize the silhouette score (SS) proposed in Section~\ref{sec:new_metrics:cdbi}. Although we proposed CDBI to improve upon SS, we found that SS achieved slightly better results in Section \ref{subsec:interpreting_matrix}: SS had higher correlation with SPECTRE than CDBI, but otherwise the two metrics performed similarly. Recall that lower SS values indicate greater overlap between clean and triggered clusters, and thus higher stealthiness. We map the range of SS ($[-1, 1]$) to a probability-like score in $[0, 1]$ as follows:
% \begin{equation}
%     S_{feat} = (1 + \text{SS}) / 2
% \end{equation}
% % In the feature space, we utilize the Class-Specific Davies-Bouldin Index (CDBI) proposed in Section~\ref{sec:new_metrics:cdbi}. Recall that higher CDBI values indicate greater overlap between clean and triggered clusters, and thus higher stealthiness. To map the unbounded positive range of CDBI to a probability-like score in $[0, 1]$, we apply a saturation transform:
% % \begin{equation}
% %     S_{feat} = 1 - \exp(-\lambda_{f} \cdot \text{CDBI})
% % \end{equation}
% % where $\lambda_{f}$ is a scaling constant. Under this formulation, distinct clusters ($\text{CDBI} \to 0$) result in $S_{feat} \to 0$, while highly overlapping clusters ($\text{CDBI} \to \infty$) result in $S_{feat} \to 1$.

% \paragraph{Parameter Space ($S_{param}$)}
% In the parameter space, we employ the TAC-UCLC Product (TUP) defined in Section~\ref{sec:new_metrics:tup} as it performed well in Sections \ref{sec:new_metrics:results} and \ref{subsec:interpreting_matrix}. Since TUP measures the specific footprint of the trigger (where lower values indicate greater stealthiness), we model the stealthiness score as an exponential decay function:
% \begin{equation}
%     S_{param} = \exp(-\lambda_{p} \cdot \text{TUP})
% \end{equation}
% where $\lambda_{p}$ is a normalization factor derived from the benign model distribution. Here, a minimal parameter footprint ($\text{TUP} \approx 0$) yields $S_{param} \approx 1$.

% \subsection{Calibration of Scaling Constants}
% To ensure fair comparison across datasets with varying metric ranges, we calibrate the scaling constant $\lambda_{p}$ using the \textit{Median Anchor Method}. This method calibrates the score such that the median attack performance in a given dataset maps to a neutral stealthiness score of $0.5$.

% Deriving from the equations above, we calculate the constants for each dataset $D$ as:
% \begin{equation}
%     \lambda_{p}^{(D)} = \frac{\ln(2)}{\text{median}(\text{TUP}^{(D)})}
% \end{equation}
% % \begin{equation}
% %     \lambda_{f}^{(D)} = \frac{\ln(2)}{\text{median}(\text{CDBI}^{(D)})}, \quad \lambda_{p}^{(D)} = \frac{\ln(2)}{\text{median}(\text{TUP}^{(D)})}
% % \end{equation}
% This calibration ensures that the metric distributions are centered and comparable, preventing outliers in raw values (e.g., high TUP in CIFAR-100) from skewing the aggregated score.

% \subsection{Tri-Space Aggregation}
% To capture the comprehensive stealthiness of an attack, we aggregate the per-space scores. Consistent with the principle that a chain is only as strong as its weakest link, we define the \textit{Worst-Case Tri-Space Stealthiness} as the minimum score across all domains:
% \begin{equation}
%     S_{tri}^{\min} = \min(S_{in}, S_{feat}, S_{param})
% \end{equation}
% This metric ($S_{tri}^{\min}$) is high if and only if the attack is simultaneously stealthy in all three spaces. Additionally, to provide a balanced summary, we report the \textit{Geometric Mean Tri-Space Stealthiness}:
% \begin{equation}
%     S_{tri}^{geo} = \sqrt[3]{S_{in} \cdot S_{feat} \cdot S_{param}}
% \end{equation}

% \subsection{Results and Analysis}
% We report the tri-space stealthiness scores for all evaluated attacks in Table~\ref{tab:tri_space_results}.

% \begin{table*}[h!]
% \centering
% \footnotesize
% \caption{Tri-Space Stealthiness Evaluation. We report the Worst-Case ($S_{tri}^{\min}$) and Geometric Mean ($S_{tri}^{geo}$) stealthiness scores. $S_{tri}^{\min}$ reflects the ``loudest footprint'' principle, where a low score indicates high detectability in at least one domain. Best results are \textbf{bolded}.}
% \label{tab:tri_space_results}
% % \footnotesize
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Attack}} & \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{c}{\textbf{Tiny-ImageNet}} & \multicolumn{2}{c}{\textbf{Imagenette}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%  & $S_{tri}^{\min}$ & $S_{tri}^{geo}$ & $S_{tri}^{\min}$ & $S_{tri}^{geo}$ & $S_{tri}^{\min}$ & $S_{tri}^{geo}$ & $S_{tri}^{\min}$ & $S_{tri}^{geo}$ \\
% \midrule
% BadNets & 0.086 & 0.325 & 0.154 & 0.316 & 0.460 & 0.604 & 0.006 & 0.112 \\
% Blend & 0.500 & 0.636 & 0.338 & 0.507 & 0.473 & 0.579 & 0.479 & 0.551 \\
% WaNet & 0.402 & 0.553 & 0.247 & 0.493 & 0.482 & 0.705 & 0.225 & 0.430 \\
% BppAttack & 0.314 & 0.484 & 0.029 & 0.172 & 0.490 & 0.626 & 0.236 & 0.535 \\
% Adap-Patch & 0.338 & 0.674 & \textbf{0.539} & \textbf{0.692} & 0.498 & 0.626 & 0.536 & 0.728 \\
% Adap-Blend & 0.680 & 0.807 & 0.492 & 0.573 & 0.424 & 0.552 & 0.522 & 0.709 \\
% DFST & 0.381 & 0.554 & 0.111 & 0.339 & 0.324 & 0.492 & 0.255 & 0.379 \\
% Narcissus & 0.532 & 0.750 & 0.585 & 0.682 & 0.360 & 0.531 & 0.568 & 0.682 \\
% Grond & \textbf{0.827} & \textbf{0.916} & 0.500 & 0.645 & \textbf{0.511} & \textbf{0.669} & \textbf{0.757} & \textbf{0.868} \\
% DFBA & 0.338 & - & 0.511 & - & 0.458 & - & 0.028 & - \\
% \bottomrule
% \end{tabular}%
% % }
% \end{table*}

% The results quantitatively confirm that achieving comprehensive stealthiness is non-trivial. Older attacks like BadNets consistently score near zero in $S_{tri}^{\min}$ (e.g., 0.006 on Imagenette), primarily due to their poor parameter-space stealthiness ($S_{param} \approx 0$). In contrast, Grond achieves the highest consistent performance across datasets, with a worst-case score of 0.827 on CIFAR-10. This indicates that Grond is the only attack in our benchmark that effectively minimizes its footprint in all three domains simultaneously. Notably, attacks like WaNet, despite being visually imperceptible ($S_{in} \to 1$), suffer from moderate scores in the unified metric due to their detectability in the feature space. This underscores the necessity of the proposed unified metric for identifying the ``loudest footprint'' of a backdoor.


\section{Tri-Space Stealthiness: A Unified Metric}
\label{sec:tri_space_stealthiness}

Our empirical results indicate that existing backdoor attacks rarely achieve stealthiness simultaneously across the input, feature, and parameter spaces. %Attacks that are visually imperceptible often leave traces in the feature or parameter space, and vice versa. 
To explicitly quantify this trade-off, we introduce a unified \textit{tri-space stealthiness} metric ($S_{tri}$) that aggregates the stealthiness contributions from all three domains into a single scalar score.

\subsection{Per-Space Stealthiness Scores}
We define a normalized stealthiness score $S_v \in [0, 1]$ for each view $v \in \{in, feat, param\}$, where $S_v \approx 1$ indicates that the backdoor is indistinguishable from benign behavior, and $S_v \approx 0$ indicates a clearly detectable footprint.

\textbf{Input Space ($S_{in}$)}
In the input space, stealthiness is determined by the perceptual similarity between clean and triggered inputs. As shown in Figure~\ref{fig:residual_correlations}, almost all of the input space metrics demonstrate low or negative correlation with evaluated defenses. We use SSIM~\cite{wang2004ssim} because it better aligns with human perceptual judgments of structural stealthiness than pixel-wise $L_p$ norms, and it naturally yields values in $[0, 1]$. We define the input-space stealthiness score directly as:
\begin{equation}
    S_{in} = \text{SSIM}(x, \mathcal{T}(x)),
\end{equation}
where a value of 1 implies perfect perceptual stealthiness.

\textbf{Feature Space ($S_{feat}$)}
In the feature space, we utilize the CDBI proposed in Section~\ref{sec:new_metrics:cdbi}. Rather than generic cluster cohesion, which favors attacks that form multiple sub-clusters, CDBI explicitly targets the adversarial objective, hiding poisoned samples within the class-conditional distribution. As we can see in Figure~\ref{fig:residual_correlations}, CDBI shows high correlations among feature-space metrics and also ranks $2^{nd}$ best among all metrics (of all 3 spaces) in the Borda count ranking~\cite{dwork2001rank} (our other proposed metric TUP ranked $1^{st}$). Recall that higher CDBI values indicate greater overlap between clean and triggered clusters, and thus higher stealthiness. To map the unbounded positive range of CDBI to a probability-like score in $[0, 1]$, we apply a saturation transform:
\begin{equation}
    S_{feat} = 1 - \exp(-\lambda_{f} \cdot \text{CDBI}),
\end{equation}
where $\lambda_{f}$ is a scaling constant. Under this formulation, distinct clusters ($\text{CDBI} \to 0$) result in $S_{feat} \to 0$, while highly overlapping clusters ($\text{CDBI} \to \infty$) result in $S_{feat} \to 1$.

\textbf{Parameter Space ($S_{param}$)}
In the parameter space, we employ TUP defined in Section~\ref{sec:new_metrics:tup}, as it indicates a clear top correlated metric in Figure~\ref{fig:residual_correlations}. Since TUP measures the specific footprint of the trigger (where lower values indicate greater stealthiness), we model the stealthiness score as an exponential decay function:
\begin{equation}
    S_{param} = \exp(-\lambda_{p} \cdot \text{TUP}),
\end{equation}
where $\lambda_{p}$ is a normalization factor derived from the benign model distribution. Here, a minimal parameter footprint ($\text{TUP} \approx 0$) yields $S_{param} \approx 1$.

\subsection{Calibration of Scaling Constants}
To ensure fair comparison across datasets with varying metric ranges, we calibrate the scaling constants $\lambda_{f}$ and $\lambda_{p}$ using the \textit{Median Anchor Method}. This method calibrates the score such that the median attack performance in a given dataset maps to a neutral stealthiness score of $0.5$.

Deriving from the equations above, we calculate the constants for each dataset $D$ as:
\begin{equation}
    \lambda_{f}^{(D)} = \frac{\ln(2)}{\text{median}(\text{CDBI}^{(D)})}, \quad \lambda_{p}^{(D)} = \frac{\ln(2)}{\text{median}(\text{TUP}^{(D)})}.
\end{equation}
This calibration ensures that the metric distributions are centered and comparable, preventing outliers in raw values (e.g., high CDBI in Imagenette) from skewing the aggregated score.

\subsection{Tri-Space Aggregation}
To capture the comprehensive stealthiness of an attack, we aggregate the per-space scores. Consistent with the principle that a chain is only as strong as its weakest link, we define the \textit{Worst-Case Tri-Space Stealthiness} as the minimum score across all domains:
\begin{equation}
    S_{tri}^{\min} = \min(S_{in}, S_{feat}, S_{param}).
\end{equation}
This metric ($S_{tri}^{\min}$) is high if and only if the attack is simultaneously stealthy in all three spaces. Additionally, to provide a balanced summary, we report the \textit{Geometric Mean Tri-Space Stealthiness}:
\begin{equation}
    S_{tri}^{geo} = \sqrt[3]{S_{in} \cdot S_{feat} \cdot S_{param}}.
\end{equation}

\subsection{Results and Analysis}
We report the tri-space stealthiness scores in Table~\ref{tab:tri-space}. The results quantitatively confirm that achieving comprehensive stealthiness is a non-trivial challenge.

\textbf{Analysis.} The unified results highlight distinct stealthiness profiles. In the \textbf{High Poisoning Rate} regime, adaptive attacks like \textit{Adap-Blend} perform slightly better on CIFAR-10 ($S_{tri}^{\min}=0.682$) and Tiny-ImageNet ($0.548$), leveraging their ability to merge triggered features with benign distributions (high CDBI). \textit{Grond} also demonstrates robustness, achieving the highest scores on Imagenette ($0.791$) and competitive scores elsewhere.
In the \textbf{Low Poisoning Rate} regime, \textit{Grond} emerges as the clear leader in comprehensive stealthiness. It achieves the best $S_{tri}^{\min}$ on CIFAR-10 ($0.827$), Tiny-ImageNet ($0.511$), and Imagenette ($0.757$). This confirms that Grond's strategy of minimizing parameter-space footprints (via ABI) allows it to maintain stealthiness even when the attack budget is constrained, unlike older attacks (e.g., BadNets), which consistently score near zero in the worst-case metric due to their detectable parameter or feature anomalies. Notably, clean-label attacks like \textit{Narcissus} also show strong performance on CIFAR-100 ($0.585$), benefitting from the natural feature overlap inherent in clean-label poisoning.


\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\caption{Tri-Space Stealthiness ($S_{tri}$) for High ($\approx 5\%$) and Low ($\approx 0.3\%$) Poisoning Rates. Min and Geo refer to $S_{tri}^{\min}$ and $S_{tri}^{geo}$ respectively. C10: CIFAR-10, C100: CIFAR-100, T-IN: Tiny-ImageNet, Inet: Imagenette. Best results in \textbf{bold}.}
\label{tab:tri-space}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Attack} & \multicolumn{2}{c}{\textbf{C10}} & \multicolumn{2}{c}{\textbf{C100}} & \multicolumn{2}{c}{\textbf{T-IN}} & \multicolumn{2}{c}{\textbf{Inet}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & Min & Geo & Min & Geo & Min & Geo & Min & Geo \\
\midrule
\rowcolor[gray]{.95} \multicolumn{9}{l}{\textit{High Poisoning Rate ($\approx 5\%$)}} \\
BadNets    & 0.156 & 0.396 & 0.158 & 0.385 & 0.147 & 0.414 & 0.069 & 0.186 \\
Blend      & 0.500 & 0.636 & 0.500 & 0.579 & 0.434 & 0.554 & 0.520 & 0.608 \\
WaNet      & 0.344 & 0.534 & 0.184 & 0.403 & 0.266 & 0.474 & 0.128 & 0.326 \\
BppAttack  & 0.090 & 0.343 & 0.030 & 0.232 & 0.002 & 0.091 & 0.116 & 0.247 \\
Adap-P.    & 0.382 & 0.635 & 0.409 & 0.660 & 0.517 & \textbf{0.761} & 0.435 & 0.592 \\
Adap-B.    & \textbf{0.682} & \textbf{0.750} & 0.516 & 0.666 & \textbf{0.548} & 0.647 & 0.512 & 0.605 \\
DFST       & 0.457 & 0.599 & 0.412 & 0.544 & 0.399 & 0.535 & 0.108 & 0.350 \\
Narcissus  & 0.513 & 0.598 & \textbf{0.558} & 0.701 & 0.360 & 0.516 & 0.615 & 0.645 \\
Grond      & 0.557 & 0.749 & 0.554 & \textbf{0.770} & 0.546 & 0.668 & \textbf{0.791} & \textbf{0.886} \\
DFBA       & 0.310 & --    & 0.493 & --    & 0.480 & --    & 0.140 & --    \\
\midrule
\rowcolor[gray]{.95} \multicolumn{9}{l}{\textit{Low Poisoning Rate ($\approx 0.3\%$)}} \\
BadNets    & 0.086 & 0.325 & 0.154 & 0.316 & 0.460 & 0.604 & 0.006 & 0.112 \\
Blend      & 0.500 & 0.636 & 0.338 & 0.507 & 0.473 & 0.579 & 0.479 & 0.551 \\
WaNet      & 0.402 & 0.553 & 0.247 & 0.493 & 0.482 & 0.705 & 0.225 & 0.430 \\
BppAttack  & 0.314 & 0.484 & 0.029 & 0.172 & 0.490 & 0.626 & 0.236 & 0.535 \\
Adap-P.    & 0.338 & 0.674 & 0.539 & \textbf{0.692} & 0.498 & 0.626 & 0.536 & 0.728 \\
Adap-B.    & 0.680 & 0.807 & 0.492 & 0.573 & 0.424 & 0.552 & 0.522 & 0.709 \\
DFST       & 0.381 & 0.554 & 0.111 & 0.339 & 0.324 & 0.492 & 0.255 & 0.379 \\
Narcissus  & 0.532 & 0.750 & \textbf{0.585} & 0.682 & 0.360 & 0.531 & 0.568 & 0.682 \\
Grond      & \textbf{0.827} & \textbf{0.916} & 0.500 & 0.645 & \textbf{0.511} & \textbf{0.669} & \textbf{0.757} & \textbf{0.868} \\
DFBA       & 0.338 & --    & 0.511 & --    & 0.458 & --    & 0.028 & --    \\
\bottomrule
\end{tabular}
\end{table}



==> sections/tsne.tex <==
\section{t-SNE Embeddings for ResNet18} 
\label{sec:tsne}

The t-SNE feature space embeddings of the backdoored ResNet18 models on the CIFAR-10, CIFAR-100, and Imagenette datasets are shown in Figures~\ref{fig:tsne_resnet18_cifar10},~\ref{fig:tsne_resnet18_cifar100}, and~\ref{fig:tsne_resnet18_imagenette}, respectively. The silhouette scores results provided in~\autoref{sec:results:feature} are based on these t-SNE embeddings.

